Computing High-dimensional Confidence Sets for Arbitrary Distributions

We study the problem of learning a high-density region of an arbitrary distribution over $\mathbb{R}^d$. Given a target coverage parameter $\delta$, and sample access to an arbitrary distribution $D$, we want to output a confidence set $S \subset \mathbb{R}^d$ such that $S$ achieves $\delta$ coverage of $D$, i.e., $\mathbb{P}_{y \sim D} \left[ y \in S \right] \ge \delta$, and the volume of $S$ is as small as possible. This is a central problem in high-dimensional statistics with applications in finding confidence sets, uncertainty quantification, and support estimation. In the most general setting, this problem is statistically intractable, so we restrict our attention to competing with sets from a concept class $C$ with bounded VC-dimension. An algorithm is competitive with class $C$ if, given samples from an arbitrary distribution $D$, it outputs in polynomial time a set that achieves $\delta$ coverage of $D$, and whose volume is competitive with the smallest set in $C$ with the required coverage $\delta$. This problem is computationally challenging even in the basic setting when $C$ is the set of all Euclidean balls. Existing algorithms based on coresets find in polynomial time a ball whose volume is $\exp(\tilde{O}( d/ \log d))$-factor competitive with the volume of the best ball. Our main result is an algorithm that finds a confidence set whose volume is $\exp(\tilde{O}(d^{1/2}))$ factor competitive with the optimal ball having the desired coverage. The algorithm is improper (it outputs an ellipsoid). Combined with our computational intractability result for proper learning balls within an $\exp(\tilde{O}(d^{1-o(1)}))$ approximation factor in volume, our results provide an interesting separation between proper and (improper) learning of confidence sets.

==> Algorithm/alg_filter_procedure.tex <==
\begin{figure}[!htb]
\begin{tcolorbox}
\begin{center}
    \textbf{Procedure} $\textsc{Iterative\_Filter}$
\end{center} 
\textbf{Input:} a set of points $\whY$\\
\textbf{Output:} an ellipsoidal shape $M$
\begin{enumerate}
    \item Set $\whY_0 = \whY$, $n_0 = \widehat\beta |\whY_0|$, the mean $\mu_0 = \frac{1}{|\whY_0|} \sum_{y \in \whY_0} y$, and the normalized covariance
    \begin{equation} \label{eq:sigmaupdate}
    \whSigma_0 = \frac{1}{n_0} \sum_{y \in \whY_0} (y-\whmu_0)(y-\whmu_0)^\top. 
    \end{equation}
        
    The set $\whY_t$ and its mean $\whmu_t$ are updated using the following iterative algorithm in the natural way; but the normalized covariance $\whSigma_t$ is always updated as a sum of squared deviations over the samples in the current $\whY_t$ divided by (the original) $n_0$. 
    
    \item Run the following algorithm iteratively: (until the number of high variance directions is less than $\beta'' V^*$ for some appropriate $\beta''=\poly\log d$) \anote{condition is meant as a comment}
    \begin{enumerate}
        \item Compute the eigenvectors $\whv_1, \dots, \whv_d$ of $\whSigma_t$ and let $\whlambda_1^2, \dots, \whlambda_d^2$ be its corresponding eigenvalues. Let $\whBig_t=\{i \in [d]: \whlambda_i^2 \ge \tau_t^2 \}$, and let $\Projj{t}{\tau_t}$ be the projection onto the subspace spanned by those eigenvectors corresponding to eigenvalues $\whlambda_i$ for $i \in \whBig_t$.
        
        \item If $|\whBig_t| \le \beta'' V^*/\tau_t^2$, then set the ellipsoidal shape $M$ as follows.
        For $|\whBig_t| = 0$, set $M=\sum_{i=1}^d a_i^2 \whv_i \whv_i^\top$, where $a_i = 1$.
        For $|\whBig_t| > 0$, set $M=\sum_{i=1}^d a_i^2 \whv_i \whv_i^\top$, where
        where $a_i = \beta_4 d$ if $\whlambda_i \ge \tau_t$ and $a_i = 1-\gamma$ otherwise, for $\gamma=\EV_{\tau_t}(\whY_t)/d$ and $\beta_4$ as given in Definition~\ref{def:goodep}; return $M$ and complete the algorithm.  
        \item Remove from $\whY_t$ all the $y$ such that 
        \[\norm{\Projj{t}{\tau_t}(y-\whmu_t)}_2^2 > \beta' V^* + \beta \tau_t^2  |\whBig_t| \]
         Update $\whmu_t$ and $\whSigma_t$ as in \eqref{eq:sigmaupdate} \[\whmu_t = \frac{1}{|\whY_t|} \sum_{y \in \whY_t} y, \text{ and } \whSigma_t=  \frac{1}{n_0} \sum_{y \in \whY_t} (y-\whmu_t)(y-\whmu_t)^\top,   \]
         and start the next iteration with the updated $\whY_t, \whmu_t, \whSigma_t$.
    \end{enumerate}
\end{enumerate}
\end{tcolorbox}
\caption{Procedure $\textsc{Iterative\_Filter}$ for filtering high variance directions}
\label{fig:algo_filter}
\end{figure}

==> Algorithm/alg_good_ellipsoid.tex <==
\begin{figure}[ht]
\begin{tcolorbox}
\begin{center}
    \textbf{Algorithm} $\textsc{Good\_Ellipsoid}$ \textbf{for finding a good ellipsoid}
\end{center}
\textbf{Input:} a set of point $Y'$, target fraction $\delta$\\
\textbf{Output:} a list of ellipsoidal shape $\{M_1,\dots, M_\ell\}$
\begin{enumerate}
    \item Guess a target $V^*$ which is within a $(\tfrac{1}{\delta})$-factor of $\EV_{\tau^*}(Y^{*})$, i.e. $\EV_{\tau^*}(Y^{*})/\delta \leq V^* \leq \EV_{\tau^*}(Y^{*})$ for $\delta = \delta_1\delta_2$, where $\EV_{\tau^*}(Y^{*})$ is the total variance along the high variance directions of the good set $Y^*$. %Also, guess $s^* = |\{i: \lambda_i(\Sigma_{Y^*}) \ge \tau\}|$. 
    
    \item Set parameter $\tau_1=\beta \tau$, where $\beta = d^{o(1)}$. %Set $\sigma_{ub}^2 = 2V^*$. \anote{We can also guess this, but a weak bound of $V^*$ is enough. }
    
    \item Run the list-decodable mean estimation algorithm of~\cite{diakonikolas2020list} on the points $Y'$ and target fraction $\delta = \delta_1 \delta_2$ to obtain a list of $m = O(1/\delta)$ subsets  
    $Y_1, \cdots, Y_m$ of $Y'$. 
    Let $Y^* \subseteq Y'$ be the unknown inliers.
    Among these candidate subsets, there exists a candidate subset $Y_i$ that satisfies (1) $\norm{\mu(Y_i) - \mu(Y^{*})}_2 \leq O(\log(1/\delta)/\sqrt{\delta})\sigma^*$; (2) $|Y_i| \geq \delta|Y'|/2$; (3) $|Y_i \cap Y^*| \geq |Y^*|/2$.
    
    \item For each subset $Y_i$ for $i\in[m]$ in the list returned by Step 3, call the Procedure \textsc{Iterative\_Filter} with input $\whY = Y_i$, and output $M_i$ returned by this procedure for each $Y_i$.
    
    %The remaining algorithm is run on each subset $Y_i$ for $i\in[m]$ in the list returned by Step 3. 
    % Define $n_0 := \widehat\beta |\whY|$ and 
    % \begin{equation} \label{eq:sigmaupdate}
    % \whSigma = \frac{1}{n_0} \sum_{x \in \whY} (x-\whmu)(x-\whmu)^\top.  
    % \end{equation}
    % The set $\whY$ and its mean $\whmu$ are updated using the following iterative algorithm in the natural way; but $\whSigma$ is always updated as a sum of squared deviations over the samples in the current $\whY$ divided by (the original) $n_0$. As shown later, $|\whY| \ge  n_0/2$ throughout the whole algorithm. 

    %\item Run the filtering algorithm of~\cite{diakonikolas2016robust} and~\cite{lai2016agnostic} with $\sigma = \sigma_{ub}$ to get a set $\whX \subset X \cap B'$ of size $(1-O(\alpha))|X \cap B'|$ with variance at most $O(\sigma_{ub}^2)$ in every direction, and let $\whmu$ be its mean; 
    %\anote{For $\delta$ fraction instead of $1-\alpha$ fraction, we can replace the above with a List-Decodable mean estimation algorithm with variance bound $V^*$. Does the list-decodable mean estimation algorithm also output a subset $\whX_j$ of size $\Omega(\delta)$ for which it is the empirical mean? }
    %The remaining algorithm is run on $\whX$. The set $\whX$ and its mean $\whmu$ are updated using the following iterative algorithm in the natural way; but $\whSigma$ is always updated as a sum of squared deviations over the samples in the current $\whX$ divided by (the original) $n_0$. As we will see later, $|\whX| \ge (1-O(\alpha))n_0$ for the whole algorithm.    
%     \item Run the following algorithm iteratively: (until the number of high variance directions is more than $\beta'' V^*$ for some appropriate $\beta''=d^{o(1)}$) \anote{condition is meant as a comment}
%     \begin{enumerate}
%         \item Compute the eigenvectors $\whv_1, \dots, \whv_d$ of $\whSigma$ and let $\whlambda_1^2, \dots, \whlambda_d^2$ be its corresponding eigenvalues. Let $\whBig=\{i \in [d]: \whlambda_i \ge \tau_1 \}$, and let $\whProj_{hi}$ be the projection onto the subspace spanned by those eigenvectors corresponding to eigenvalues $\whlambda_i$ for $i \in \whBig$.
%         \item If $|\whBig| \le \beta'' V^*$, then set $M=\sum_{i=1}^d a_i^2 \whv_i \whv_i^\top$, where $a_i = \beta_4 d$ if $\whlambda_i \ge \tau_1$ and $a_i = 1-\gamma$ otherwise, where $\gamma=\EV_{\tau_1}(\whX)/d$ and $\beta_4$ is as given as in Definition~\ref{def:goodep}; return $M$ and complete the algorithm.  
%         \item Remove from $\widehat{X}$ all the $x$ such that 
%         \[\norm{\whProj_{hi}(x-\whmu)}_2^2 > \beta' V^* + \tau^2 \beta |\whBig| \]
%          Also set as in \eqref{eq:sigmaupdate} \[\whmu = \frac{1}{|\whX|} \sum_{x \in \whX} x, \text{ and } \whSigma=  \frac{1}{n_0} \sum_{x \in \whX} (x-\whmu)(x-\whmu)^\top,   \]
%          and start the next iteration with the updated $\whX, \whmu, \whSigma$.
%     \end{enumerate}
 \end{enumerate}
\end{tcolorbox}
\caption{Algorithm $\textsc{Good\_Ellipsoid}$ for finding a good ellipsoid}
\label{fig:algo_ellipsoid}
\end{figure}

==> Algorithm/alg_greedy_density.tex <==
\begin{figure}[htbp]
\begin{tcolorbox}

\begin{center}\textbf{Algorithm} \textsc{Greedy\_Density}\end{center}

\textbf{Input:} coverage level $\delta \in (0,1)$, slack $\gamma \in (0, (1-\delta)/2)$, number of sets $k \in \Z_{> 0}$, error $\varepsilon \in (0,\gamma/4k)$, and failure probability $\delta' \in (0,1)$ \\
\textbf{Output:} confidence set $\widehat C \subseteq \R^d$
%\hline
%\vspace{10pt}
%\hline

%\noindent {\bf Algorithm Greedy Density}
 \begin{enumerate}
     \item Set $t=0$ and $\widehat C_t = \varnothing$. %Parameter $\gamma,k$ (by default set $\gamma = \alpha/8,k=1$). 
     \item Repeat (until $\widehat C_t$ covers at least $\delta$ probability mass):
     \begin{enumerate}
     \item Draw $n = O(k^2 D\log (kD)\log(1/\delta)/(\gamma\varepsilon^2))$ $i.i.d.$ fresh samples $Y_{t+1}$ from $\calD$.
     \item Select $S_{t+1} \in \calF$ that maximizes the empirical density:
     \begin{align}\label{eq:greedy_program}
     S_{t+1}= \arg\max_{S \in \calF}~~ & \frac{|Y_{t+1}\cap (S \setminus \widehat C_t)|}{\vol(S)}  \\
     \text{ s.t. }&  \frac{|Y_{t+1} \cap (S \setminus \widehat C_t)|}{n} \ge \frac{\gamma}{2k}, ~\text{and}~ \frac{|Y_{t+1} \cap S|}{n} \le \delta+\gamma+3\varepsilon. \nonumber
     \end{align}
     \item Update $\widehat C_{t+1} = \widehat C_t \cup S_{t+1}$
     \item If $|Y_{t+1} \cap \widehat C_{t+1}|/n \ge \delta+\varepsilon$, then STOP and output $\widehat C = \widehat C_{t+1}$; \\Else $t\leftarrow t+1$ and loop. 
     \end{enumerate}
 \end{enumerate}

\end{tcolorbox}
\label{fig:alggreedy}
\caption{Algorithm for finding the small  confidence set}
\end{figure}

==> Paper/ellipsoids.tex <==
\newcommand{\ProjSigmahi}{\Pi_{\Sigma,hi}}
\section{Finding Smaller Ellipsoidal Prediction Sets}

\anote{Work in progress.}
We will use the following notion of good ellipsoids, whose axes directions and lengths are approximately aligned with the covariance matrix of the points inside the ball. Moreover, the conditions of the ellipsoid ensure that the ellipsoid is not skinny in any direction, and is elongated in the large variance directions. A good ellipsoid $E_M$ for a ball $B$ will be of smaller size but continue to contain most (but not all) of the points that belong to $B$. Furthermore, as in the previous section, the choice of ellipsoid $E_M$ will depend on the covariance matrix of the points inside the optimal ball $B^*$. However, we do not have access to $B^*$, but to a larger ball $B' \supseteq B^*$. Our goal in this section is to use the points in the bigger ball $B'$ and an appropriate scaling (that is guessed) to construct an ellipsoid $E_M$ that is a {\em good ellipsoid} for $B^*$. 


We will consider a simpler choice of ellipsoids $E_M$ from the family $\calM$ where the eigenvalues of corresponding matrix $M$ only take on two possible values $\{O(\sqrt{d}),1-\gamma\}$ for some appropriate choice of $\gamma \in (0,1)$: 
\begin{equation}\label{eq:threelevels}
\calM=\Big\{M: \lambda_i(M) \in \{a^2, 1-\gamma\} \Big\},  
\end{equation}
for some appropriate value of $a^2$ where $\lambda_1(M), \dots, \lambda_d(M)$ are the eigenvalues of $M$. \anote{Can change if needed.}


\anote{Should we change it to "Good Ellipsoidal shape"?}
\begin{definition}[Good Ellipsoid]\label{def:goodep}
%There exists constants $c_1, c_2 \ge 1$ such that the following holds. 
Consider a ball $B=\Ball(0,R)$ containing points $Y$, and ellipsoid $E_M$ given by $E_M=\{x: x^\top M x \le R^2\} \in \calM$. Let the covariance matrix of $Y$ be $\Sigma_Y$ with % $\Sigma_X= R^2 \cdot U \diag(\lambda) U^\top$, where 
eigenvalues $\eigval_1^2 R^2/d, \dots, \eigval_d^2 R^2/d$, \footnote{Note that $\sum_{i=1}^d \sigma_i^2 \leq d$ since points $Y$ are contained in $B = \Ball(0,R)$ and $\sum_{i=1}^d \sigma_i^2R^2/d = \tr(\Sigma_Y) = \E_Y\|x-\E_Y(x)\|^2 \leq R^2$.} and for any $\tau \ge 1$, 
let $\EV_\tau(Y)=\sum_{i: \sigma_i \geq \tau} \sigma_i^2$ denote the excess variance of $Y$.
%let $\EV_\tau(Y)=\sum_{i=1}^d (\max\{\eigval_i^2 -\tau^2,0\})R^2/d$ denote the excess variance of $Y$. 
The ellipsoid is said to be $(\tau, \beta)$-{\em good} for $B,Y$ if there exists $\tau \ge 1$ and  $1 \le \beta_1\le  \beta_2 \le  \beta_3 \le \beta$ and $1 \le \beta_4, \beta_5 \le \beta$ such that
\begin{enumerate}
    \item[(i)]Let the eigendecompostion of $M$ be  $V \diag(a)^2 V^\top$ with eigenvalues $a_1^2, \dots, a_d^2$. Then the eigenvalues satisfy $\forall i \in [d], ~ a_i^2 \in \{\beta_4 d,1-\gamma\}$ for some $\gamma \in (0,1/4)$  s.t. 
    \lnote{
    $$
    \text{If } \EV_\tau(Y) > \sqrt{d} \tau, \text{then } \frac{\EV_{\tau} (Y)}{\beta_3 d} \le \gamma \le \frac{ \EV_\tau (Y)}{\beta_2 d}; \quad\text{Otherwise, } \gamma=0. %\text{ and } a_i^2=1 ~\forall i \in [d].
    $$
    }
    \[ \frac{\EV_{\tau} (Y)}{\beta_3 R^2} \le \gamma \le \frac{ \EV_\tau (Y)}{\beta_2 R^2} \text{ if } \EV_\tau(Y) \ge \frac{R^2}{d}. ~~~\text{ Otherwise } \gamma=0, \text{ and } a_i^2=1 ~\forall i \in [d]. \label{eq:gamma:cond}\]
    \anote{double check the otherwise condition. It's meant to be the trivial case.}
%and \anote{need to add something about the total $a_i^2$?}
    \item[(ii)]  \anote{Needs to be adjusted.}{\em (Elongated along high variance directions)} We want \[\forall v, ~~v^\top M v \ge \frac{1}{2\tau^2} v^\top \Sigma_Y v\] and if $\ProjMhi$ be the projector onto the subspace $\spn(\{v_i: a_i > 1\})$ corresponding to large eigenvalues of $M$ and $\Pi_{\Sigma,hi}$ is the projector onto the eigenspace corresponding to eigenvalues of $\Sigma$ that are at least $\tau^2 R/d$, we have \[\forall x:~ \norm{\Pi_{\Sigma, hi} x}_2^2 \ge \eta \EV_\tau(Y) ~\implies~ \norm{\ProjMhi x}_2^2 \ge \frac{\tau^2}{\beta_1 d} \cdot \eta \EV_\tau(Y)\]
     \anote{Reworking:
    $M \succeq \frac{\lambda_{\max}(M)}{\beta_1} \Sigma_Y $.
     Let $\ProjMhi$ be the projector onto the subspace $\spn(\{v_i: a_i > 1\})$ corresponding to large eigenvalues of $M$. For any eigenvector $u \in \R^d$ of $\Sigma_Y$ such that $u^\top \Sigma_Y u \ge \tau^2 R^2/d$, we have \anote{changed definition. Can also write it as $\Pi_{M,hi} \Pi_{\Sigma,>\tau^2} \Pi_{M,hi}\succeq \frac{1}{\beta_1}\Pi_{\Sigma, >\tau^2}$ }
     \begin{equation}\label{eq:goodep:cond1}
         \norm{\ProjMhi u}_2^2 \ge 1/\beta_1, \text{ and } \forall v, ~~v^\top M v \ge \frac{1}{\beta_1} v^\top \Sigma_Y v
     \end{equation}
     }
% \anote{The second part is separate and more easily guaranteed.}
    \item[(iii)] The number of high eigenvalues of $M$ is upper bounded i.e.,
    \lnote{$|\{i: a_i^2 >1 \}| \leq \frac{\beta_5 \EV_\tau(Y)}{\tau^2}$.}
    $|\{i: a_i^2 >1 \}| \leq \frac{\beta_5 d \EV_\tau(Y)}{\tau^2 R^2}$. \anote{The $\cdot /\tau^2$ doesn't really matter since $\beta_5$ can swallow it up; just there to give sense of scale. }
\end{enumerate}
%We will call the quantity $\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2$ 
\end{definition}
In the above definition, we will think of $\beta, \tau = (\log d)^{O(1)}$. \anote{or is it $d^{o(1)}$? }

The following lemma motivates our definition of a good ellipsoid $E_M$ by showing that the ellipsoid has smaller volume than $B$, brings down the maximum variance and retains many points in $Y$.  

\begin{lemma}[Properties of good ellipsoids]\label{lem:goodep}
Consider a ball $B=\Ball(0,R)$ containing points $Y$. Let ellipsoid $E_M$ given by $E_M=\{x: x^\top M x \le R^2\}$ be a $(\tau,\beta)$-good ellipsoid for $B,Y$ with the large eigenvalue $\lambda_{\max}(M)=\beta_4 d$ for $\beta_4 \geq \max\{\frac{\beta_1}{\tau^2}, 4\ln d,\frac{\beta_2}{2}\}$. The number of large eigenvalues of $M$ is $\frac{\beta_5 \EV_\tau(Y)}{\tau^2}$ for $\beta_5 \leq \frac{\tau^2}{2\beta_3 \beta_4}$. Then, the following properties hold %There exists universal constants $c_1, c_2 \ge 1$ such that %for any $\delta>0$,
\begin{enumerate}
     \item[(a)] The points in $Y$ have bounded variance in the transformed space $M^{-1/2} x$ i.e.,  for each unit vector $u \in \R^d$, $\Var_{x \unif Y}[\iprod{M^{-1/2} x,u}] \le O(\tau^2 R^2/d)$. 
     \item[(b)] 
     The volume of $E_M$ is at most 
     $$
     \vol(E_M) \leq \vol(B) \cdot \exp\left(d^{1-c_2+o(1)}\right).
     $$
     %is smaller i.e.,
     %$$
     % \vol(E_M) \le \vol(B) \cdot \exp\left(-\frac{4\ln d -2}{4}\right).
     % $$
     %$ \vol(E_M) \le \vol(B) \cdot \exp\Big( - c_2 \big(\tau^2 \beta \log (\beta d)\big)^{-1} \cdot \EV_\tau (Y) \Big).$
     %\anote{We may not need this much improvement?}
     \item[(c)] Most points with non-negligible mass on the high variance directions also belong to $E_M$ i.e., for $\eta \leq 1/d^\varepsilon$ for a small constant $\varepsilon$, we have that for any point $x \in Y$, it holds 
     $$\sum_{i: \eigval_i^2 \ge \tau^2} \iprod{x , u_i}^2 \ge \eta \EV_\tau(Y) ~~\implies~~ x \in E_M. $$
     \anote{Earlier it was $\E[\sum_{i: \eigval_i^2 \ge \tau} \iprod{x , u_i}^2]$ instead of $\EV_\tau(Y)$. Dependencies need to be checked. }
     \vnote{Can this just be the length of the projection onto the high eigenspace?  This looks like the squared length?}
     % \begin{align}
     %     \Pr_{X}\Big[ \sum_{i \in \tBig] \iprod{x , v_i}^2 \le \eta \E_X[\sum_{i \in \tBig] \iprod{x , v_i}^2]\Big] \le 1-\delta  ~~\implies~ \Pr_X[x \notin E_M] \le \delta + c.
     % \end{align} 
     %For at least $1-\delta$ fraction of the points, we have that the length of $x$ restricted to the coordinates $\tBig$ is significantly smaller than its expectation i.e., \[\sum_{i \in \tBig} x_i^2 \le \eta \sum_{i \in \tBig} r_i^2, \label{eq:case2}\] 
%     \item[(iii)] 
 \end{enumerate}

\end{lemma}
\begin{proof}
We show that the good ellipsoid satisfies all properties.

\noindent \textbf{Property (a):} The first property (a) follows from property (ii) of good ellipsoids with $\beta_1 \leq \beta_4 \tau^2$. To upper bound the variance of $M^{-1/2} x$ along every direction by $O(\tau^2 R^2/d)$, it suffices to prove that for 
$$\forall u \in \R^d, ~ \frac{u^\top \Sigma_Y u}{u^\top M u} \le O(\tau^2 R^2/d).$$
On the one hand, for directions $u$ with variance $u^\top \Sigma_Y u$ at least $\tau^2 R^2/d$, property (ii) implies that 
$$u^\top M u \ge \lambda_{\max}(M) \norm{\ProjMhi u}_2^2 \ge \beta_4 d \cdot \frac{1}{\beta_1} \ge \frac{\beta_4 d}{\beta_1} \cdot \frac{u^\top \Sigma_Y u}{R^2} \ge  \frac{d}{\tau^2 R^2} \cdot u^\top \Sigma_Y u, $$
as required, since $\beta_1 \le \beta_4 \tau^2$ and $u^\top \Sigma_Y u \leq R^2$. On the other hand, if the variance $u^\top \Sigma_Y u$ is smaller than $\tau^2 R^2/d$, then we can use the fact that $a_i^2 \ge 1/2$ to get property (a).  %In particular for every large variance direction $u$ with variance at least $\tau R^2/d$, \eqref{eq:goodep:cond1} ensures that the variance of $M^{-1/2} x$ along $u$ is $u M^{-1/2} \Sigma_X M^{-1/2}$
%uses $M \succeq \beta \Sigma$. Hence for any unit vector $u \in \R^d$
%$$\Cov_X[M^{-1/2} x] = M^{-1/2} \Sigma_X M^{-1/2} \preceq (\beta \Sigma_X)^{-1/2} \Sigma_X (\beta \Sigma_X)^{-1/2} \preceq \big(\tfrac{1}{\beta}\big)  I. $$

\noindent \textbf{Property (b):} We now show property (b). %Let $M_0 = \tfrac{1}{\tau^2} \Sigma_X + (1-\gamma/c) I$. 
%\anote{Can move some of the following description to the proof overview.}
Let $a_1^2, \dots, a_d^2$ be the eigenvalues of $M$ and let $v_1, \dots, v_d$ be its corresponding eigenvectors. Compared to the ball $B=\{x: \sum_i x_i^2 \le R^2\}$,  the volume of $E_M$ is 
$\vol(E_M)/\vol(B)  = a_1 a_2 \cdots a_d$ i.e., 
$$2\ln\Big(\frac{\vol(E_M)}{\vol(B)}\Big) = \sum_{i=1}^d \ln(a_i^2).$$ 
Hence the quantity $\vol(E_M)/\vol(B) \le 1$ if $a_1^2 + \dots + a_d^2 \le d$ by the AM-GM inequality; in fact, the more skewed the values $\{a_i: i \in [d]\}$, the smaller it is as given by Claim~\ref{claim:concavity} which uses the concavity of the logarithm function. However, in our case $\sum_i a_i^2$ is larger than $d$, since some the large eigenvalues of $M$ have been magnified by a $\poly(d)$ factor. However, since there are only a few of them and from properties of the logarithm function, we can appeal to Claim~\ref{claim:robust_concavity} which gives a robust analogue of Claim~\ref{claim:concavity}.  


First, we consider the case where the excess variance $\EV_{\tau}(Y) \leq \sqrt{d} \tau$. In this case, we have $\gamma = 0$. Note that the number of big eigenvalues in $M$ is at most $|\tBig_M| \leq \beta_5 \cdot \EV_\tau(Y) \leq \EV_\tau(Y)$ since $\beta_5 < 1$. Thus, we have
$$
2\ln\Big(\frac{\vol(E_M)}{\vol(B)}\Big) = \sum_{i=1}^d \ln(a_i^2) = |\tBig_M| \ln(\beta_4 d) \leq \sqrt{d}\tau \ln(\beta_4 d),
$$
where the last inequality is from $|\tBig_M| \leq \EV_\tau(Y) \leq \sqrt{d}\tau$. Since $\beta_4 = O(\poly\log d)$ and $\tau = d^{1/2-c_2}$, we get the required volume bound on $\vol(E_M)$.

Suppose the excess variance $\EV_{\tau}(Y) > \sqrt{d}\tau$.
Let $\tBig_M = \{i \in [d]: a_i^2 >1\}$ and $\tSmall_M = \{i \in [d]: a_i^2 <1\}$ refer to the big and small eigenvalues of $M$ respectively. 
We first note that $M$ is a good ellipsoid, and by property (iii) we have the number of big eigenvalues is at most $|\tBig_M| = |\{i \in [d]: a_i^2 > 1\}| \leq  \beta_5 \cdot \EV_\tau(Y)$.
By the definition of the excess variance $\EV_\tau(Y)$, we have the number of large eigenvalues $|\tBig_M|$ is 
$$
|\tBig_M| \leq \beta_5 \cdot \EV_\tau(Y) = \beta_5 \cdot \sum_{i: \sigma_i \geq \tau} \sigma_i^2.
$$
Since $\beta_5 < 1/2$, and $\sum_{i=1}^d \sigma_i^2 \leq d$, we have $|\tBig_M| \leq d/2$ and $|\tSmall_M| \geq d/2$. Thus, we have 
\begin{align*}
\sum_{i: a_i^2\leq 1 } a_i^2 = (1-\gamma) | \tSmall_M| \le d- |\tBig_M| - \frac{\gamma d}{2}.    
\end{align*}
Since the excess variance $\EV_\tau(Y) > 0$, then we have $\gamma \geq \frac{\EV_\tau(Y)}{\beta_3 d}$. 
Since $\beta_3 \leq \frac{1}{2\beta_5 \beta_4}$, we have 
$$
\sum_{i: a_i^2 > 1} \frac{a_i^2}{d} = \beta_4 |\tBig_M| \leq \beta_4 \cdot \beta_5 \cdot \EV_\tau(Y) \leq \frac{d}{2} \cdot \frac{\EV_\tau(Y)}{\beta_3 d} \leq \frac{d\gamma}{2}. 
$$
Then, we let $b_i^2 = a_i^2 = 1-\gamma$ for $a_i^2 \leq 1$ and $b_i^2 = a_i^2/d = \beta_4$ for $a_i^2 = \beta_4 d > 1$.  Therefore, we have 
$$
\sum_{i=1}^d b_i^2 = \sum_{i: a_i^2 \geq 1} \frac{a_i^2}{d} + \sum_{i: a_i^2< 1 } a_i^2 \leq d.
$$
By Claim~\ref{claim:robust_concavity}, we have the ratio of the volumes $\vol(E_M)$ and $\vol(B)$ is at most
$$
\frac{\vol(E_M)}{\vol(B)} \leq \exp\left(-\frac{1}{4} \sum_{i=1}^d \max\{b_i^2 - 2, 0\} \right) \leq \exp\left(-\frac{4\ln d-2}{4}\right),
$$
where the last inequality is due to $\beta_4 \geq 4\ln d$ and $|\tBig_M| \geq 1$.


\noindent \textbf{Property (c):} Finally, we verify property (c).
Let $\Zbig(y)=\sum_{i: \eigval_i^2 \ge \tau^2} \iprod{y, u_i}^2$ be the mass of $y$ in the high-variance directions, where $u_i$ is the eigenvector of $\Sigma_Y$ corresponding to eigenvalue $\sigma_i^2R^2/d$. 
Consider a point $y \in Y$ such that $\Zbig(x) \ge \eta \EV_\tau(Y) R^2/d$ as assumed in the property (c). 
Let $y_i = \iprod{y,v_i}$, where $v_i$ be the eigenvector of $M$ corresponding to eigenvalue $a_i^2$. 
We will now use the condition that $\sum_{i=1}^d y_i^2 \leq R^2$ is deterministically true (for $y \in B$) to show that most such point $y$ with $\Zbig(y) \ge \eta \EV_\tau(Y) R^2/d$ is contained in $E_M$. 
For ellipsoid $E_M$, the coefficient of $y_i^2$ for $i \in \tBig_M$ is very small (it is $1/a_i^2 =O(1/d)$), while the coefficient for $y_i^2$ for $i \in \tSmall_M$ is slightly larger than $1$ (it is $(1-\gamma)^{-1}$).
The main intuition is that if $\Zbig(y)$ is not negligible i.e., $\Zbig(y) \ge \eta \EV_\tau(Y)$, then the mass of $y$ on the directions in $\tSmall_M$ is upper bounded by $R^2 - \Zbig(y)$. This is sufficiently smaller than $R^2$ to compensate for the extra factor of $(1+\gamma)$.  


First, we consider any point $y \in Y$ that satisfies $\sum_{i: \sigma_i^2 \geq \tau^2} \iprod{x,u_i}^2\geq \eta\EV_{\tau}(Y) R^2/d$.
Let $\Proj_Y^{\geq \tau}$ be the projection onto the eigenspace of $\Sigma_Y$ with eigenvalues at least $\tau^2$. Thus, we have for this point $y$
$$
\norm{\Proj_Y^{\geq \tau} y}_2^2 \geq \eta \EV_\tau(Y)R^2/d.
$$
Since the eigenvalues are at least $\tau^2$ for the eigenspace used in the projection $\Proj_Y^{\geq \tau}$, we have 
$$
y^\top \Proj_Y^{\geq \tau} \Sigma_Y \Proj_Y^{\geq \tau} y \geq \tau^2 \eta \EV_\tau(Y)R^2/d.
$$
By the property (ii) of the good ellipsoid, we have $M \succeq \frac{1}{\beta_1}\Sigma_Y$. Thus, we have for this point $y$, 
$$
y^\top M y \geq \frac{1}{\beta_1} y^\top \Sigma_Y y \geq \tau^2 \eta \EV_\tau(Y)\frac{R^2}{\beta_1 d}.
$$
Let $\Proj_M^{\geq 1}$ be the projection onto the eigenspace of $M$ with eigenvalues at least $1$, corresponding to the big directions in $\tBig_M$. Let $\Proj_M^{< 1}$ be the projection onto the complement space of $\Proj_M^{\geq 1}$. 
Then, we have 
$$
y^\top M y = y^\top \Proj_M^{\geq 1} M \Proj_M^{\geq 1} y + y^\top \Proj_M^{< 1} M \Proj_M^{< 1} y.
$$
Since $y \in \Ball(0,R)$, we have 
$$
y^\top \Proj_M^{< 1} M \Proj_M^{< 1} y \leq \norm{\Proj_M^{< 1} y}_2^2 \leq \norm{y}_2^2 \leq R^2. 
$$
Therefore, we have 
$$
y^\top \Proj_M^{\geq 1} M \Proj_M^{\geq 1} y \geq y^\top M y - y^\top \Proj_M^{< 1} M \Proj_M^{< 1} y \geq \tau^2 \eta \EV_\tau(Y) \frac{R^2}{\beta_1 d}  - R^2.
$$
Since the large eigenvalues in $M$ are $\beta_4 d$, we get
$$
\norm{\Proj_M^{\geq 1}y}_2^2 \geq \frac{y^\top \Proj_M^{\geq 1} M \Proj_M^{\geq 1} y}{\beta_4 d} \geq \frac{\tau^2 \eta \EV_\tau(Y) R^2}{\beta_4 \beta_1 d^2} -\frac{R^2}{\beta_4 d}.
$$
Let $v_i$ be the eigenvector of $M$ corresponding to eigenvalue $a_i^2$. 
Let $y_i = \iprod{y,v_i}$. Since this point $y \in B = \Ball(0,R)$,  $\sum_{i=1}^d y_i^2 \le R^2$. 
Thus, we have 
$$
\sum_{i \in \tSmall_M} y_i^2 = \sum_{i=1}^d y_i^2 - \sum_{i \in \tBig_M} y_i^2 \leq R^2 - \frac{\tau^2 \eta \EV_\tau(Y) R^2}{\beta_4 \beta_1 d^2} +\frac{R^2}{\beta_4 d}.
$$
Then, we show that this point $y$ is contained in $E_M$.
If $\EV_\tau(Y) \leq \sqrt{d}\tau$, then we have $\gamma = 0$. In this case, since all eigenvalues of $M$ are at least $1$, all points in $Y \subseteq \Ball(0,R)$ are also contained in $E_m$. 
Next, we consider the case where $\EV_\tau(Y) > \sqrt{d}\tau$. In this case, we have
\begin{align*}
    \sum_{i=1}^d \frac{y_i^2}{a_i^2} &= \frac{1}{\beta_4 d}  \sum_{i \in \tBig_M} y_i^2  + \frac{1}{1-\gamma} \sum_{i \in \tSmall_M} y_i^2\\
    &\leq \frac{R^2}{\beta_4 d} + (1+2\gamma) \cdot \left(R^2 - \frac{\tau^2 \eta \EV_\tau(Y) R^2}{\beta_4 \beta_1 d^2} +\frac{R^2}{\beta_4 d}\right)\\
    &\leq R^2 + R^2\left((2+2\gamma)\frac{1}{\beta_4 d} + 2\gamma  - (1+2\gamma)\frac{\tau^2 \eta \EV_\tau(Y)}{\beta_4 \beta_1 d^2} \right).
\end{align*}
By property (i) of the good ellipsoid, we have $\gamma \leq \frac{\EV_\tau(Y)}{\beta_2 d}$ for some $\beta_2 = O(1/d^{c_1})$ for a small constant $c_1$. We also have $\beta_1, \beta_4 = O(\poly \log d)$ and $\eta = 1/d^\varepsilon$ for a small constant $\varepsilon \ll c_1$. Since $\tau = d^{1/2-c_2}$ for some constant $c_2 \leq (c_1 - 2\varepsilon)/2$, we have 
$$
(2+2\gamma)\frac{1}{\beta_4 d} + 2\gamma = O\left(\frac{1}{d^{c_1}}\right) \leq O\left(\frac{1}{d^{2c_2+2\varepsilon}}\right) \leq (1+2\gamma)\frac{\tau^2 \eta \EV_\tau(Y)}{\beta_4 \beta_1 d^2},
$$
which implies that point $y$  is contained in $E_M$.


\lnote{old proof}


Let $\tBig_M = \{i \in [d]: a_i^2 >1\}$ and $\tSmall_M = \{i \in [d]: a_i^2 <1\}$ refer to the big and small eigenvalues of $M$ respectively. To use Claim~\ref{claim:robust_concavity} we first note that $M$ is a good ellipsoid, and by property (iii) we have $|\tBig_M| = |\{i \in [d]: a_i^2 > 1\}| \leq  \beta_5 \cdot d\EV_\tau(Y)/(\tau^2R^2)$.
Hence the total contribution to $\sum_{i=1}^d a_i^2$ from the large eigenvalues of $M$ is  
$$
\sum_{i: a_i^2 > 1} a_i^2 = |\tBig_M| \cdot  \beta_4 d \leq \beta_4 d \cdot \beta_5 \frac{d\EV_\tau(Y)}{\tau^2 R^2}.
$$ 
By the definition of the excess variance $\EV_\tau(Y)$, we have the number of large eigenvalues $|\tBig_M|$ is 
$$
|\tBig_M| \leq \beta_5 \cdot \frac{d\EV_\tau(Y)}{\tau^2R^2} = \beta_5 \cdot \frac{\sum_{i=1}^d \max\{\sigma_i^2 - \tau^2,0\}}{\tau^2}.
$$
Since $\beta_5 \leq \tau^2/2$, and $\sum_{i=1}^d \sigma_i^2 \leq d$, we have $|\tBig_M| \leq d/2$ and $|\tSmall_M| \geq d/2$. Thus, we have 
\begin{align*}
\sum_{i: a_i^2\leq 1 } a_i^2 = (1-\gamma) | \tSmall_M| \le d- |\tBig_M| - \frac{\gamma d}{2}.    
\end{align*}
If the excess variance $\EV_\tau(Y) \geq R^2/d$, then we have $\gamma \geq \frac{\EV_\tau(Y)}{\beta_3 R^2}$. 
Since $\beta_5 \leq \frac{\tau^2}{2\beta_3 \beta_4}$, we have 
$$
\sum_{i: a_i^2 > 1} \frac{a_i^2}{d}  \leq \beta_4 \cdot \beta_5 \cdot \frac{d\EV_\tau(Y)}{\tau^2 R^2} \leq \frac{d}{2} \cdot \frac{\EV_\tau(Y)}{\beta_3 R^2} \leq \frac{d\gamma}{2}. 
$$
Then, we let $b_i^2 = a_i^2 = 1-\gamma$ for $a_i^2 \leq 1$ and $b_i^2 = a_i^2/d = \beta_4$ for $a_i^2 = \beta_4 d > 1$.  Therefore, we have 
$$
\sum_{i=1}^d b_i^2 = \sum_{i: a_i^2 \geq 1} \frac{a_i^2}{d} + \sum_{i: a_i^2< 1 } a_i^2 \leq d.
$$
By Claim~\ref{claim:robust_concavity}, we have the ratio of the volumes $\vol(E_M)$ and $\vol(B)$ is at most
$$
\frac{\vol(E_M)}{\vol(B)} \leq \exp\left(-\frac{1}{4} \sum_{i=1}^d \max\{b_i^2 - 2, 0\} \right) \leq \exp\left(-\frac{4\ln d-2}{4}\right),
$$
where the last inequality is due to $\beta_4 \geq 4\ln d$ and $|\tBig_M| \geq 1$.

% If $\EV_\tau(Y) < R^2/d$, then we have $a_i^2 = 1$ for all $i \in [d]$.

%Let $\tBig=\{i \in [d]: \eigval_i^2 \ge \tau^2\}$ refer to the large eigenvalues. %To use Claim~\ref{claim:robust_concavity}, we first note that $|\tBig| \le 2\EV_\tau(Y)/\tau^2$. 

%\lnote{Why do we need this? The number of big eigenvalues is bounded using the following property, right?} \anote{You're right. I changed property (iii) slightly, and forgot to update this part.}
% To use Claim~\ref{claim:robust_concavity} we first not that $M$ is a good ellipsoid, and by property (iii) we have $|\{i \in [d]: a_i^2 > 1\}| \le  O(\beta_5) \cdot \EV_\tau(Y)/\tau^2$. Hence the total contribution to the log-volume from the large eigenvalues of $M$ is  $$\sum_{i: a_i^2 > 1} \log(a_i^2) \le |\{i: a_i > 1\}| \cdot  \log (\max_i a_i^2) \le O\Big(\beta_5  \log (\beta_4 d)\Big) \cdot \frac{\EV_\tau(Y)}{\tau^2}.$$ 
% Let $\tBig_M = \{i \in [d]: a_i^2 >1\}$ and $\tSmall_M = \{i \in [d]: a_i^2 <1\}$ refer to the big and small eigenvalues of $M$ respectively. Note $|\tSmall_M| \ge d/2$ since $\tau^2 \ge 2$.  
% Moreover, the value of $\gamma$ is chosen so that %the contribution to the log-volume from the rest of the eigenvalues ($\{i: a_i^2 \le 1\}$) is
% \begin{align*}
% \sum_{i: a_i^2< 1 } a_i^2 = (1-\gamma) | \tSmall_M| \le d- |\tBig_M| - \frac{\gamma d}{2} \le d - \Omega(\EV_\tau(Y)).    
% \end{align*}

% \anote{Need to verify definition of $\gamma$ to replace the $\Omega(\cdot)$ by an appropriate $\beta$... There's slack here if needed, but the robust claim needs to match this.}\anote{Liren, see above.}

Finally, we verify property (c).
%\anote{Need to copy paste the proof from my notes.}
Let $\Zbig(x)=\sum_{i: \eigval_i^2 \ge \tau^2} \iprod{x, u_i}^2$ be the mass of $x$ in the high-variance directions, where $u_i$ is the eigenvector of $\Sigma_Y$ corresponding to eigenvalue $\sigma_i^2R^2/d$. Consider a point $x \in Y$ such that $\Zbig(x) \ge \eta \EV_\tau(Y)$ as assumed in property (c). 
Let $x_i = \iprod{x,v_i}$, where $v_i$ be the eigenvector of $M$ corresponding to eigenvalue $a_i^2$. 
We will now use the condition that $\sum_{i=1}^d x_i^2 \le R^2$ is deterministically true (for $x \in B$) to show that most such $x \in E_M$. 
For ellipsoid $E_M$, the coefficient of $x_i^2$ for $i \in \tBig_M$ is very small (it is $1/a_i^2 =O(1/d)$), while the coefficient for $x_i^2$ for $i \in \tSmall_M$ is slightly larger than $1$ (it is $(1-\gamma)^{-1}$). The main intuition is that if $\Zbig(x)$ is not negligible i.e., $\Zbig(x) \ge \eta \EV_\tau(Y)$, then the mass of $x$ on the directions in $\tSmall_M$ is upper bounded by $R^2 - \Zbig(x)$. This is sufficiently smaller than $R^2$ to compensate for the extra factor of $(1+\gamma)$.  
%\anote{Add the intuitive explanation... about how Markov inequality doesn't work. }


First we see that 
\begin{align*}
\norm{\ProjMhi x}_2^2 \ge \frac{1}{\beta_4 d} (x^\top M x - .....  \sum_{i=1}^d \iprod{x,u_i}^2 u_i^\top \ProjMhi u_i \ge \frac{1}{\beta_1} \Zbig(x) \ge \frac{\eta}{\beta_1} \EV_\tau(Y).
\end{align*}


\anote{Need to replace this:}Let $u_i$ be the eigenvector of $\Sigma_Y$ corresponding to eigenvalue $\sigma_i^2R^2/d$. Since the high-variance direction $u_i$ corresponding to $\sigma_i^2 \geq \tau^2$ satisfies $u_i^\top \Sigma_Y u_i \geq \tau^2R^2/d$, we have $\norm{\ProjMhi u_i}_2^2 
 \geq \frac{1}{\beta_1}$ by the property (ii) of good ellipsoid.
Thus, we observe that 
\begin{align*}
\norm{\ProjMhi x}_2^2 \ge \sum_{i=1}^d \iprod{x,u_i}^2 u_i^\top \ProjMhi u_i \ge \frac{1}{\beta_1} \Zbig(x) \ge \frac{\eta}{\beta_1} \EV_\tau(Y).
\end{align*}

Let $v_i$ be the eigenvector of $M$ corresponding to eigenvalue $a_i^2$. Let $x_i = \iprod{x,v_i}$. Since this point $x \in B = \Ball(0,R)$,  $\sum_{i=1}^d x_i^2 \le R^2$. Thus, we have $\sum_{i \in \tSmall_M} x_i^2 = \sum_{i=1}^d x_i^2 - \sum_{i \in \tBig_M} x_i^2 \leq R^2 - \eta\EV_\tau(Y)/\beta_1$.
Hence, we have 
\begin{align*}
\sum_{i \in \tSmall_M} \frac{\iprod{x,v_i}^2}{(1-\gamma)} & \le \frac{1}{1-\gamma} \Big(R^2 - \frac{\eta}{\beta_1} \EV_\tau(Y)\Big),
% \end{align*}
% \begin{align*}
\text{ and } \sum_{i \in \tBig_M} \frac{\iprod{x,v_i}^2}{a_i^2}  = \frac{1}{\beta_4 d} \sum_{i \in \tBig_M} \iprod{x,v_i}^2 \le \frac{R^2}{\beta_4 d}.
\end{align*}
Combining them, 
\begin{align*}
\sum_{i \in [d]} \frac{\iprod{x,v_i}^2}{a_i^2} & \le \frac{R^2}{\beta_4 d}+ \frac{1}{1-\gamma} \Big(R^2 - \frac{\eta}{\beta_1} \EV_\tau(Y)\Big) \\
&\le \frac{R^2}{\beta_4 d} + \left(1 + \frac{\gamma}{1-\gamma}\right) R^2 - \frac{\eta}{\beta_1} \EV_\tau(Y) \le R^2 + R^2 \Big( \frac{1}{\beta_4 d} + 2\gamma - \frac{\eta \EV_\tau(Y)}{\beta_1 R^2}\Big). 
\end{align*}
Since $\gamma \le \EV_\tau(Y)/ (\beta_2 R^2)$, $\eta \geq 4\beta_1/\beta_2$, $\beta_4 \geq \beta_2/2$, and $\EV_\tau(Y) \geq R^2/d $, we have
\begin{align*}
\sum_{i \in [d]} \frac{\iprod{x,v_i}^2}{a_i^2} &\leq R^2 + R^2 \Big( \frac{1}{\beta_4 d} + \frac{2\EV_\tau(Y)}{\beta_2 R^2} - \frac{4 \EV_\tau(Y)}{\beta_2 R^2}\Big) \\
&\leq R^2 + R^2 \Big( \frac{1}{\beta_4 d} - \frac{2 \EV_\tau(Y)}{\beta_2 R^2}\Big) \\
&\leq R^2,
\end{align*}
which implies $x\in E_M$. 
\end{proof}

The above lemma requires that $\Zbig(x) > \eta \cdot \EV_\tau(Y)$ to show that $x \in E_M$. While we may expect this to be true in typical distributions, there may be cases when the large variance for these coordinates arises from just a few points which put all its mass on these few high variance directions. The next lemma shows that we can avoid the final precondition on $x$ by grouping the $x$ into different ranges based on their values for $\Zbig$.
\anote{Should add a figure that shows the bad situation where the high variances in some directions are actually because of a small fraction of points with high mass on those big variance directions. }

\anote{Need to set the parameters accordingly. }
\begin{lemma} \label{lem:covering-good-ellipsoids} 
%Suppose $\varepsilon \in (0,1)$ and $1 \le \tau \le (\log d)^{O(1)}$ are given, and 
%Suppose $\tau \ge 2$. 
Suppose there is a ball $B=\Ball(0,R)$ containing points $Y$. There exists parameters $\delta=O(1/ \log d), \eta = 1/d^{\varepsilon}$ for $\varepsilon \in (0,1)$, such that %$\delta >1/(\log^{O(1)} d)$ and $\beta \ge 1$ with $\beta, \beta' = d^{o(1)}$ and $\eta \in (0,1)$ with $\eta \ge d^{-o(1)}$  \anote{aiming to set $L=O(\log d/\log log d), \beta, \tau = (\log d)^{O(1)}$} such that 
there exists a subset $Y^* \subseteq Y$ of size $|Y^*| \ge \frac{1}{\log^{1/\varepsilon} d} \cdot |Y|$ and $(\tau^*)^2 \in (2, 4^{1+1/\varepsilon}\log^{1/\varepsilon} d)$ such that if $\Sigma^*$ is the covariance matrix of $Y^*$ and $\Projj{*}{\tau^*}$ is the projection matrix onto the eigenspace with eigenvalues greater than $\tau^*$, then one of the following properties holds
\begin{enumerate}
    \item $\lambda_{\max}(\Sigma^*) \le (\tau^*)^2$;
    \item there exists $\Yin \subseteq Y^*$ of size $|\Yin| \geq (1-\delta) |Y^*|$ \vnote{\((1 - \delta)\)? or just \(\delta\)?} \vnote{It would be nice to rename this \(\delta_3\), since \(\delta\) already means the fraction of points in the optimal solution. } such that for any $y \in \Yin$,
    $$
    \norm{\Proj^{>\tau^*}_{*} y}_2^2 \ge \eta \cdot \EV_{\tau^*}(Y^*).
    $$
\end{enumerate}
%\[  \text{either } \lambda_{\max}(\Sigma^*) \le 4\tau^2 , \text{ or } \Pr_{x \unif Y^*}\Big[\norm{\Proj^{>\tau}_{*} x}_2^2 \ge \eta \cdot \EV_{\tau}(Y^*) \Big] \ge 1-\delta \]
Note that the covariance $\Sigma^*$ and corresponding projector $\Proj^{>\tau}_*$ is for the set $Y^*$ and not $Y$. 
%such that there are disjoint subsets $Y_1, \dots, Y_L \subseteq Y$ with $|Y_1 \cup \dots \cup Y_L| \ge (1-\varepsilon)|Y|$ and $\beta_1, \dots, \beta_L \ge 1$ and  $1 \le \tau_1 \le \tau_2 \dots \le  \tau_L \le d^{o(1)}$ such that the following holds:\\ for $j \in [L]$, if $\Sigma_j$ is the covariance matrix of the (unknown) $Y_j$ and $\Projj{Y_j}{\tau_j}$ is the projection operator on to the eigenspace of $\Sigma_j$ corresponding to eigenvalues larger than $\tau_j$, then for all $j \in [L], x \in Y_j$, we have that $\norm{\Projj{Y_j}{\tau_j} x}_2^2 \ge \eta \cdot \EV_{\tau_j}(Y_j)$.  
\anote{removed: and ellipsoids $E_{M_1}, \dots, E_{M_L}$  corresponding to matrices $M_1, E_2, \dots, M_L$ such that:\\
(i) $Y_j \subset E_{M_j}$ for all $j \in [L]$, (ii) $E_{M_j}$ is a $(\tau,\beta)$-good ellipsoid for the ball $B$ and the set of points $Y_j$.} 


% \begin{itemize}
%     \item $Y
% \end{itemize}
\end{lemma}
\newcommand{\Ygood}{Y_{\textrm{good}}}
\newcommand{\Ybad}{Y_{\textrm{bad}}}
\newcommand{\Zbigg}[1]{\Zbig^{(#1)}}
%\anote{May need to rewrite the above lemma to include an algorithm that finds these good ellipsoid shapes...}
\begin{proof}
%\anote{Will fill this in later; sketch:}
Set $L=1/\varepsilon$, $\delta = 1/\log d$, $\eta=1/d^\varepsilon$.  
Given $Y \subset \Ball(0,R)$, we construct the sets $Y^{(0)}=Y, Y^{(1)}, \dots, Y^{(L)}$ until we produce a set $Y^*$ that satisfies the desired property. 
Let $\Sigma_j$ be the covariance matrix for $Y^{(j)}$. 
We set $\tau_0^2 = 2$ and $\tau_j^2 = 2\cdot (4/\delta)^j$ for $j \in [L]$.
For each $j \ge 0$, we define $\Projj{j}{\tau_j}$ to be the projection onto eigenspace of the covariance $\Sigma_j$ of $Y^{(j)}$ with eigenvalues greater than $\tau_j$. 
Then we define 
\begin{align*}
    Y^{(j+1)} &= \{y \in Y^{(j)}: \norm{\Projj{j}{\tau_j} y}_2^2 < \eta \cdot \EV_{\tau_j}(Y^{(j)}) \}, 
    \text{ and } \whY^{(j)}= Y^{(j)} \setminus Y^{(j+1)}. 
\end{align*}

We inductively maintain the property that $|Y^{(j)}| \ge \delta^j |Y| \geq \frac{1}{\log^{1/\varepsilon} d}|Y|$.
Note that $|Y_0| = |Y|$ which satisfies this property.
We then consider any level $j \in [L]$ and suppose $|Y^{(j)}| \ge \delta^j |Y|$.
We consider the following two cases: (1) $|\whY^{(j)}| \ge (1-\delta) |Y^{(j)}|$; (2) $|\whY^{(j)}| < (1-\delta) |Y^{(j)}|$.

\noindent \textbf{Case 1:}
If $|\whY^{(j)}| \ge (1-\delta) |Y^{(j)}|$, then 
we show that the set $Y^{(j)} \subseteq Y$ satisfies the required properties. The size of $Y^{(j)}$ is at least $|Y^{(j)}| \ge \delta^j |Y| \geq \frac{1}{\log^{1/\varepsilon} d}|Y|$. 
We also have the set $\whY^{(j)} \subseteq Y^{(j)}$ of size $|\whY^{(j)}| \ge (1-\delta) |Y^{(j)}|$ satisfies 
for any $y \in Y'$,
    $$
    \norm{\Proj^{>\tau}_{*} y}_2^2 \ge \eta \cdot \EV_{\tau}(Y^*).
    $$

%$Y^{(j)}$ already satisfies the properties of the lemma, and we are done. 
\noindent \textbf{Case 2:}
Suppose $|\whY^{(j)}| < (1-\delta) |Y^{(j)}|$. Then, we have $|Y^{(j+1)}|\ge \delta |Y^{(j)}| \geq \delta^{j+1} |Y|$. This implies that $\Sigma_{j+1} \preceq \frac{1}{\delta} \Sigma_j$. Then, we set $\tau_{j+1}^2 = 4\tau_j^2 /\delta$. We now show that the excess variance decreases by a factor of $4\eta$, i.e. $\EV_{\tau_{j+1}}(Y^{(j+1)}) \leq 4\eta \cdot \EV_{\tau_{j}}(Y^{(j)})$. By the definition of $\Projj{j+1}{\tau_{j+1}}$, we have
\begin{align*}
    \EV_{\tau_{j+1}}(Y^{(j+1)}) = \sum_{i: \sigma_i^{(j+1)} \geq \tau_{j+1}} \left(\sigma_i^{(j+1)}\right)^2 =\tr\left(\Projj{j+1}{\tau_{j+1}}\Sigma_{j+1}\Projj{j+1}{\tau_{j+1}}\right),
\end{align*}
where $\sigma^{(j+1)}_i$ is the eigenvalues of the covariance $\Sigma_{j+1}$.

By Claim~\ref{claim:trace_decompose} with $\Sigma_1 = \Sigma_{j}$, $\Sigma_2 = \Sigma_{j+1}$, $\Pi_1 = \Projj{j}{\tau_{j}}$, $\Pi_2 = \Projj{j+1}{\tau_{j+1}}$, and $c = 1/\delta$, we have
\begin{align}\label{eq:excess_variance_decompose}
    &\EV_{\tau_{j+1}}(Y^{(j+1)}) = \tr\left(\Projj{j+1}{\tau_{j+1}}\Sigma_{j+1}\Projj{j+1}{\tau_{j+1}}\right) \nonumber \\
    &\leq 2\tr\left(\Projj{j}{\tau_{j}}\Sigma_{j+1}\Projj{j}{\tau_{j}}\right) + \frac{2}{\delta} \cdot \|\Projjperp{j}{\tau_{j}}\Sigma_{j}\Projjperp{j}{\tau_{j}}\|_2\cdot \rank\left(\Projj{j+1}{\tau_{j+1}}\right), 
\end{align}
where $\Projjperp{j}{\tau_{j}} = I - \Projj{j}{\tau_{j}}$ is the projection onto the eigenspace of $\Sigma_{j}$ with eigenvalues at most $\tau_j$.

By the definition of $Y^{(j+1)}$, for any $y \in Y^{(j+1)}$ we have $\norm{\Projj{j}{\tau_j} y}_2^2 < \eta \cdot \EV_{\tau_j}(Y^{(j)})$. Thus, we have the first term in the right-hand side of~(\ref{eq:excess_variance_decompose}) is at most
\begin{align*}
    \tr\left(\Projj{j}{\tau_{j}}\Sigma_{j+1}\Projj{j}{\tau_{j}}\right) = \frac{1}{|Y^{(j+1)}|}\cdot \sum_{y \in Y^{(j+1)}} \norm{\Projj{j}{\tau_j} y}_2^2 \leq \eta \cdot \EV_{\tau_j}(Y^{(j)}).
\end{align*}

We now consider the second term in the right-hand side of~(\ref{eq:excess_variance_decompose}). Since $\Projjperp{j}{\tau_{j}}$ projects any vector onto the eigenspace of $\Sigma_{j}$ with eigenvalues at most $\tau_j$, we have 
$\|\Projjperp{j}{\tau_{j}}\Sigma_{j}\Projjperp{j}{\tau_{j}}\|_2  \leq \tau_j^2$. Since $\tau_j^2 \leq \delta\tau_{j+1}^2/4$, we have 
\begin{align*}
    \frac{2}{\delta} \cdot \|\Projjperp{j}{\tau_{j}}\Sigma_{j}\Projjperp{j}{\tau_{j}}\|_2\cdot \rank\left(\Projj{j+1}{\tau_{j+1}}\right) &\leq \frac{2}{\delta} \cdot \tau_j^2 \cdot \rank\left(\Projj{j+1}{\tau_{j+1}}\right) \\
    &\leq \frac{1}{2}\EV_{\tau_{j+1}}(Y^{(j+1)}).
\end{align*}

Combining two parts of~(\ref{eq:excess_variance_decompose}), we get
\begin{align*}
    \EV_{\tau_{j+1}}(Y^{(j+1)}) \leq 2\eta \cdot \EV_{\tau_{j}}(Y^{(j)}) + \frac{1}{2}\cdot \EV_{\tau_{j+1}}(Y^{(j+1)}), 
\end{align*}
which implies $\EV_{\tau_{j+1}}(Y^{(j+1)}) \leq 4\eta \cdot \EV_{\tau_{j}}(Y^{(j)})$. 
%%%%%%%%%%%%%%%%%
 
% Hence $\Projj{j+1}{\tau_{j+1}} \preceq \Projj{j}{\tau_j}$. Moreover, 
% \begin{align*}
% \forall x \in Y^{(j+1)}, ~~\norm{\Projj{j}{\tau_j} x}_2^2 &\le \eta \cdot \EV_{\tau_j}(Y^{(j)})  \\
% \implies \forall x \in Y^{(j+1)},~~ \norm{\Projj{j+1}{\tau_{j+1}} x}_2^2 &\le \eta \cdot \EV_{\tau_j}(Y^{(j)})\\
% \text{Hence, } \EV_{\tau_{j+1}}(Y^{(j+1)}) &\le \E_{x \unif Y^{(j+1)}}\norm{\Projj{j+1}{\tau_{j+1}} x}_2^2 \le \eta \cdot \EV_{\tau_j}(Y^{(j)}).
% \end{align*}
Furthermore, $|Y^{(j+1)}| \ge \delta |Y^{(j)}| \ge \delta^j |Y| \ge \frac{1}{\log^{1/\varepsilon} d} \cdot |Y|$ since $\delta = 1/\log d$. Finally from our choice of $\eta = 1/d^{\varepsilon}$, we see that after $L=1/\varepsilon$ iterations, as $\eta^L \le 1/d$, we get that $\EV_{\tau_{L-1}}(Y^{(L-1)}) \le \eta^L \cdot d \leq \tau_L^2$, which implies $\lambda_{\max}(\Sigma_{Y^{(L)}}) \leq \tau_L^2$. Hence, in the next iteration, the algorithm succeeds. 

% We have levels of sets $Y_0=Y$, thresholds $\tau_0$ and the big sets. $\Ygood=\{x \in Y: \Zbigg{0}(x) \ge \eta \EV_{\tau_0}(Y)\}$. If $\Pr[x \in \Ygood ] \ge 1- \delta_0$, then we are done; we will throw out the rest. If $\delta_0$ is not negligible, then we set $Y_1 = Y_0 \setminus \Ygood$, and set $\tau_1 = \tau_0/\delta_0$. Simple observation that no new direction is added to $\tBig_1$ i.e., $\tBig_1 \subset \tBig_0$. Also  $\EV_{\tau_1}(Y_1) \le \eta \EV_{\tau_0}(Y_0)$, since every point in $Y_1$ has $Z_{Big,0}(x) \le \eta \EV_{\tau_0}(Y)$ i.e., has much smaller mass on the big coordinates than before. And then recurse $O(\log d/ \log(1/\eta))$ times...  

% \anote{I have worked out a recursive procedure that seems to work with parameters like $d^{\eps}$ for any $\eps>0$; but I now think a bucketting procedure also likely works with a better tradeoff. Need to work it out.}

\end{proof}

\begin{claim}\label{claim:trace_decompose}
    For any two $d\times d$ projection matrices $\Pi_1$ and $\Pi_2$ and any two PSD matrices $\Sigma_1$ and $\Sigma_2$ with $\Sigma_2 \preceq c \Sigma_1$ for some $c > 0$, it holds that
    $$
    \tr(\Pi_2 \Sigma_2 \Pi_2) \leq 2\tr(\Pi_1 \Sigma_2 \Pi_1) + 2c\cdot \norm{\Pi_1^\perp \Sigma_1 \Pi_1^\perp}_2 \cdot \rank(\Pi_2).
    $$
\end{claim}

\begin{proof}
    Let $\Pi_1^\perp$ be the projection onto the orthogonal complement of the space onto which $\Pi_1$ projects. Then, we have $\Pi_1 + \Pi_1^\perp = I$. Thus, we have
    \begin{align*}
        \tr(\Pi_2 \Sigma_2 \Pi_2) &= \tr( \Pi_2 (\Pi_1 + \Pi_1^\perp) \Sigma_2 (\Pi_1 + \Pi_1^\perp) \Pi_2) \\
        &= \tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1 \Pi_2) + \tr(\Pi_2 \Pi_1^\perp \Sigma_2 \Pi_1^\perp \Pi_2) + 2\tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1^\perp \Pi_2).
    \end{align*}
    Since $\Sigma_2$ is the PSD matrix, it has a square root $\Sigma_2^{1/2}$. By Cauchy-Schwarz inequality, we have
    \begin{align*}
        2\tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1^\perp \Pi_2) & = 2\langle \Pi_2 \Pi_1 \Sigma_2^{1/2},  \Pi_2 \Pi_1^\perp \Sigma_2^{1/2} \rangle \\
        & \leq 2\langle \Pi_2 \Pi_1 \Sigma_2^{1/2},  \Pi_2 \Pi_1 \Sigma_2^{1/2} \rangle^{1/2} \cdot \langle \Pi_2 \Pi_1^\perp \Sigma_2^{1/2},  \Pi_2 \Pi_1^\perp \Sigma_2^{1/2} \rangle^{1/2} \\
        &\leq \langle \Pi_2 \Pi_1 \Sigma_2^{1/2},  \Pi_2 \Pi_1 \Sigma_2^{1/2} \rangle + \langle \Pi_2 \Pi_1^\perp \Sigma_2^{1/2},  \Pi_2 \Pi_1^\perp \Sigma_2^{1/2} \rangle \\
        & = \tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1 \Pi_2) + \tr(\Pi_2 \Pi_1^\perp \Sigma_2 \Pi_1^\perp \Pi_2).
    \end{align*}
    Thus, we have 
    \begin{align}\label{eq:trace}
        \tr(\Pi_2 \Sigma_2 \Pi_2) \leq 2\tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1 \Pi_2) + 2\tr(\Pi_2 \Pi_1^\perp \Sigma_2 \Pi_1^\perp \Pi_2).
    \end{align}

    For the first term in the right-hand side of~(\ref{eq:trace}), by the Holder's inequality for matrix, 
    we have 
    \begin{align*}
        \tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1 \Pi_2) = \tr(\Pi_2 \Pi_1 \Sigma_2 \Pi_1) \leq \|\Pi_2\|_2\cdot \tr(\Pi_1 \Sigma_2 \Pi_1) \leq \tr(\Pi_1 \Sigma_2 \Pi_1).
    \end{align*} 

    For the second term in the right-hand side of~(\ref{eq:trace}), since $\Sigma_2 \preceq c\Sigma_1$, we have 
    \begin{align*}
        \tr(\Pi_2 \Pi_1^\perp \Sigma_2 \Pi_1^\perp \Pi_2) \leq c \cdot \tr(\Pi_2 \Pi_1^\perp \Sigma_1 \Pi_1^\perp \Pi_2) = c \cdot \tr(\Pi_2 \Pi_1^\perp \Sigma_1 \Pi_1^\perp).
    \end{align*}
    By the Holder's inequality for matrix, we have 
    \begin{align*}
        \tr(\Pi_2 \Pi_1^\perp \Sigma_1 \Pi_1^\perp) = \langle \Pi_1^\perp \Sigma_1 \Pi_1^\perp, \Pi_2 \rangle \leq \|\Pi_1^\perp \Sigma_1 \Pi_1^\perp\|_2 \cdot \tr(\Pi_2).
    \end{align*}
    Since $\Pi_2$ is a projection matrix, we have $\tr(\Pi_2) = \rank(\Pi_2)$.
\end{proof}



The following claim uses the concavity of the log-function to argue about the shrinking of volume when we move to an ellipsoid with more skewed axes. %to have, though may not be needed. 
\begin{claim}\label{claim:concavity}
For any ellipsoid $E_M=\{x: x^\top M x \le 1\}$ where $M$ has positive eigenvalues $a_1^2, \dots, a_d^2$ with $a_1^2+\dots+a_d^2 \le d$, it holds
\begin{equation}
\frac{\vol(E_M)}{\vol(\Ball(0,1))} \le \exp\Big(-\frac{1}{4} \sum_{i=1}^d \max\{a_i^2 - 2,0 \}\Big).
\end{equation}
The term $\sum_{i=1}^d \max\{a_i^2 - 2,0 \}$ captures the mass on the eigenvalues much larger than $1$. 
\end{claim}

\begin{proof}
By the definition of the ellipsoid volume, we have    
\begin{align*}
2\ln\Big(\frac{\vol(E_M)}{\vol(\Ball(0,1))}\Big) & = \ln( a^2_1 a^2_2 \cdots a^2_d) = \sum_{i=1}^d \ln(a_i^2). 
\end{align*}
We now show that 
\begin{align*}
    \sum_{i=1}^d \ln(a_i^2) \leq -\frac{1}{2}\sum_{i=1}^d \max\{a_i^2- 2,0\}.  
\end{align*}
We define the function $f(x) = \ln(x) + \frac{1}{2}\max\{x-2,0\}$. We also define a piecewise function
$$
g(x) =
\begin{cases} 
\ln(x) & \text{if } 0 < x < 1, \\
x - 1 & \text{if } x \geq 1.
\end{cases}
$$
We have $f(x) = g(x) = \ln(x)$ for $0<x < 1$. We have the derivative $f'(x) = 1/x$ for $1\leq x < 2$ and $f'(x) = 1/x + 1/2$ for $x \geq 2$. Since the function $f$ is continuous on $(0,\infty)$, we have $f'(x) \leq 1$ for $x \geq 1$ and $g'(x) = 1$ for $x \geq 1$. Thus, we have $f(x) \leq g(x)$ for every $x > 0$. It is easy to see that $g$ is monotone increasing and concave on $(0,+\infty)$. By Jensen's inequality, we have for any $a_1,\cdots,a_d > 0$ with $a_1^2+\cdots+a_d^2 \leq d$.
\begin{align*}
    \frac{1}{d}\cdot \sum_{i=1}^d g(a_i^2) \leq g\left(\frac{1}{d}\sum_{i=1}^d a_i^2\right) \leq g(1) = 0.
\end{align*}
Since $f(x) \leq g(x)$ for every $x > 0$, we have $\sum_{i=1}^d f(a_i^2) \leq 0$. Thus, we have 
\begin{align*}
    \ln\Big(\frac{\vol(E_M)}{\vol(\Ball(0,1))}\Big) \leq \frac{1}{2} \sum_{i=1}^d \ln(a_i^2) \leq -\frac{1}{4}\sum_{i=1}^d \max\{a_i^2-2,0\},
\end{align*}
which completes the proof.
\end{proof}

%\anote{It's not crucial right now, but can someone see if they can find a proof of this claim? Intuitively this seems correct... in the $2\log\vol$ computation, the large eigenvalues which each contribute a $\log$ term have to be compensated by eigenvalues smaller than $1$ and since $\log(1-x) \approx x$ this accumulates linearly. It should help and may make proofs simpler. It could simplify the definition of good ellipsoid etc.}

The following is a robust version of the above claim.

\begin{claim}\label{claim:robust_concavity}
For $d\geq 2$, $b_1, \dots, b_d >0$ with $b_1^2+\dots+b_d^2 \leq d$ and $\beta_4 \geq 4\ln d$, consider the ellipsoid $E_M=\{x: x^\top M x \le 1\}$ where $M$ has positive eigenvalues $a_1^2, \dots, a_d^2$ with $a_i = b_i$ for $b_i < \beta_4$ and $a_i = d\cdot b_i$ for $b_i \geq \beta_4$. Then, it holds that
\begin{equation}
\frac{\vol(E_M)}{\vol(\Ball(0,1))} \le \exp\Big(-\frac{1}{4} \sum_{i=1}^d \max\{b_i^2 - 2,0 \}\Big).
\end{equation}
The term $\sum_{i=1}^d \max\{b_i^2 - 2,0 \}$ captures the mass on the eigenvalues much larger than $1$. 
\end{claim}

\begin{proof}
Define a piecewise function 
$$
f(x) =
\begin{cases} 
\ln(x) + \frac{1}{2} \max\{x-2,0\} & \text{if } 0 < x < \beta_4, \\
\ln(d x) + \frac{1}{2} (x-2) & \text{if } x \geq \beta_4.
\end{cases}
$$
We also define a piecewise function 
$$
g(x) =
\begin{cases} 
\ln(x) & \text{if } 0 < x < 1, \\
x - 1 & \text{if } x \geq 1.
\end{cases}
$$
It is easy to see that $f(x)$ is continuous on $(0,\beta_4)$ and $(\beta_4, \infty)$. The function $f$ is discontinuous at $x = \beta_4$ with a jump of value $\ln(d)$.

We have $f(x) = g(x) = \ln(x)$ for $0<x < 1$. We have the derivative $f'(x) = 1/x$ for $1\leq x < 2$ and $f'(x) = 1/x + 1/2$ for $x \in (2,\beta_4) \cup (\beta_4,\infty)$. Thus, we have $f'(x) \leq 1 =g'(x)$ for $x \in (2,\beta_4) \cup (\beta_4,\infty)$.
For $x = \beta_4$, since $\beta_4 \geq 4\ln d$ and $d \geq 2$, we have 
$$
f(\beta_4) = \ln(\beta_4 d) + \frac{\beta_4-2}{2} \leq \ln(d\beta_4) + \frac{\beta_4-2}{2} \leq \beta_4-1 = g(\beta_4). 
$$
Therefore, we have $f(x) \leq g(x)$ for every $x > 0$. It is easy to see that $g$ is monotone increasing and concave on $(0,+\infty)$. By Jensen's inequality, we have for any $b_1,\cdots,b_d > 0$ with $b_1^2+\cdots+b_d^2 \leq d$.
\begin{align*}
    \frac{1}{d}\cdot \sum_{i=1}^d g(b_i^2) \leq g\left(\frac{1}{d}\sum_{i=1}^d b_i^2\right) \leq g(1) = 0.
\end{align*}
Since $f(x) \leq g(x)$ for every $x > 0$, we have $\sum_{i=1}^d f(b_i^2) \leq 0$. Thus, we have 
\begin{align*}
    \ln\Big(\frac{\vol(E_M)}{\vol(\Ball(0,1))}\Big) \leq \frac{1}{2} \sum_{i=1}^d \ln(a_i^2) \leq -\frac{1}{4}\sum_{i=1}^d \max\{b_i^2-2,0\},
\end{align*}
which completes the proof.
\end{proof}

%\lnote{I will prove the robust version soon. I think the constants above should work.}
%\anote{Liren, see my note above in Proof of Lemma 5.2 about the version needed.}


\subsection{Algorithm to find Good Ellipsoids}

\begin{lemma}\label{lem:find:goodep}
Given a ball $B'=Ball(c',R')$, let  $Y' \subset \R^d$ be all points within ball $B'$. Suppose there is an unknown ball $B^* = Ball(c^*,R^*)$ contained in $B'$ with $R' \leq 2R^*$ such that $Y = Y' \cap B^*$ contains $|Y| \geq \delta_1 |Y'|$ points and a subset of points $Y^* \subseteq Y$ contains $|Y^*| \geq \delta_2 |Y|$ points and one of the following properties holds
\begin{enumerate}
    \item $\lambda_{\max}(\Sigma^*) \le (\tau^*)^2$;
    \item there exists $\Yin \subseteq Y^*$ of size $|\Yin| \geq (1-\delta_3) |Y^*|$ \vnote{it would be nice to name this \(\delta_3\) since \(\delta\) already means the fraction of points in the optimal ball.} such that for any $y \in \Yin$,
    $$
    \norm{\Proj^{>\tau^*}_{*} y}_2^2 \ge \eta \cdot \EV_{\tau^*}(Y^*).
    $$
\end{enumerate}
where $\Sigma^*$ is the covariance of $Y^*$ and $\Proj^{>\tau^*}_{*}$ is the projection operator onto the eigenspace of $\Sigma^*$ with eigenvalues  greater than $\tau^*$.

Then, Algorithm \textsc{Good\_Ellipsoid} finds a list of $\ell=\poly(d)$ ellipsoidal shapes $M_1, \dots, M_\ell$ such that there exists $M \in \{M_1, \dots, M_\ell\}$ for which the shifted ellipsoid $E_M=\{x: (x-c)^\top M (x-c) \le (R^*)^2\}$ is a good ellipsoid for $B^*,Y^*$. \vnote{parameters missing here.  Assuming this is a \((\tau^\star, \beta)\)-good ellipsoid in the theorem proof, any changes should be ported there as well.}

\vnote{Where is the dependence on \(\beta'\) here?  Are we assuming it's a constant?}\lnote{I think it should be poly(log d). In Lemma 4.3, delta = loglog d/log d. here, 1/beta' = delta/2 or delta/O(log d).}

%(unknown) $B=Ball(0,R)$ with $R' \le 2R$ \anote{radius bound not needed for this part?}, and $|X \cap B| \ge (1-\alpha) |X \cap B'|$. Then in polynomial time, we can find a $\ell=\poly(d)$ sized list of ellipsoidal shapes $M_1, \dots, M_\ell$ such that there exists $M \in \{M_1, \dots, M_\ell\}$, a (unknown)  $c \in \R^d$ and (unknown) $Y \subset X \cap B$ with $|Y| \ge (1-\gamma) |X \cap B|$,  such that the appropriately shifted ellipsoid $E_M=\{x: (x-c)^\top M (x-c) \le R^2\}$ is a good ellipsoid for $B,Y$.   \anote{I assume implicit scaling by $R$, which we can guess of course.}
\end{lemma}

\input{Algorithm/alg_good_ellipsoid}

\input{Algorithm/alg_filter_procedure}
%\anote{The above is a claim that I'm hoping we can show. }

%\anote{I think the lemma holds. Writing down algorithm and proof sketch below.}

%\paragraph{Algorithm for finding a good ellipsoid $M$}
%\anote{We need to put this in an algorithm environment}

% \begin{figure}[htbp]
% \begin{tcolorbox}
% \begin{center}
%     \textbf{Algorithm} $\textsc{Good\_Ellipsoid}$ \textbf{for finding a good ellipsoid}
% \end{center}
% \begin{enumerate}
%     \item Guess a target $V^*$ which is within a $(\tfrac{2}{1-\alpha})$-factor of $\EV_\tau(X \cap B^*)d/(R^*)^2$, which is the total variance along the high variance directions of the optimal solution. Also, guess $s^* = |\{i: \lambda_i(\Sigma_{X \cap B^*}) \ge \tau\}|$. 
%     \item Set parameter $\tau_1=\beta \tau$, where $\beta = d^{o(1)}$. Set $\sigma_{ub}^2 = 2V^*$. \anote{We can also guess this, but a weak bound of $V^*$ is enough. }
%     \item Run the filtering algorithm of~\cite{diakonikolas2016robust} and~\cite{lai2016agnostic} with $\sigma = \sigma_{ub}$ to get a set $\whX \subset X \cap B'$ of size $(1-O(\alpha))|X \cap B'|$ with variance at most $O(\sigma_{ub}^2)$ in every direction, and let $\whmu$ be its mean; let $n_0 := |\whX|$ and 
%     \begin{equation} \label{eq:sigmaupdate}
%     \whSigma = \frac{1}{n_0} \sum_{x \in \whX} (x-\whmu)(x-\whmu)^\top.  
%     \end{equation}
%     \anote{For $\delta$ fraction instead of $1-\alpha$ fraction, we can replace the above with a List-Decodable mean estimation algorithm with variance bound $V^*$. Does the list-decodable mean estimation algorithm also output a subset $\whX_j$ of size $\Omega(\delta)$ for which it is the empirical mean? }
%     The remaining algorithm is run on $\whX$. The set $\whX$ and its mean $\whmu$ are updated using the following iterative algorithm in the natural way; but $\whSigma$ is always updated as a sum of squared deviations over the samples in the current $\whX$ divided by (the original) $n_0$. As we will see later, $|\whX| \ge (1-O(\alpha))n_0$ for the whole algorithm.    
%     \item Run the following algorithm iteratively: (until the number of high variance directions is more than $\beta'' V^*$ for some appropriate $\beta''=d^{o(1)}$) \anote{condition is meant as a comment}
%     \begin{enumerate}
%         \item Compute the eigenvectors $\whv_1, \dots, \whv_d$ of $\whSigma$ and let $\whlambda_1^2, \dots, \whlambda_d^2$ be its corresponding eigenvalues. Let $\whBig=\{i \in [d]: \whlambda_i \ge \tau_1 \}$, and let $\whProj_{hi}$ be the projection onto the subspace spanned by those eigenvectors corresponding to eigenvalues $\whlambda_i$ for $i \in \whBig$.
%         \item If $|\whBig| \le \beta'' V^*$, then set $M=\sum_{i=1}^d a_i^2 \whv_i \whv_i^\top$, where $a_i = \beta_4 d$ if $\whlambda_i \ge \tau_1$ and $a_i = 1-\gamma$ otherwise, where $\gamma=\EV_{\tau_1}(\whX)/d$ and $\beta_4$ is as given as in Definition~\ref{def:goodep}; return $M$ and complete the algorithm.  
%         \item Remove from $\widehat{X}$ all the $x$ such that 
%         \[\norm{\whProj_{hi}(x-\whmu)}_2^2 > \beta' V^* + \tau^2 \beta |\whBig| \]
%          Also set as in \eqref{eq:sigmaupdate} \[\whmu = \frac{1}{|\whX|} \sum_{x \in \whX} x, \text{ and } \whSigma=  \frac{1}{n_0} \sum_{x \in \whX} (x-\whmu)(x-\whmu)^\top,   \]
%          and start the next iteration with the updated $\whX, \whmu, \whSigma$.
%     \end{enumerate}
% \end{enumerate}
% \end{tcolorbox}
% \caption{Algorithm $\textsc{Good\_Ellipsoid}$ for finding a good ellipsoid}
% \label{fig:algo_ellipsoid}
% \end{figure}

By Lemma~\ref{lem:covering-good-ellipsoids}, there exists a subset $Y^* \subseteq Y$ of size $|Y^*| \ge \frac{1}{\log^{1/\varepsilon} d}\cdot |Y|$ such that one of the following properties holds
\begin{enumerate}
    \item $\lambda_{\max}(\Sigma^*) \le (\tau^*)^2$;
    \item there exists $\Yin \subseteq Y^*$ of size $|\Yin| \geq (1-\delta) |Y^*|$ such that for any $y \in \Yin$,
    $$
    \norm{\Proj^{>\tau^*}_{*} y}_2^2 \ge \eta \cdot \EV_{\tau^*}(Y^*).
    $$
\end{enumerate}
where $\Sigma^*$ is the covariance of $Y^*$ and $\Proj^{>\tau^*}_{*}$ is the projection operator onto the eigenspace of $\Sigma^*$ with eigenvalues  greater than $\tau^*$.
Then, we consider $Y^* \subseteq Y'$ as the inliers at Step 3 of Algorithm~\textsc{Good\_Ellipsoid}. In Step 3, we run the list-decodable mean estimation algorithm by~\cite{diakonikolas2020list}. We use the following theorem.

\begin{theorem}[\cite{diakonikolas2020list}]\label{thm:list_decodable}
    Let $Y'$ be a set of $n$ points in $\R^d$. Let $Y^* \subseteq Y'$ be an unknown subset of points with $|Y^*| \geq \delta|Y'|$ for $\delta \in (0,1)$ and unknown bounded variance $\Sigma_{Y^*} \preceq \sigma^2 I$. There is an algorithm that, on input $Y'$ and $\delta$, runs in $\tilde O(n^2d/\delta^2)$ time and outputs a list of $O(1/\delta)$ subsets $Y_i \subseteq Y'$ such that with high probability, at least one of these subsets $Y_i$ satisfies  
    \begin{enumerate}
        \item $\|\mu(Y_i) - \mu(Y^*)\|_2 \leq O(\sigma \log(1/\delta)/\sqrt{\delta})$;
        \item $|Y_i| \geq \delta |Y'|/2$;
        \item $|Y_i \cap Y^*| \geq |Y^*|/2$. 
    \end{enumerate}
\end{theorem}

In Step 4, Algorithm~\textsc{Good\_Ellipsoid} runs the Procedure~\textsc{Iterative\_Filter} on each subset $Y_i$ in the list returned by the list-decodable mean estimation algorithm in Step 3. In the following analysis, we consider the call of Procedure~\textsc{Iterative\_Filter} on the subset $Y_i$ that satisfies the properties in Theorem~\ref{thm:list_decodable}. Let $\whY_0 = Y_i$ be the initial set of points in this call of Procedure~\textsc{Iterative\_Filter}. 

Note that across each iteration of the algorithm, the matrix $\whSigma_{t+1}$ is PSD-dominated (according to the Loewner ordering) by the corresponding matrix $\whSigma_t$ in the previous iteration (since it is just a sum of PSD matrices, one for each point $x \in \whY_t$ and the algorithm only remove points from $\whY_t$). Hence there are no new elements added to $\whBig_t$ across iterations (some elements may get removed).  
%Let $\mu^*$ be the mean of $Y^*$. 
%After Step 3 of the above algorithm, we have that $\norm{\whSigma} \le O(\sigma_{ub}^2) \le  O(V^*)$. Since both $\whX$ and $X\cap B^*$ contains at least $1-O(\alpha)$ fraction of $X\cap B'$ and has variance at most $O(\sigma_{ub}^2)$ in every direction, we have $\norm{\whmu-\mu^*}_2 \le O(\sigma_{ub}) = O(\sqrt{V^*})$.   
We now prove the following two claims about each iteration (Steps 2(a)-2(c)) of the Procedure \textsc{Iterative\_Filter}. 
%\anote{Maybe in what follows $\EV_\tau$ etc. also has to be redefined in terms of $\whSigma$ i.e., using \eqref{eq:sigmaupdate} which normalizes with the original $n_0$.}

\begin{claim}[Most points from $Y^*$ remain in $\whY_t$]\label{claim:inlier_remain} 
Consider any iteration $t$ of Algorithm~\textsc{Good\_Ellipsoid} with $|\whY_t \cap Y^*| \geq |Y^*|/4$. Then, at least $(1-4/\beta)$ fraction of the points in $\whY_t \cap Y^*$ survive after Step 2(c) in each iteration.   
\end{claim}

\begin{proof}
Let $\whY_t$ be the set of points at the beginning of iteration $t+1$ of Algorithm \textsc{Good\_Ellipsoid}.
Consider any iteration $t+1$ with $|\whY_t \cap Y^*| \geq |Y^*|/4$.


We consider the set $\whY_0 = Y_i$ is a good candidate subset returned by the list-decodable mean estimation.  Thus, we have $\|\whSigma_0\| \leq O(\log(1/\delta)\sigma^2)$.
Since $|\whY_t| \geq |\whY_t \cap Y^*| \geq n_0/2$ and $\whY_t \subseteq \whY_0$, the variance of $\whY_t$ in every direction is also bounded by $O(\log(1/\delta)\sigma^2)$. Similarly, we have the variance of $\whY_t \cap Y^*$ in every direction is bounded by $O(\log(1/\delta)\sigma^2)$. 
Thus, we have $\norm{\mu^* - \whmu_t}_2$ and $\norm{\mu^* - \mu(\whY_t \cap Y^*)}_2$ are both upper bounded by $O(\sigma \log(1/\delta)/\sqrt{\delta})$. %$O(\sigma_{ub}^2) = O(V^*)$.

%Thus, we have $\norm{\mu^* - \whmu_t}_2$ and $\norm{\mu^* - \mu(\whY_t \cap Y^*)}_2$ are both upper bounded by $O(\sigma \log(1/\delta)/\sqrt{\delta})$. 

%First, we show that since $|\whY_t \cap Y^*| \ge \delta |\whY_t|$ we have that all the high eigenvalue (variance) directions of $\whSigma$ restricted to $(\whX \cap B^*)$ remain directions of high variance corresponding to $\whSigma$ \anote{need to modify this for $\delta$ fraction}.

By the covariance decomposition, we have 
\begin{align*}
    \sum_{x \in \whY_t \cap Y^*}(x-\whmu_t)(x-\whmu_t)^\top =& \sum_{x \in \whY_t \cap Y^*}\big(x-\mu(\whY_t \cap Y^*)\big)\big(x-\mu(\whY_t \cap Y^*)\big)^\top \\
    &+ |\whY_t \cap Y^*| \big(\mu(\whY_t \cap Y^*) - \whmu_t\big)\big(\mu(\whY_t \cap Y^*) - \whmu_t\big)^\top\\
    \preceq& \sum_{x \in \whY_t \cap Y^*}(x-\mu^*)(x-\mu^*)^\top + Q,
\end{align*}
where  $Q=|\whY_t \cap Y^*|\Big(\big(\mu(\whY_t \cap Y^*) - \mu^*\big)^{\otimes 2}+ \big(\mu(\whY_t \cap Y^*) - \whmu_t\big)^{\otimes 2}\Big)$
is a rank-one matrix.
Since $\norm{\mu^* - \whmu_t}_2 , \norm{\mu^* - \mu(\whY_t \cap Y^*)}_2 = O(\sigma \log(1/\delta)/\sqrt{\delta}) = O(\log(1/\delta) \sqrt{V^*})$, we have $\tr(Q)= O(\log^2(1/\delta) n_0 V^*)$. 
Let $$\Sigma_t' = \frac{1}{|\whY_t \cap Y^*|}\sum_{x \in \whY_t \cap Y^*}(x-\mu^*)(x-\mu^*)^\top.$$
Thus, we have
\begin{align}\label{eq:expected_high_variance_length}
    \frac{1}{|\whY_t \cap Y^*|}\sum_{x \in \whY_t \cap Y^*} \norm{ \Projj{t}{\tau_t} (x -\whmu_t)}_2^2 &= \tr(\Projj{t}{\tau_t} \Sigma_{\whY_t \cap Y^*} \Projj{t}{\tau_t}) \nonumber\\
    &\leq \frac{1}{|\whY_t \cap Y^*|}\tr(\Projj{t}{\tau_t} Q \Projj{t}{\tau_t}) + \tr(\Projj{t}{\tau_t} \Sigma_t' \Projj{t}{\tau_t})\nonumber\\
    &\leq \frac{1}{|\whY_t \cap Y^*|}\tr(Q) + \frac{1}{|\whY_t \cap Y^*|}\sum_{x \in \whY_t \cap Y^*} \norm{ \Projj{t}{\tau_t} (x -\mu^*)}_2^2.
\end{align}

Let $\Sigma^*$ be the true covariance of $Y^*$ with eigenvalues $\lambda_1^2, \dots, \lambda_d^2$, and corresponding eigenvectors $u_1, \dots, u_d$.  Then, we have 
\begin{align*}
\sum_{x \in \whY_t \cap Y^*} (x-\mu^*)(x-\mu^*)^\top &\preceq \sum_{x \in Y^*} (x-\mu^*)(x-\mu^*)^\top = |Y^*| \cdot \Sigma^*.
\end{align*}

We now bound the total variance of points in $Y^*$ on the high-variance directions of $\whSigma_t$. We have
\begin{align}\label{eq:total_high_variance_Y*}
\frac{1}{|Y^*|}\sum_{x \in Y^*}\norm{\Projj{t}{\tau_t}(x -\mu^*)}^2_2 & = \tr\left(\Projj{t}{\tau_t}  \Sigma^* \Projj{t}{\tau_t}\right) = \sum_{i=1}^d \lambda_i^2 \norm{\Projj{t}{\tau_t} u_i}_2^2  \nonumber\\
&\le  \sum_{i: \lambda_i^2 \ge \tau_t^2} \lambda_i^2 \norm{\Projj{t}{\tau_t} u_i}_2^2 + \tau_t^2 \sum_{i=1}^d \norm{\Projj{t}{\tau_t} u_i}_2^2 \nonumber\\
&\le \sum_{i: \lambda_i^2 \ge \tau_t^2} \lambda_i^2 + \tau_t^2  \tr\left(\Projj{t}{\tau_t} \left(\sum_{i=1}^d u_i u_i^{\top}\right) \Projj{t}{\tau_t} \right) \nonumber\\
&= \EV_{\tau_t}(Y^*) + \tau_t^2 \tr\left(\Projj{t}{\tau_t}\right) \leq \delta \cdot V^* + \tau_t^2 |\whBig_t|.
\end{align}
Hence, we also have
$$
\sum_{x \in \whY_t \cap Y^*}\norm{\Projj{t}{\tau_t} (x -\mu^*)}^2_2 \leq \sum_{x \in Y^*}\norm{\Projj{t}{\tau_t} (x -\mu^*)}^2_2 \leq |Y^*| \left(\delta\cdot V^* + \tau_t^2 |\whBig_t|\right). 
$$

By combining the Equation~(\ref{eq:expected_high_variance_length}) and ~(\ref{eq:total_high_variance_Y*}), we have
\begin{align*}
    \frac{1}{|\whY_t \cap Y^*|}\sum_{x \in \whY_t \cap Y^*} \norm{ \Projj{t}{\tau_t} (x -\whmu_t)}_2^2  &\le \frac{1}{|\whY_t \cap Y^*|}\tr(Q) +  \frac{1}{|\whY_t \cap Y^*|}   \sum_{x \in \whY_t \cap Y^*}\norm{\Projj{t}{\tau_t}(x -\mu^*)}^2_2  \\ 
    &\le O(V^*)+ \frac{|Y^*|}{|\whY_t \cap Y^*|} \cdot \left( \delta \cdot V^* + \tau_t^2 |\whBig_t| \right) \\
    &\le 4 \cdot \Big( O(V^*)+  \tau_t^2 |\whBig_t|\Big),
\end{align*}
where the last inequality is from $|\whY_t \cap Y^*| \geq |Y^*|/4$.
By Markov's inequality, for at least $(1-4/\beta)$-fraction of points $x \in \whY_t \cap Y^*$, we have $\norm{ \Projj{t}{\tau_t} (x -\whmu_t)}_2^2$ is upper bounded by $\beta' V^* + \beta\tau_t^2 |\whBig_t|$. 
%\anote{Also need to argue the last sentence in the claim is maintained, maybe by induction... but should be fine since we only plan to do $\tilde{O}(1)$ iterations.} 
\end{proof}
% Moreover note that along any direction $u$, $u^\top \whSigma u$ is non-decreasing across iterations (since it is just a sum over $\whX$ and each point contributes a psd term to $\whSigma$).

\begin{claim}[Excess variance of $\whSigma$ decreases quickly] \label{claim:outlierdecrease}
If $|\whBig_t| \ge \beta'' V^*/\tau_t^2$, then after iteration $t$, the normalized excess variance $\widehat\EV_{\tau_t}(\whY_t)$ decreases by a factor of $\eta'< 1/\beta''$. %where $\beta_1, \beta''$ depend on $\beta$ appropriately and are at most $d^{o(1)}$. 
\end{claim}

\begin{proof}
%\anote{We need to set the different $\beta$s and $\tau$s correctly for this proof to work. }
Since $|\whBig_t| > \beta'' V^*/ \tau_t^2$, we have %$\EV_{\tau_1/2}(\whSigma) \ge \tau_1^2 |\whBig|/4  > 2 \beta'' V^*$; hence 
$$\EV_{\tau_t}(\whY_t) \ge \tau_t^2 |\whBig_t|  \geq \beta'' V^*.$$
%(We will set $\beta_1$ later appropriately)

We now show that after iteration $t$, the excess variance $\EV_{\tau_{t}}(\whY_t)$ decreases by a factor of $\eta'$. Let $\Projj{t}{\tau_t}$ be the projection onto the eigenspace of the covariance $\whSigma_t$ with eigenvalues greater than $\tau_t$. Then, we have
\begin{align*}
    \EV_{\tau_{t+1}}(\whY_{t+1}) = \tr\left(\Projj{t+1}{\tau_{t+1}} \Sigma_{\whY_{t+1}} \Projj{t+1}{\tau_{t+1}} \right).
\end{align*}
%By Claim~\ref{claim:inlier_remain}, we have $|\whY_{t+1} \cap Y^*| \geq (1-4/\beta)|\whY_t \cap Y^*|$ for each iteraion $t$, which implies that $\whSigma_{t+1} \preceq \frac{1}{1-1/\beta}\whSigma_t$. 
Since we define $\whSigma_t = \frac{1}{n_0} \sum_{y \in \whY_t} (y - \whmu_t)(y-\whmu_t)^\top$, we have
\begin{align*}
    \whSigma_{t+1} = \frac{1}{n_0} \sum_{y \in \whY_{t+1}} (y - \whmu_{t+1})(y-\whmu_{t+1})^\top \preceq \frac{1}{n_0} \sum_{y \in \whY_{t+1}} (y - \whmu_t)(y-\whmu_t)^\top \preceq \frac{1}{n_0} \sum_{y \in \whY_{t}} (y - \whmu_t)(y-\whmu_t)^\top = \whSigma_{t}.
\end{align*}
By Claim~\ref{claim:trace_decompose} with $\Sigma_1 = \Sigma_{\whY_{t}}$, $\Sigma_2 = \Sigma_{\whY_{t+1}}$, $\Pi_1 = \Projj{t}{\tau_{t}}$ and $\Pi_2 = \Projj{t+1}{\tau_{t+1}}$, we have
\begin{align*}
    &\EV_{\tau_{t+1}}(\whY_{t+1}) = \tr\left(\Projj{t+1}{\tau_{t+1}} \Sigma_{\whY_{t+1}} \Projj{t+1}{\tau_{t+1}} \right) \\
    &\leq 2\tr\left(\Projj{t}{\tau_{t}} \Sigma_{\whY_{t+1}} \Projj{t}{\tau_{t}}  \right) +  2 \cdot \|\Projjperp{t}{\tau_{t}}\Sigma_{\whY_t}\Projjperp{t}{\tau_{t}}\|_2\cdot \rank\left(\Projj{t+1}{\tau_{t+1}}\right).
\end{align*}
According to the Procedure~\textsc{Iterative\_Filter}, for any point $x$ remaining in $\whY_{t+1}$, we have 
$$
\norm{\Projj{t}{\tau_t}(x - \whmu_t)}_2^2 \leq \beta' V^* + \tau_t^2 \beta |\whBig_t|.
$$
Thus, we have 
\begin{align*}
    \tr\left(\Projj{t}{\tau_{t}} \whSigma_{t+1} \Projj{t}{\tau_{t}}  \right) &= \frac{1}{n_0} \sum_{x \in \whY_{t+1}} \norm{\Projj{t}{\tau_t}(x - \whmu_t)}_2^2 \\
    &\leq \frac{|\whY_{t+1}|}{n_0} \cdot \left(\beta' V^* + \tau_t^2 \beta |\whBig_t| \right) \leq \frac{1}{\widehat\beta} \cdot \left(\beta' V^* + \tau_t^2 \beta |\whBig_t| \right),
\end{align*}
where the last inequality is due to $|\whY_{t+1}| \leq |\whY_0|$ and $n_0 = \widehat\beta |\whY_0|$.

Note that $\|\Projjperp{t}{\tau_{t}}\Sigma_{\whY_t}\Projjperp{t}{\tau_{t}}\|_2 \leq \tau_t^2$. Since $\tau_{t}^2 \leq \tau_{t+1}^2/4$, we have 
\begin{align*}
    \|\Projjperp{t}{\tau_{t}}\Sigma_{\whY_t}\Projjperp{t}{\tau_{t}}\|_2\cdot \rank\left(\Projj{t+1}{\tau_{t+1}}\right) &\leq \tau_t^2 \cdot \rank\left(\Projj{t+1}{\tau_{t+1}}\right) \\
    &\leq \frac{\tau_{t+1}^2}{4} \cdot \rank\left(\Projj{t+1}{\tau_{t+1}}\right) \leq \frac{\EV_{\tau_{t+1}}(\whY_{t+1})}{4}.
\end{align*}
Therefore, by combining the two terms, we have
\begin{align*}
    \EV_{\tau_{t+1}}(\whY_{t+1}) \leq \frac{4}{\widehat \beta} \cdot \left(\beta' V^* + \tau_t^2 \beta |\whBig_t| \right) \leq \frac{1}{\beta''} \EV_{\tau_{t}}(\whY_{t}).
\end{align*}

%%%%%%%%%%%%%%%%%%%%

% Hence, it suffices to show that $\sum_{x \in \whX} \norm{ \whProj_{hi} (x -\whmu)}_2^2$ drops by a factor of $1/\beta_1$.

% Let $X'$ be the set of points that remain, let $\mu'$ be the mean of points in $X'$. Also let $\Proj'_{hi}$ be the updated $\whProj_{hi}$ in the next iteration; we have $\Proj'_{hi} \preceq \whProj_{hi}$. We have by removal rule, 
% \begin{align*}
% n_0 \EV_{\tau_1}(X')&\le  \sum_{x \in X'} \norm{ \Proj'_{hi} (x -\mu')}_2^2 \le \sum_{x \in X'} \norm{ \Proj'_{hi} (x -\whmu)}_2^2\\
% &\le \sum_{x \in X'} \norm{ \whProj_{hi} (x -\whmu)}_2^2 \le |X'|(\beta' V^* + \tau^2 \beta |\whBig|) \\
% &\le |X'| \frac{1}{\beta''}\EV_{\tau_1/2}(\whSigma)\le \frac{|X'|}{\beta''} \EV_{\tau_1}(X'). \\
% \text{Hence } \EV_{\tau_1}(X')&\le \frac{1}{\beta''} \EV_{\tau_1}(X'),
% \end{align*}
% which concludes the proof. 
\end{proof}

Now, we prove Lemma~\ref{lem:find:goodep} by combining Claim~\ref{claim:inlier_remain} and Claim~\ref{claim:outlierdecrease}.

\begin{proof}[Proof of Lemma~\ref{lem:find:goodep}]
    Let $M^*$ be the ellipsoidal shape returned by Algorithm \textsc{Good\_Ellipsoid} with the correct guess of $V^*$ and on the subset $\whY_0 = Y_i$ satisfies the conditions in Lemma~\ref{lem:find:goodep}. We now show that the appropriately shifted ellipsoid $E_{M^*} = \{x: (x-c)^\top M^* (x-c) \leq R^*\}$ is a good ellipsoid for $B^*$ and $Y^*$.

    %Since the remaining points $\whX$ are contained in $B' = Ball(c',R')$ with $R' \leq 2R^*$, we have the excess variance $\EV_{\tau}(\whX) \leq R^2$. 
    By Claim~\ref{claim:outlierdecrease}, the normalized excess variance of $\whY_t$ goes down by a $1/\beta'' = 1/\log^{\Omega(1)} d$ factor in each iteration. 
    Note that the normalized excess variance $\widehat\EV_{\tau_t}(\whY_t)$ is at most $d$.
    Suppose $\EV_{\tau^*}(Y^*) > 0$, then $\EV_{\tau^*}(Y^*) \geq (\tau^*)^2 \geq 2$.
    Since $\widehat\EV_{\tau_t}(\whY_t) \geq 4\beta''\beta' V^* \geq 4\beta''\beta' \EV_{\tau^*}(Y^*)/\delta \geq 1/\poly\log(d)$, then after $O(\log d)$ iterations, we have $\widehat\EV_{\tau_t}(\whY_t) \leq 4\beta''\beta' V^*$, which implies $|\whBig_t| < \beta'' V^*$ and the Procedure~\textsc{Iterative\_Filter} stops.
    By Claim~\ref{claim:inlier_remain}, if $|\whY_t \cap Y^*| \geq |Y^*|/4$, then at least $1-4/\beta$ fraction of points in $\whY_t \cap Y^*$ survives in iteration $t$ for $\beta = \omega(\log d)$.
    Thus, after at most $O(\log d)$ iterations, we have $|\whY_t \cap Y^*| \geq |Y^*|/4$. 
    Let $\widehat\beta = \poly\log(d)$.
    
    By the construction of the ellipsoidal shape $M^*$, it is easy to see that $E_{M^*}$ satisfies the property (i) of $(\tau^*, \beta^*)$-good ellipsoid. 
    The number of high eigenvalues of $M$ is at most $|\whBig_t| \leq \beta'' V^*/\tau_t^2 \leq \beta'' \EV_{\tau^*}(Y^*)/\tau_t^2$. Since $\tau_t^2 \geq \tau_0^2 = d^{c_3}$,  we have $E_{M^*}$ satisfies the property (iii) with $\beta_5 = \beta''/ \tau_t^2 = O(1/d^{c_3})$.
    We now show $M^*$ satisfies the property (ii). Since $|Y^*| \geq \delta_1 |Y|$ and the final set $\whY_t$ used to generate $M^*$ satisfies $|\whY_t \cap Y^*| \geq |Y^*|/4$, we have $|\whY_t \cap Y^*| \geq \delta_1 |\whY_t|$. Thus, we have $\Sigma_{\whY_t} \succeq \delta_1 \Sigma_{Y^*}$. 

    Suppose $\EV_{\tau^*}(Y^*) = 0$, then we have the correct guess $V^* = 0$. Since after each iteration the normalized excess variance $\widehat\EV_{\tau_t}(\whY_t)$ decreases by a factor of $1/\beta'' = 1/\log^{\Omega(1)} d$ and $\tau_t^2$ increases by a factor of $4$,
    Thus, after $L$ iterations, we have 
    \begin{align*}
        \tau_L^2 \cdot |\whBig_L| =(2^L)\tau_0^2 \cdot |\whBig_L|  \leq \widehat\EV_{\tau_L}(\whY_L) \leq \frac{1}{(\beta'')^L} \cdot d.
    \end{align*}
    Thus, for $\tau_0 = \poly\log (d)$, we have after $L=O(\log d/\log\log d)$ iterations, 
    $|\whBig_L| \leq \frac{1}{(2\beta'')^L \tau_0^2} d < 1$, which means $|\whBig_L| = 0$ and the procedure stops.

    % At this point, we can combine Claim~\ref{claim:inlier_remain} and Claim~\ref{claim:outlierdecrease} to argue that even after $O(\log d)$ iterations, most of the points from $X \cap B^*$ remain since we only lose $1-1/\beta$ fraction of the points in each step and $\beta = \omega(\log d)$. On the other hand, the excess variance of $\whX$ goes down by a $1/\beta'' = 1/\log^{\Omega(1)} d$ factor in each iteration. Combining them, we see that after $O(\log d)$ iterations we succeed in finding a set $\whX$ has that $|\whBig| \le \poly\log(d) \cdot \EV_\tau(\whX)$. Hence we can now construct the natural choice of $M$ from this to get a good ellipsoid. 
    % This completes the proof of Lemma~\ref{lem:find:goodep}.
\end{proof}

 \anote{Need to add some extra details, but the argument seems there.}  
\anote{This now needs to be combined with proof of Lemma 5.3, to apply this algorithm recursively to get an algorithmic version of Lemma 5.3.  }
%%%% OLD STUFF %%%%%%%%%%%%%%%%%%%
% The next proposition shows how we can cover most of the set of points inside the ball using $O(1)$ many good shrinking ellipsoids. 


% \begin{enumerate}
%     \item[(i)] {\em (Capturing high variance directions)}  Let $\ProjMhi$ be the projector onto the subspace $\span(\{v_i: a_i > 1\})$ corresponding to large eigenvalues of $M$. For any unit vector $u \in \R^d$ such that $\Var_{x \unif X}[\iprod{u,x}] \ge \tau_1 R^2/d$, we have 
%     \begin{equation}\label{eq:goodep:cond1}
%         \frac{c_1 d}{R^2} \cdot \Var_{x \unif X}[\iprod{u,x}] \le u^\top M u , \text{ and } \norm{\Pi_{M,\ge \tau'} u}_2^2 \ge 1/c_2,
%     \end{equation}
%     where $\Pi_{M,\ge \tau}$ is the projector onto the subspace corresponding to the eigenvalues of $M$ larger than $\tau'$. 
%     \anote{Took out $\le \frac{c_2 d}{R^2} \cdot \Var_{x \unif X}[\iprod{u,x}].$.}
%     \item[(ii)] Let $\tSmall(M)=\{i \in [d]:a_i < 1\}$. We have 
%     $$1 - \frac{\EV(X)}{c_1 |\tSmall(M)|} \le a^2_i \le 1 - \frac{c_2 \EV(X)}{|\tSmall(M)|} ~~\forall i \in \tSmall(M).$$
%     Moreover for all $i \in [d] \setminus \tBig  \setminus \tSmall$, $\frac{1}{2} \le a_i \le c_2 \tau$. \anote{Maybe we can relax it to $1-\gamma$ too.} 
%     \anote{There may be a lot of slack here as well e.g., this doesn't need to hold for all $i \in \tSmall$.}
    
%     % where $\gamma = $
%     \item[(iii)] We also have that $\sum_{i=1}^d \max\{a_i^2 -1 ,0\} = O(\EV(X))=O(1) \cdot \sum_{i=1}^d \max\{\eigval_i^2 -1,0\}$.\anote{change it to a universal constant?}
% \end{enumerate}
% We will call the quantity $\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2$ the {\em excess variance} of $X$. 
% \end{definition}

% \anote{Should it be $\gamma=\frac{\sum_{i=1}^d (\max\{\eigval_i^2 -\tau^2,0\})R^2}{d}$ instead?}

% %The following definition seems to be more natural and elegant, and seems almost the same. 
% \anote{There is a different definition potentially inspired by Vaidehi's suggestion to be of the form $\alpha \Sigma + \beta I$.. but there seemed to be some issues, and needed some non-linearity...}

% % \begin{definition}[Good Shrinking Ellipsoid for a ball $B$]\label{def:goodep:vaidehi}
% %  Consider a ball $B=\Ball(0,R)$ containing points $X$, and ellipsoid $E_M$ given by $E_M=\{x: x^\top M x \le R^2\}$. %where $M = V \diag(a)^2 V^\top$ is its eigendecomposition with eigenvalues $a_1^2, \dots, a_d^2$. 
% %  Let the covariance matrix of $X$ be $\Sigma_X$ with % $\Sigma_X= R^2 \cdot U \diag(\lambda) U^\top$, where 
% % eigenvalues $\eigval_1^2 R^2, \dots, \eigval_d^2 R^2$  (note: $\sum_{i=1}^d \eigval_i^2 \le 1$), and let $\EV(X)=\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2$. Given $\tau, c\ge 1 $, $M$ is $(\tau,c)$-good  if $\exists$ constants $c_1, c_2, c' \ge 1$ s.t.
% % \begin{align}\label{def:goodep:vaidehi}
% %    \frac{1}{\tau^2 R^2} ~ \Sigma_X + \Big(1-\frac{\gamma}{c}\Big) I &\preceq M \preceq \frac{c'}{\tau^2 R^2} ~  \Sigma_X + \Big(1-\frac{c' \gamma}{c}\Big) I + M_{err}, \\
% %    \text{where }  \gamma = \frac{\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2}{d}, &\text{ and } M_{err} \succeq 0 \text{ with } \tr(M_{err}) = O(\EV(X)).
% % \end{align}
% % 
% % %and $\tr(M_{err}) \le \EV(X)$. 
% % %with % $\Sigma_X= R^2 \cdot U \diag(\lambda) U^\top$, where 
% % % eigenvalues $\eigval_1^2 R^2, \dots, \eigval_d^2 R^2$  (note: $\sum_{i=1}^d \eigval_i^2 \le 1$), and let $\EV(X)=\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2$. The ellipsoid is said to be $(\tau,c_1, c_2)${\em good} for $B,X$ if there exists $\tau \ge 1$ and constants\anote{check} $c_1, c_2$ such that
% % % \begin{enumerate}
% % %     \item[(i)] {\em (Elongated along high variance directions)}  For any unit vector $v \in \R^d$ such that $\Var_{x \unif X}[\iprod{u,x}] \ge \tau^2 R^2/d$, we have 
% % %     \begin{equation}
% % %         \frac{1}{c_1} \cdot \Var_{x \unif X}[\iprod{u,x}] \le \norm{M u}_2^2 \le c_2 \Var_{x \unif X}[\iprod{u,x}].
% % %     \end{equation}
% % %     \item[(ii)] For all $r_i \le 1$, we have $1 - \frac{\gamma}{c_1} \le r_i \le 1 - c_2 \gamma$
% % %     \item[(iii)] We also have that $\sum_{i=1}^d \max\{a_i^2 -1 ,1\} = O(\EV(X))=O(1) \cdot \sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2)$.\anote{change it to a universal constant?}
% % % \end{enumerate}
% % % We will call the quantity $\sum_{i=1}^d (\max\{\eigval_i^2 -1,0\})R^2$ the {\em excess variance} of $X$. 
% % \end{definition}


% % \begin{lemma}\label{lem:ellipsoid-shrink}
% % Let $Y$ be a set of points in the ball $B^*$ with center $c$ and radius $R$, and let $\Sigma_Y=V \diag(r)^2 V^\top$ be its covariance matrix with eigenvalues $r_1^2, r_2^2, \dots, r_d^2$ and eigenvectors given by $V$. For any constants $c_1, c_2 \ge 1, \delta \in (0,1)$, and any sufficiently large $a \ge a_0(c_1, c_2)$ \anote{we may want to make it $\log d$ or even $d^{\epsilon}$?} such that any $\eta \in (0,1)$ if $\tBig=\{i \in [d], r_i^2 \ge \frac{a^2 R^2}{d} \}$, the following holds. Consider any ellipsoid $\widehat{E}$ given by $(x-c)^\top M (x-c) \le R^2$ such that $M=V \diag(a)^2 V^\top$ with 
% % $$a_i = \begin{cases} \end{cases}.$$
% % %are the same as that of $\Sigma_Y$ with corresponding eigenvalues satisfying $$ then 
% % Then at least one of the following holds:
% % \begin{enumerate}
% %     \item[(i)] $\sum_{i \in \tBig} r_i^2 \le O(\log (d/\delta))$. \anote{note sure how best to set this RHS; maybe even a large constant suffices.}
% %     \item[(ii)] For at least $1-\delta$ fraction of the points, we have that the length of $x$ restricted to the coordinates $\tBig$ is significantly smaller than its expectation i.e., \[\sum_{i \in \tBig} x_i^2 \le \eta \sum_{i \in \tBig} r_i^2, \label{eq:case2}\] 
% %     \item[(iii)] 
% % \end{enumerate}
% % \end{lemma}

% \begin{lemma}[Properties of good shrinking ellipsoids]\label{lem:goodep}
% Consider a ball $B=\Ball(0,R)$ containing points $X$, and let ellipsoid $E_M$ given by $E_M=\{x: x^\top M x \le R^2\}$ be a $(\tau,c)$-good shrinking ellipsoid for $X$. There exists universal constants $c'\ge 1$ such that for any $\delta>0$, if $\tBig = \{i \in [d]: a_i^2 \ge c' \tau^2 \}$, then 
% \begin{enumerate}
%      \item[(a)] The points in $X$ have bounded variance in the transformed space $M^{-1/2} x$ i.e.,  for each unit vector $u \in \R^d$, $\Var_X[\iprod{M^{-1/2} x,u}] \le c_1 \tau R/\sqrt{d}$. 
%      \item[(b)] The volume of $E_M$ is smaller i.e.,  
%      $$ \Vol(E_M) \le \Vol(B) \cdot \exp\Big( - \Omega(1/\tau^2) \cdot  \cdot \EV(X) \Big)$$
%      \anote{We may not need this much improvement?}
%      \item[(c)] Most points with non-negligible mass on the big coordinates also belong to $E_M$ i.e., there exists a universal constant $c_1>0$ such that for any $\eta \ge c_1/c$ we have that for at least $1-O(1/c)$ points of $X$, 
%      $$\sum_{i\in \tBig} \iprod{x , v_i}^2 \ge \eta \E_X\Big[\sum_{i \in \tBig} \iprod{x , v_i}^2\Big] ~~\implies~~ x \in E_M. $$
%      \anote{The dependence on $c, \beta$ in the last claim needs to be checked.}
%      % \begin{align}
%      %     \Pr_{X}\Big[ \sum_{i \in \tBig] \iprod{x , v_i}^2 \le \eta \E_X[\sum_{i \in \tBig] \iprod{x , v_i}^2]\Big] \le 1-\delta  ~~\implies~ \Pr_X[x \notin E_M] \le \delta + c.
%      % \end{align} 
%      %For at least $1-\delta$ fraction of the points, we have that the length of $x$ restricted to the coordinates $\tBig$ is significantly smaller than its expectation i.e., \[\sum_{i \in \tBig} x_i^2 \le \eta \sum_{i \in \tBig} r_i^2, \label{eq:case2}\] 
% %     \item[(iii)] 
%  \end{enumerate}

% \end{lemma}
% \begin{proof}
% The first property (a) follows from property (i) of good shrinking ellipsoids. To upper bound the variance of $M^{-1/2} x$ along every direction by $O(\tau R^2/d)$, it suffices to prove that for 
% $$\forall u \in \R^d, ~ \frac{u^\top \Sigma_X u}{u^\top M x} \le c_1 \tau R^2/d.$$
% For directions $u$, with variance $> \tau R^2/d$, property (1) implies the above. On the other hand if the variance is smaller than $\tau R^2/d$, then we can use the fact that $a_i^2 \ge 1/2$.  %In particular for every large variance direction $u$ with variance at least $\tau R^2/d$, \eqref{eq:goodep:cond1} ensures that the variance of $M^{-1/2} x$ along $u$ is $u M^{-1/2} \Sigma_X M^{-1/2}$
% %uses $M \succeq \beta \Sigma$. Hence for any unit vector $u \in \R^d$
% %$$\Cov_X[M^{-1/2} x] = M^{-1/2} \Sigma_X M^{-1/2} \preceq (\beta \Sigma_X)^{-1/2} \Sigma_X (\beta \Sigma_X)^{-1/2} \preceq \big(\tfrac{1}{\beta}\big)  I. $$

% We now show property (b). %Let $M_0 = \tfrac{1}{\tau^2} \Sigma_X + (1-\gamma/c) I$. 
% Let $a_1^2, \dots, a_d^2$ be the eigenvalues of $M_0$ and let $v_1, \dots, v_d$ be its corresponding eigenvectors. The ellipsoid $E_{M_0}=\{x: x^top M_0 x \le R^2 \} \supseteq \{x: x^\top M x \le R^2\} = E_M$. Compared to the ball $B=\{x: \sum_i x_i^2 \le R^2\}$ their volumes
% \begin{align*}
% \frac{\vol(E_M)}{\vol(B)} & \le \frac{\vol(E_{M_0})}{\vol(B)} = a_1 a_2 \cdots a_d \le 1, 
% \end{align*}
% by the AM-GM inequality, since $a_1^2 + \dots + a_d^2 \le d$; note that the expression is maximized when all the $a_i = 1$ (i.e., the ball of radius $R$).  


% Before we quantify the volume shrinkage, we first get bounds for the eigenvalues $a_i^2$.  

% % \begin{claim}
% % Let $\tSmall(M)=\{i \in [d]:a_i < 1\}$. We have 
% %     $$1 - \frac{\EV(X)}{c_1 |\tSmall(M)|} \le a^2_i \le 1 - \frac{c_2 \EV(X)}{|\tSmall(M)|} ~~\forall i \in \tSmall(M).$$
% % \end{claim}

% We now quantify the volume shrinkage using the concavity of the logarithm function. 




% \begin{align*}
% 2\log\Big(\frac{\vol(E_M)}{\vol(B)}\Big) & = \log( a^2_1 a^2_2 \cdots a^2_d) = , 
% \end{align*}

% \anote{Some difficulty with the last part...}

% \end{proof}


\begin{theorem}
    Suppose we are given a set of points \(Y \subseteq \mathbb{R}^d, |Y| = n\), and \(0 \le \delta \le 1, 0 \le \gamma \le 1\), such that there exists a subset \(Y^\star \subseteq Y\), \(|Y^\star| \ge \delta |Y|\), that is contained in an unknown ball \(B^\star = B(c^\star, R^\star)\). 

    Then we can find an ellipsoid \(\widehat{E}\) such that \(|\widehat{E} \cap Y| \ge \delta_2 |Y^\star|\) \vnote{Include what this fraction is, it's now much smaller than in the ball case}, and 
    \[\frac{\mathrm{vol}(\widehat{E})}{\mathrm{vol}(B^\star)} \le \exp \left( \frac{d^{1/2 + o(1)}}{\sqrt{\delta}}  \right). \]
\end{theorem}

\begin{proof}
    \vnote{Taking \(\delta = \delta_1\) to mean \(\frac{|Y^\star|}{|Y|}\).}
    Applying Lemma \ref{lem:covering-good-ellipsoids} to \(Y^\star\) tells us that there exists a subset \(Y^{\star\star} \subseteq Y^\star\) of size \(|Y^{\star\star}| \ge \frac{1}{\log^{1/\varepsilon} d} \cdot |Y^\star|\) \vnote{i.e., \(\delta_2 = \frac{1}{\log^{1/\varepsilon} d}\)} and \((\tau^{\star\star})^2 \in (2, 4^{1 + 1/\varepsilon} \log^{1/\varepsilon} d)\) such that if \(\Sigma^{\star\star}\) is the covariance matrix of \(Y^{\star\star}\) and \(\mathrm{Proj}_{\star\star}^{> \tau^{\star\star}}\) is the projection matrix onto the eigenspace with eigenvalues larger than \(\tau^{\star\star}\), then one of the following properties holds:
    \begin{enumerate}
        \item \(\lambda_{\mathrm{max}}(\Sigma^{\star\star}) \le (\tau^{\star\star})^2\) ;
        \item there exists \(\Yin \in Y^{\star\star}\) of size \(|\Yin| \ge (1 - \delta_3) |Y^{\star\star}|\) \vnote{Double check that this should actually be \((1 - \delta_3)\) and not just \(\delta_3\).} such that for any \(y \in \Yin\),
        \[\|\mathrm{Proj}_{\star\star}^{> \tau^{\star\star}} y \|^2_2 \ge \eta \cdot \mathrm{EV}_{\tau^{\star\star}}(Y^{\star\star}),\]
    \end{enumerate}
    where \(\delta_3 = O(1 / \log d)\) and \(\eta = 1 / d^{\varepsilon}\) for \(\varepsilon \in (0, 1)\).

    This condition allows us to apply Lemma \ref{lem:find:goodep}, which tells us that Algorithm \textsc{Good\_Ellipsoid} finds a list of $\ell=\poly(d)$ ellipsoidal shapes $M_1, \dots, M_\ell$ such that there exists $M \in \{M_1, \dots, M_\ell\}$ for which the shifted ellipsoid $E_{M}=\{x: (x-c)^\top M (x-c) \le (R^*)^2\}$ is a \((\tau^{\star\star}, \beta)\)-good ellipsoid for $B^{\star},Y^{\star\star}$. \vnote{The parameters of the good ellipsoid appear here by magic.  The chain of parameters needs to be tracked down.  What is \(\beta\)?}  

    Lemma \ref{lem:goodep} tells us that \(E_M\) being a \((\tau^{\star\star}, \beta)\)-good ellipsoid for \(B^\star, Y^{\star\star}\) means that  
    \begin{enumerate}
        \item[(a)] the points in \(Y^{\star\star}\) have bounded variance in the transformed space \(M^{-1/2} y\), i.e., for each unit vector \(u \in \mathbb{R}^d\)
        \[\mathrm{Var}_{y \sim_{u} Y} \left[ \langle M^{-1/2} y, u\rangle \right] \le O(\tau^{\star\star} R^2 / d).\]
        \item[(b)] The volume of \(E_M\) is smaller, i.e., 
        \[ \mathrm{vol}(E_M) \le \mathrm{vol}(B) \cdot \exp\left( - \frac{4 \ln d - 2}{4} \right).\]
        \item[(c)] We have that for any point \(y \in Y^{\star\star}\), it holds that 
        \[\|\mathrm{Proj}_{\star\star}^{>\tau^{\star\star}} y\|^2_2 \ge \eta \cdot \mathrm{EV}_{\tau^{\star\star}}(Y^{\star\star}) \qquad \Longrightarrow \qquad y \in E_M.\]
    \end{enumerate}
    In particular, this means that \(\Yin \subseteq E_M\).  

    Now, for each potential ellipsoid \(M_i\) in the list, we can do the following.  We transform all points \(Y\) by \(M_i^{-1/2}\).  Then, we apply the algorithm from Corollary \ref{cor:ball-bounded-variance-better-bounds} with the fraction of inliers set to \(\delta \cdot \delta_2 \cdot (1 - \delta_3)\) \vnote{or is it \(\delta_3\)?}.  This returns a ball \(B\) in the transformed space, and we take \(E_i = M^{1/2} B\) as a candidate ellipsoid.  Note that \(E_i\) is guaranteed to contain \(\delta \cdot \delta_2 \cdot (1 - \delta_3) \cdot (1 - \gamma)\) fraction of \(Y\).  Of all of the candidate ellipsoids, we output the one with minimum volume.

    Let \(M^\star\) be the ellipsoid in our list that is a \((\tau^{\star\star}, \beta)\)-good ellipsoid for $B^{\star},Y^{\star\star}$.  Since the points in \(Y^{\star\star}\) have bounded variance in the transformed space \(M^{-1/2} y\), we have that the ball \(\Bhat\) output by Corollary \ref{cor:ball-bounded-variance-better-bounds} will have radius at most 
    \[R^\star \left(1 +  O( (\gamma^{-1/2} + (\delta \delta_2 (1 - \delta_3))^{-1/2}) (\tau^{\star\star})^{1/2})\right),\]
    where \(R^\star\) is an upper bound on the radius of \(E_{M^\star}\) in the transformed space.  Thus, the ratio of the volume of \(\Bhat\) to the transformed \(E_{M^\star}\) is 
    \[\le \exp \left( d \cdot (\gamma^{-1/2} + (\delta \delta_2 (1 - \delta_3))^{-1/2}) (\tau^{\star\star})^{1/2} \right) ,\]
    and the ratio of the volume of the candidate ellipsoid to the volume \(E_{M^\star}\) is the same. 

    Setting parameters appropriately \vnote{help!} we get that this volume ratio is bounded by 
    \[\le \exp \left( \frac{d^{1/2 + o(1)}}{\sqrt{\delta}}  \right). \]
    
\end{proof}

\newpage

==> Paper/hardness.tex <==
\section{Hardness}
In this section, we show the approximation hardness of finding one ellipsoid or the union of ellipsoids with the smallest volume that achieves the required coverage. 

We first show the hardness of finding the smallest ellipsoid with required coverage. 

\begin{theorem}
    
\end{theorem}

We show the approximation hardness of finding the union of ellipsoids with the smallest volume that achieves the coverage condition through the hardness of the continuous learning with errors (CLWE) by~\cite*{bruna2021continuous}. We first define the $m$-homogeneous CLWE distribution and the corresponding decision problem $\mathrm{hCLWE}^{(m)}_{\beta,\gamma}$.

\begin{definition}[$m$-homogeneous CLWE distribution]
    Let $d$ be the dimension and $0<m<d$ be the number of secret directions. Let $W \in \R^{d\times m}$ be a matrix with orthonormal columns $w_1,\dots,w_m$. For parameters $\beta,\gamma>0$, the $m$-homogeneous CLWE distribution $H_{W,\beta,\gamma}$ is defined on $\R^d$ with the density at $x$ proportional to 
    $$
    \rho_1(x) \cdot \prod_{i=1}^m \sum_{k \in \Z} \rho_{\beta} (k-\inner{x}{w_i}),
    $$
    where $\rho_s(x) = \exp(-\pi\cdot \|x\|_2^2/s^2)$ is the density of the Gaussian distribution  with covariance $s^2/(2\pi) \cdot I_d$.
\end{definition}

\begin{definition}
    For parameters $\beta,\gamma>0$ and $0<m<n$, the decision problem $\mathrm{hCLWE}^{(m)}_{\beta,\gamma}$ is to distinguish the following two distributions on $\R^d$: (1) $m$-homogeneous CLWE distribution $H_{W,\beta,\gamma}$, and (2) the spherical Gaussian $N(0, \frac{1}{2\pi}I_d)$.
\end{definition}

\begin{theorem}
    Let $\beta = \beta(d) \in (0,1)$ and $\gamma = \gamma(d) \geq 2\sqrt{d}$ and $\gamma/\beta$ is polynomial in $d$ and $1\leq  m < d- d^c$ for some constant $c$. If there is a polynomial time algorithm that finds a coverage set with $(\gamma/\beta)^m$ volume approximation, then there is a polynomial time algorithm that solves $m$-homogeneous CLWE, $\mathrm{hCLWE}^{(m)}_{\beta,\gamma}$.
\end{theorem}

\begin{proof}
    Consider the $m$-homogeneous CLWE distribution $H_{W,\beta,\gamma}$ for some matrix $W \in \R^{d\times m}$ with orthonormal columns $w_1,\cdots, w_m$. For any point $x \in \R^d$, the density at this point is proportional to $$
    \rho_1(x) \cdot \prod_{i=1}^m \sum_{k \in \Z} \rho_{\beta} (k-\inner{x}{w_i}),
    $$
    where $\rho_s(x) = \exp(-\pi\cdot \|x\|_2^2/s^2)$ is the density of the Gaussian distribution  with covariance $s^2/(2\pi) \cdot I_d$. The distribution $H_{W,\beta,\gamma}$ can be equivalently defined as a mixture of Gaussians. The density at point $x$ is 
    \begin{align*}
        f(x) = C_{\beta,\gamma} \cdot \sum_{k \in \Z} \rho_{\sqrt{\beta^2+\gamma^2}}(k) \cdot \rho_1(\pi_{W^{\bot}}x) \cdot
        \prod_{i=1}^m \rho_{\beta/\sqrt{\beta^2+\gamma^2}}\left(\inner{x}{w_i}- \frac{\gamma}{\gamma^2+\beta^2} \cdot k\right),
    \end{align*}
    where $C_{\beta,\gamma} = 1/\sum_{k \in \Z} \rho_{\sqrt{\beta^2+\gamma^2}}(k) \approx 1/\sqrt{\beta^2+\gamma^2}$ is the normalization factor.
    
    % Note that $\sum_{k \in \Z} \rho_{\sqrt{\beta^2+\gamma^2}}(k) = \int_{-\infty}^\infty e^{-\pi x^2/(\beta^2+\gamma^2)} \mathrm{d} x = \sqrt{\beta^2+\gamma^2}$.
    % Thus, we have $C_{\beta,\gamma} = 1/\sqrt{\beta^2+\gamma^2}$. 
    Then, the hCLWE distribution is a mixture of Gaussians where each component is labeled by $k \in \Z$. The component with label $k$ has a weight $C_{\beta,\gamma} \cdot \rho_{\sqrt{\beta^2+\gamma^2}}(k)$ and follows the Gaussian distribution with variance $\frac{1}{2\pi}\cdot \frac{\beta^2}{\beta^2+\gamma^2}$ on $m$ secret directions and variance $\frac{1}{2\pi}$ on the orthogonal directions.

    We now bound the smallest volume among sets that cover at least $1-\alpha$ probability mass for this hCLWE distribution. We consider each component separately. Specifically, we pick a threshold $t > 0$, and then for each component $k \in \Z$, we pick the ellipsoid set $E_k$ with point $x$ such that 
    $$
    C_{\beta,\gamma} \cdot \rho_{\sqrt{\beta^2+\gamma^2}}(k) \cdot f_k(x) \geq t,
    $$
    where $f_k(x)$ is the density of the Gaussian distribution for component $k$.

    Without loss of generality, we shift the origin to the mean of the component $k$ and pick $w_1,\cdot w_m$ as basis vectors and expand it to $\R^d$. Let $\Sigma$ be the covariance matrix of the Gaussian distribution for component $k$. Then, we have $\Sigma = \mathrm{diag}(\sigma_1^2,\cdots, \sigma_d^2)$, where $\sigma_1,\dots,\sigma_m$ are $\frac{1}{2\pi}\cdot\frac{\beta^2}{\beta^2+\gamma^2}$ and others are $\frac{1}{2\pi}$. Then, the ellipsoid $E_k$ is 
    $$
    E_k = \left\{x: \sum_{i=1}^d \frac{x_i^2}{\sigma_i^2} \leq R_k^2\right\},
    $$
    where $R_k^2 = \max\left\{0,-2\ln\left(t(2\pi)^{d/2} \prod_{i=1}^d \sigma_i/ (C_{\beta,\gamma}\cdot \rho_{\sqrt{\beta^2+\gamma^2}(k)})\right)\right\}$. The probability mass of the component $k$ covered by this ellipsoid is 
    $F_{\chi_d^2}(R_k^2)$ fraction, where $F_{\chi_d^2}$ is the CDF of the chi-squared distribution with degree $d$. To cover at least $1-\alpha$ fraction of the hCLWE, we have to pick $t$ such that 
    $$
    \sum_{k \in \Z} C_{\beta,\gamma}\cdot \rho_{\sqrt{\beta^2+\gamma^2}}(k) \cdot F_{\chi_d^2}(R_k^2) \geq 1-\alpha.
    $$
    Note that $R_k^2 = R_0^2 -2\pi \cdot \frac{k^2}{\beta^2+\gamma^2}$. By picking $\widetilde k = \sqrt{\ln(1/\varepsilon)(\beta^2+\gamma^2)}$, then we have 
    $$
    \sum_{k = - \widetilde k}^{\widetilde k} C_{\beta,\gamma}\cdot \rho_{\sqrt{\beta^2+\gamma^2}}(k) \cdot F_{\chi_d^2}(R_k^2) \geq \left(1-\frac{\sqrt{\beta^2+\gamma^2}}{\pi \widetilde k}\cdot e^{-\pi \widetilde k^2/(\beta^2+\gamma^2)}\right) F_{\chi_d^2}(R_{\widetilde k}^2) \geq (1-\varepsilon) F_{\chi_d^2}(R_{\widetilde k}^2).
    $$
    By taking $R_{\widetilde k} = r$ such that $F_{\chi_d^2}(r^2) = (1-\alpha)/(1-\varepsilon)$, we get the coverage condition.

    The total volume of these ellipsoids $E_k$ for $k$ from $-\widetilde k$ to $\widetilde k$ is 
    $$
    \sum_{k=-\widetilde k}^{\widetilde k} \vol(E_k) = C_d \cdot \prod_{i=1}^d \sigma_i \cdot \sum_{k = -\widetilde k}^{\widetilde k} R_k^d,
    $$
    where $C_d = \pi^{d/2}/(\Gamma(d/2)+1)$.

    We next consider the spherical Gaussian with dimension $d$ and variance $\frac{1}{2\pi}$. Let $B_r = \{x: 2\pi \|x\|_2^2 \leq r^2\}$ be the ball with radius $r/\sqrt{2\pi}$ cantered at the origin.
    Since we pick $r$ such that $F_{\chi_d^2}(r^2) = (1-\alpha)/(1-\varepsilon)$, we have the ball $B_r$ covers $(1-\alpha)/(1-\varepsilon)$ probability mass of this spherical Gaussian. The volume of this ball is 
    $$
    \vol(B_r) = C_d \cdot (2\pi)^{-d/2}\cdot r^d.
    $$

    Note that $R_0^2 = r^2 + 2\pi\ln(1/\varepsilon)$. Then, we have the ratio of the volume is 
    \begin{align*}
        \frac{\vol(B_r)}{\sum_{k=-\widetilde k}^{\widetilde k}\vol(E_k)} = \frac{r^d}{\sum_{k = -\widetilde k}^{\widetilde k} R_k^d} \cdot \left(\frac{\sqrt{\beta^2+\gamma^2}}{\beta}\right)^m \geq \frac{1}{2\widetilde k+1} \cdot \left(\frac{r^2}{r^2 + 2\pi \ln(1/\varepsilon)}\right)^{d/2}\cdot \left(\frac{\sqrt{\beta^2+\gamma^2}}{\beta}\right)^m.
    \end{align*}
    For some constant $\alpha \in (0,1)$, we have $r = \Omega(\sqrt{d})$. Since $\widetilde k = \ln(1/\varepsilon) \gamma$ and $\gamma \geq 2\sqrt{d}$ and $\beta \in (0,1)$, we have this ratio is at least 
    $$
    \frac{\vol(B_r)}{\sum_{k=-\widetilde k}^{\widetilde k}\vol(E_k)} \geq \frac{1}{\sqrt{d}}\cdot e^{-c_1}\cdot \left(\frac{\gamma}{\beta}\right)^m.
    $$
\end{proof} 

==> Paper/oldhighdimballs.tex <==
\section{Old Algorithm for Finding Highest Density Ball using List Decodable Mean Estimation}

The goal of this section is to give a polynomial time algorithm that gives an improved an improved $\exp(O(\sqrt{d}))$-approximation for finding the densest ball containing at least $\Omega(n)$ points. 

We start with algorithms based on coresets that obtain a $(1+\varepsilon)^d$ approximation in $n^{1/\varepsilon}$ time for any set of points. This uses the following surprising fact about the existence of coresets of constant size for the minimum enclosing ball.

\begin{fact}[Coreset]\cite{BadiouHI02,BadiouC04,KumarY03}
For any $\varepsilon>0$, given any set of $n$ points $X \subset \R^d$, there exists a subset $S \subseteq X$ of size $|S|=\lceil 1/\varepsilon \rceil$ such that $(1+\varepsilon)$ expansion of the minimum enclosing ball for $S$ contains $X$.  
\end{fact}
This immediately implies an algorithm for the densest ball by guessing the $1/\varepsilon$ sized coreset in $n^{1/\varepsilon}$ time for the subset of points that corresponds to the densest ball.   
\begin{theorem}\label{thm:coreset}
The following holds for any given constants $\gamma, \eps \in (0,1)$. Suppose we are given $n$ points $X \subset \R^d$ with an (unknown) subset $S^* \subseteq X$ of size at least $\gamma n$ enclosed in a ball $B^*$ of radius $r^*>0$. Then the algorithm runs in time $n^{1+1/\epsilon}$, and outputs a ball $B'$ containing at least $\gamma n$ points with density at least $\exp(-\eps d)$ times the density of $B^*$. 
\end{theorem}
\anote{Need to fill this in with 1-2 lines proof.} 


\begin{definition}[Approximately isotropic distributions]\label{def:isotropic}
For $\beta \ge 1$ the distribution $\calD$ over $\R^d$ is $\beta$-approximately isotropic if 
%the maximum variance along any direction is at most $\beta$ factor worse than the average variance i.e.,  
\begin{equation}
\forall v \in \R^d ~~\E_{x \sim D}\big[ \iprod{x-\E[x]}^2 \big] \le \frac{\beta}{d} \cdot \E_{x \sim D} \big[\norm{x}_2^2 \big], \text{ or in other words } \norm{\Sigma_\calD} \le \frac{\beta}{d} \tr(\Sigma_\calD), \text{ where }
\end{equation}
%In other words, if 
$\Sigma_\calD$ is the covariance matrix of $\calD$ and $\norm{\Sigma_\calD}$ denotes its spectral norm. %, then $\norm{\Sigma_\calD} \le \beta \norm{\Sigma_\calD}_F/d$.

For any $r>0$, the distribution $\calD$ is $(r,\beta)$-approximately isotropic if the distribution $\calD$ if the truncated distribution of $\calD$
%truncated 
within the ball $\Ball(\E_\calD[x], r)$ satisfies that the maximum variance in any direction is at most $\beta \cdot r^2/d$. (Note that this is potentially weaker than asking $\calD$ truncated to the ball of radius $r$ being $\beta$-approximately isotropic.) 
\end{definition}
Note that any distribution with finite covariance satisfies $\beta$-approximate isotropicity for $\beta=d$. The notion of $(r,\beta)$-approximate isotropicity also allows us to capture heavy-tailed distributions like the Cauchy distribution which may not even have finite covariance.   

We now show an algorithm that gives better guarantees for any distribution that is $\beta$-approximately isotropic for a non-trivial value of $\beta$. 

\begin{theorem}\label{thm:isotrop}
For any given constant $\gamma \in (0,1)$, there exists a constant $c=c(\gamma)>0$ such that the following holds. Suppose we are given $n$ points $X \subset \R^d$ with an (unknown) subset $S^* \subseteq X$ of size at least $\gamma n$ enclosed in a ball $B^*$ of radius $r^*>0$, and suppose additionally that $S^*$ is $(r^*, \beta)$-approximately isotropic. Then the algorithm runs in polynomial time, and with high probability outputs a ball $B'$ containing at least $\Omega(\gamma n)$ points with density at least $\exp(-c \sqrt{\beta d})$ times the density of $B^*$. 
\end{theorem}

Note that the above result gives an exponential improvement as long as the optimal solution (the densest ball) is approximately isotropic.  

In what follows we will use a polynomial time algorithm for list-decodable mean estimation for bounded covariance distributions \cite{Diakonikolas-Kane-book}. Given $n'$ points $Y$ that there is a cluster with at least $\alpha n'$ points, with mean $\mu$ of variance bounded by $\sigma^2$ in every direction, the algorithm outputs a list of $\poly(1/\alpha)$ means such that at least one of them, say $\mu'$, satisfies $\norm{\mu' - \mu}_2 \le O(1/\sqrt{\alpha}) \cdot \sigma $.  

\anote{State the formal list-decodable mean estimation guarantee for bounded covariance distributions.}

\begin{figure}[htbp]
\begin{center}
\fbox{\parbox{0.98\textwidth}{

\begin{center}\textbf{\Large{Highest Density Ball Algorithm}}\end{center}
%\hline
\vspace{10pt}
%\hline

\textbf{Input:} Parameters $\gamma>0, \beta \ge 1$ and a set of $n$ points $X \subset \R^d$. Set $\gamma'= 2\gamma/3$ \anote{may need to be adjusted}. 

%\anote{Algorithm may need some modifications}
%\noindent {\bf Algorithm Greedy Density}
 \begin{enumerate}
     \item Try out all of the $n$ points as centers, and all of the $n$ possible radii (given by the distances to the other $n-1$ points) to find a ball $\widehat{B}$ containing at least $\gamma n$ points of smallest radius. Note that the radius of $\widehat{B}$ is at most $2 r^*$.  
     %Let $\widehat{\mu}$ be the center of the ball $\widehat{B}$. 
     Set $\sigma = \text{radius}(\widehat{B}) \sqrt{\beta/d}$, and $B' = \widehat{B}$.   
     \anote{The first step may not even be necessary, if we know a guess for $\sigma$...}
     \item Run the algorithm for list-decodable mean estimation to produce a list $L \subset \R^d$ with $|L|\le \poly(1/\alpha)$ of candidate means. 
     \item For each $\mu' \in L$, 
     %do the following procedure
     %\begin{itemize}
      %\item 
      check if there is a ball with center $\mu' \in L$ and appropriate radius (we only need to try out $n-1$ different radii) that contains at least $\gamma' n$ points and has density more than that of $B'$. If yes, update $B'$. 
   %   For different guesses of $\sigma$ (e.g., try out geometrically decaying radii of the form $1/2^i \times \text{radius}(\widehat{B})$):
   %   \begin{itemize}
   % %   \item Let $\widehat{\mu}$ be the center for $\widehat{B}$. Set $\mu'  = \widehat{\mu}+ (\mu_Y - \widehat{\mu}) \Big(1 -\frac{100 \sigma}{\norm{\mu_Y - \widehat{\mu}}} \Big) $.
   %  % \item Set $r' = R^2 - \Ball(\mu', 100\sqrt{d}\sigma)$. 
   %  \item Set $Check if $B''$ contains at least $\gamma' n$ points, and if $\density(B'') > \density(B')$, then set $B' \leftarrow B''$. 
   %   \anote{Unsure yet if what follows needs to be applied recursively many times.}
   %   \end{itemize}
  %   \end{itemize}
 \end{enumerate}
}
}
\end{center}
\label{fig:alggreedy}
\end{figure}

The correctness of the above algorithm relies on the following lemma. This shows that for a high density ball, the mean of the points inside the ball has to be close to the center. 
\begin{lemma}\label{lem:shrinking}
There exists constants $c,c'>0$ such that the following holds. 
Given any set of points $Y$ with mean $\mu_Y$ variance at most $\sigma^2$ contained in a ball $B$ with center $0$ and radius $R$. %, and suppose $Y$ is $(R,\beta)$-approximately isotropic. 
Then for any $t \ge 1$, the ball $\bar{B}$ with center $\bar{\mu}=\mu_Y - t \sigma \frac{\mu_Y}{\norm{\mu_Y}}$ contains at least $(1-\tfrac{1}{t^2})\gamma n$ points and has volume
$$ \frac{\vol(\bar{B})}{\vol(B)} \le \exp \Big(-\frac{d (\norm{\mu_Y} - t\sigma)^2}{4R^2}\Big)
%\le \exp \Big(-\frac{ (\norm{\mu_Y} - t\sigma)^2}{4\sigma^2}\Big).
$$ 
\anote{Earlier it also said $\exp \Big(-\frac{d (\norm{\mu_Y} - t\sigma)^2}{4R^2}\Big)
\le \exp \Big(-\frac{ (\norm{\mu_Y} - t\sigma)^2}{4\sigma^2}\Big)$, but this may not be true..?}
%\le \exp\Big( - \sqrt{d} \cdot \frac{\sqrt{d} \sigma}{R} \Big).$$ %\le  \exp \Big(-\frac{d \norm{\mu_Y}}{4R}\Big) \le \exp( - \beta \sqrt{d} ).$$
Hence (setting $t=2$) we have that either $\norm{\mu_Y}_2 \le 8 \sigma$, or else $\density(\bar{B})/\density(B) \ge 5$ with $\bar{B}$ containing at least $3 \gamma n/4$ points. 
\end{lemma}

\begin{proof}
The main idea is that if the center of the ball is far from the mean $\mu_Y$, then we can move the center of the ball in the direction of $\mu_Y$ towards $\mu_Y$ and shrink the radius by a non-negligible amount.   

Let $v_\mu$ be the unit vector along $\mu_Y$. Let $\bar{\mu} = \mu_Y - t \sigma v_\mu$ be the new center of the ball. %, where $t$ will be set appropriately later. 
So $\bar{\mu} = (\norm{\mu_Y} - t \sigma) v_\mu$. % for an appropriate $\gamma>0$ that will set later on. 
As we are moving the center only along $v_\mu$, the contribution to the distance of each point $x_i$ to the new center $\bar{\mu}$ only changes along the $v_\mu$ component. We have  

\begin{align}
%\forall x_i \in Y ~~ \norm{x_i - \bar{\mu}}_2^2 &= \norm{x_i}_2^2 - 2 \norm{\bar{\mu}} \Bigiprod{x_i-\mu_Y, \frac{\bar{\mu}}{\norm{\bar{\mu}}}}+ \norm{\bar{\mu}}_2^2 \Big( 1- \frac{2}{1-\gamma} \Big).  
\forall x_i \in Y ~~ \norm{x_i}_2^2 &= \norm{x_i - \bar{\mu} + \bar{\mu}}_2^2 = \norm{x_i - \bar{\mu}}_2^2 + \norm{\bar{\mu}}_2^2 + 2 \iprod{x_i-\bar{\mu}, \bar{\mu}} \nonumber\\
\norm{x_i - \bar{\mu}}_2^2 & = \norm{x_i}_2^2 - \norm{\bar{\mu}}_2^2 - 2 \iprod{(\mu_Y - \bar{\mu}), \bar{\mu}} - 2 \iprod{ x_i - \mu_Y, \bar{\mu}} \nonumber\\
&\le  R^2 - (\norm{\mu_Y}^2 - t^2 \sigma^2) - 2 (\norm{\mu_Y}-t \sigma) \iprod{ x_i - \mu_Y, v_\mu} \nonumber \\
&\le R^2 - (\norm{\mu_Y} - t \sigma) \Big( \frac{\norm{\mu_Y} + t \sigma}{2} - \iprod{x_i - \mu_Y, v_\mu}\Big)\label{eq:shrinking:1}
\end{align}
We want to show that for many points $x_i$ in $Y$, we have $\norm{x_i - \bar{\mu}}$ is significantly smaller than $\norm{x_i}$, so that the radius can be decreased. 
By Chebychev inequality applied to the projections along $v_\mu$ (the unit vector along $\mu_Y$), we have for at least $(1-1/t^2)$ fraction of $Y$ that $\iprod{x_i-\mu_Y,v} \le t \sigma$. Hence from \eqref{eq:shrinking:1}, we have that %for at least $1-1/t^2$ fraction of the $x_i$ in $Y$,   
\begin{align} \label{eq:cheb}
\Pr_{x_i \in_U Y}\Big[\norm{x_i-\bar{\mu}}_2^2 \le R^2 - \frac{1}{2}(\norm{\mu_Y} - t\sigma)^2 \Big] \ge 1 - \frac{1}{t^2}.  
\end{align}

Hence by picking the ball $\bar{B}$ to be centered at $\bar{\mu}$ with radius $\sqrt{R^2 - (\norm{\mu_Y} - t \sigma)^2}$ we get 
\begin{align}
\frac{\vol(\bar{B})}{\vol(B)}  &\le \Big(\frac{\sqrt{R^2 - \tfrac{1}{2}(\norm{\mu_Y} - t \sigma)^2}}{R}\Big)^d = \Big(1 - \tfrac{1}{2}\Big(\frac{\norm{\mu_Y} - t \sigma}{R}\Big)^2\Big)^{d/2}  \le \exp \Big(-\frac{d (\norm{\mu_Y} - t\sigma)^2}{4R^2}\Big)
%&\le \exp \Big(-\frac{(\norm{\mu_Y} - t\sigma)^2}{4\sigma^2}\Big),
\end{align}
%where the last inequality  uses the fact that $\sigma^2 \le R^2/d$ (since all the points lie inside a ball of radius $R$). 
When $\norm{\mu_Y} \ge 4t \sigma$, we additionally have 
\begin{align}
\frac{\vol(\bar{B})}{\vol(B)} & \le \exp \Big(-\frac{d (\norm{\mu_Y} - t\sigma)^2}{4R^2}\Big) \le e^{-9d\sigma^2/R} \le e^{-9/4},
%&\frac{\density(\bar{B})}{\density(B)}  \ge \frac{1-1/t^2}{\vol(\bar{B})/\vol(B)} \ge  (1-\tfrac{1}{t^2}) \exp \Big(\frac{d (\norm{\mu_Y} - t\sigma)^2}{4R^2}\Big)
\end{align}
where the last inequality  uses the fact that $d\sigma^2 \le R^2$ (since all the points lie inside a ball of radius $R$). 
This gives the required conclusion.

The $1/2$ in (\ref{eq:cheb}) can be removed by replacing (\ref{eq:shrinking:1}) with the argument below.
\begin{eqnarray*}
\|x_i-\bar{\mu}\|^2 &=& \|x_i\|^2 + (\|\mu_Y\|-2\sigma)^2 -2(\|\mu_Y\|-2\sigma)\iprod{x_i,\frac{\mu_Y}{\|\mu_Y\|}} \\
&=& \|x_i\|^2 + (\|\mu_Y\|-2\sigma)\left(\|\mu_Y\|-2\sigma-2\iprod{x_i-\mu_Y,\frac{\mu_Y}{\|\mu_Y\|}}-2\|\mu_Y\|\right) \\
&=& \|x_i\|^2 - (\|\mu_Y\|-2\sigma)\left(\|\mu_Y\|+2\sigma+2\iprod{x_i-\mu_Y,\frac{\mu_Y}{\|\mu_Y\|}}\right) \\
&\leq& R^2-(\|\mu_Y\|-2\sigma)^2,
\end{eqnarray*}
as long as $\iprod{x_i-\mu_Y,\frac{\mu_Y}{\|\mu_Y\|}}\geq -2\sigma$,
which is satisfied by at least $3/4$ fraction of points according to Chebyshev.
\end{proof}

We now state the following easy claim that by moving the center, we can find a slightly larger ball that achieves a slightly lower density. 
\begin{claim}\label{claim:closeby}
Suppose $B$ is a ball centered at $\mu$ with radius $R$, then the ball $\bar{B}$ centered at $\bar{\mu}$ with radius $R+\norm{\bar{\mu}-\mu}$ has volume at most $\vol(B') \le \vol(B) \cdot (1+\norm{\bar{\mu}-\mu}/R)^d \le \exp(d \norm{\bar{\mu}-\mu}/R)$, and contains at least as many points as $B$.
\end{claim}

We now proceed to the proof of the main theorem of this section. 
\begin{proof}[Proof of Theorem~\ref{thm:isotrop}]
Suppose $B^*$ is the highest density ball with at least $\gamma n$ points $S^*$. 
In the first step of the algorithm, at least one of the balls centered around (an appropriate) point in $S^*$ will contain all of $S^*$ and have radius at most $2r^*$. Let us denote this ball by $B$ and its radius by $R \le 2 r^*$. %\anote{We may not need the first step at all..}
Set $Y=S^*$, let $\mu_Y$ be the mean of the points in $Y=S^*$, and let $\mu^*$ be the center of the ball $B^*$. 

$S^*$ is $(R, \beta)$-approximately isotropic (since $S^*$ is $(r^*,\beta)$-approximately isotropic). 
Hence the maximum variance $\sigma^2$ of $S^*$ satisfies 
\begin{equation}\sigma \le R \cdot \sqrt{\frac{\beta}{d}} \le r^*  \sqrt{\frac{4\beta}{d}}  . \label{eq:sigmabound}\end{equation}

%Set $\sigma = $ . 
Now $S^* \subset B$ and since $|S^*| \ge \gamma n$, we have that $|S^*|/|B \cap X| \ge \gamma$. %Let $Y$ denote $B \cap X$. 
 % and let $\mu_Y$ denote the mean of $Y=B \cap X$. 
The algorithm for list-decodable mean estimation outputs a list $L$ which contains a candidate mean $\mu'$ such that $\norm{\mu' - \mu_Y} \le c_\gamma \sigma $ (here $c_\gamma = O(1/\sqrt{\gamma})$ suffices). 

Moreover, by applying Lemma~\ref{lem:shrinking} with $Y=S^*$ and ball $B^* \subset B$, we get that $\norm{\mu_Y - \mu^*} \le 6 \sigma$. Otherwise $S^*$ is not the optimal density ball, and we call instead continue this argument with the ball given by Lemma~\ref{lem:shrinking} instead (with a small loss in $\gamma$ i.e., with $\gamma' \ge 3\gamma/4$). 

Applying the triangle inequality along with \eqref{eq:sigmabound} we get %But $\norm{\mu' - \mu_Y} \le c_\gamma \sigma$. Combining them, we get $\norm{\mu' - \mu^*} \le (c_\gamma+8) \sigma$.

%Again from $(R,\beta)$-approximate isotropicity,  
\begin{align}
\norm{\mu'-\mu^*} &\le \norm{\mu' - \mu_Y} + \norm{\mu_Y - \mu^*} \le (c_\gamma+8) \sigma 
 \le c' r^* \cdot \sqrt{\frac{\beta }{d}},
\end{align}
for some $c' \le 2(c_\gamma+8)$.
By using Claim~\ref{claim:closeby}, we get that the ball $B'$ centered around $\mu'$ with radius at most $r^*+ \norm{\mu' - \mu^*}$ contains at least $3 \gamma/4$ points in $S^*$ and has volume 
$$\vol(B') \le \vol(B^*) \cdot \exp\Big( d \cdot c' r^* \sqrt{\frac{\beta}{d}}  \cdot \frac{1}{r^*} \Big) \le \vol(B^*) \cdot \exp\Big( c' \sqrt{\beta d}\Big).$$

As the algorithm considers the ball $B'$ with mean $\mu'$ and all appropriate radii, we get the required guarantee.  

\end{proof}


The following result shows that a $2^{o(d)}$ density approximation is possible without any assumption.

\begin{theorem}
Suppose a subset of size $\gamma n$ is enclosed in a ball $B^*$. Then, there exists an algorithm that runs in polynomial time, and with high probability outputs a ball containing at least $3\gamma n/4$ points with density at least $\exp\left(Cd\left(\frac{\log\log d}{\log d}\right)^{1/2}\right)$ times the density of $B^*$.
\end{theorem}
\begin{proof}
We use the notation $B^*=B(\theta,R)$. Without loss of generality, let us write $\gamma=1$, and we can assume $R\asymp\max_i\|x_i-\bar{x}\|$. Let $\mu$ and $\Sigma$ be the sample mean and covariance of the data points. The eigenvalues of the covariance are denoted by $\lambda_1\geq\cdots\geq\lambda_d$. Let $X\in\mathbb{R}^{n\times d}$ be the centered data matrix, which means the $i$th row of $X$ is given by $(x_i-\bar{x})^T$.
Since
$$\frac{R^2}{m}\sum_{j=1}^d\mathbb{I}\{\lambda_j\geq R^2/m\}\leq \sum_{j=1}^d\lambda_j=\frac{1}{n}\|X\|_F^2\leq R^2,$$
we get $\sum_{j=1}^d\mathbb{I}\{\lambda_j\geq R^2/m\}\leq m$. This implies $\lambda_j\leq \frac{R^2}{m}$ for all $j>m$. Denote the eigen-matrix associated with $\lambda_1,\cdots,\lambda_m$ by $U\in\mathbb{R}^{d\times m}$. Then, $P=UU^T$ and $I_d-P$ are both projection matrices. We also define $\sigma^2=\frac{R^2}{m}$, and $\sigma^2$ bounds the variance of the data points $\{(I_d-P)x_i\}_{i\in[n]}$.

Find an $\epsilon$-cover of the set $\{u:Pu=u, \|P(u-\theta)\|\leq 2R\}$. Note that we should actually cover $\{u:Pu=u,u\in\widehat{B}\}$ with $\widehat{B}$ computed from Step 1 of the highest density ball algorithm. The cardinality of the cover is bounded by $\left(\frac{R}{\epsilon}\right)^{O(m)}$. We use $v$ for an arbitrary vector in the cover satisfying $v=Pv$ and $\|v-P\theta\|\leq \epsilon$.

Apply list-decodable mean estimation in the subspace $\{u:(I_d-P)u=u\}$. The output $\hat{\mu}$ satisfies $\hat{\mu}=(I_d-P)\hat{\mu}$ and $\|(I_d-P)(\hat{\mu}-\mu)\|\lesssim \sigma$.

\textit{Case 1.} Suppose $\|(I_d-P)(\mu-\theta)\|\leq 8\sigma$. This implies $\|(I_d-P)(\hat{\mu}-\theta)\|\lesssim \sigma$ by triangle inequality. Since
$$\|(\hat{\mu}+v)-\theta\|^2=\|(I_d-P)(\hat{\mu}-\theta)\|^2+\|P(v-\theta)\|^2\lesssim \sigma^2+\epsilon^2,$$
we obtain the bound $\|(\hat{\mu}+v)-\theta\|^2\lesssim \frac{R^2}{m}$ by taking $\epsilon^2\leq \frac{R^2}{m}$. In this case, we could output the ball $B'=B(\hat{\mu}+v,\|(\hat{\mu}+v)-\theta\|+R)$, and the volume ratio is bounded by
$$\frac{\vol(B')}{\vol(B(\theta,R))}\leq \left(1+\frac{C}{m^{1/2}}\right)^d\leq\exp\left(O\left(\frac{d}{m^{1/2}}\right)\right).$$

\textit{Case 2.} Suppose $\|(I_d-P)(\mu-\theta)\|> 8\sigma$. Define
$$\bar{\mu}=(I_d-P)\mu-2\sigma\frac{(I_d-P)(\mu-\theta)}{\|(I_d-P)(\mu-\theta)\|}.$$
By the same analysis in the proof of Lemma \ref{lem:shrinking}, we know that
\begin{eqnarray*}
&& \|(I_d-P)(x_i-\bar{\mu})\|^2 \\
&\leq& \|(I_d-P)(x_i-\theta)\|^2 -\left(\|(I_d-P)(\mu-\theta)\|-2\sigma\right)^2 \\
&\leq& \|(I_d-P)(x_i-\theta)\|^2 - 36\sigma^2,
\end{eqnarray*}
for at least $3n/4$ points by Chebyshev. The $1/2$ in (\ref{eq:cheb}) can be removed. See the argument added in the end of the proof of Lemma \ref{lem:shrinking}.
We also have
$$\|Px_i-v\|^2\leq (\|Px_i-P\theta\|+\|P\theta-v\|)^2\leq \|Px_i-P\theta\|^2 + 2\epsilon R+\epsilon^2.$$
The above bounds implies
\begin{eqnarray*}
&& \|x_i-(\bar{\mu}+v)\|^2 \\
&\leq& \|(I_d-P)(x_i-\theta)\|^2+\|Px_i-v\| - 36\sigma^2 \\
&\leq& \|(I_d-P)(x_i-\theta)\|^2+\|Px_i-P\theta\|^2 + 2\epsilon R+\epsilon^2 - 36\sigma^2 \\
&=& \|x_i-\theta\|^2 + 2\epsilon R+\epsilon^2 - 36\sigma^2 \\
&\leq& R^2-30\frac{R^2}{m},
\end{eqnarray*}
where we take $\epsilon$ satisfying $\epsilon\leq \frac{R}{m}$. To summarize, the ball $B(\bar{\mu}+v,\sqrt{R^2-30\frac{R^2}{m}})$ contains at least $3n/4$ points, and its volume is bounded by
$$\frac{\vol(B(\bar{\mu}+v,\sqrt{R^2-30\frac{R^2}{m}}))}{\vol(B(\theta,R))}\leq \left(1-\frac{30}{m}\right)^{d/2}\leq \exp\left(-C'\frac{d}{m}\right).$$
Since $\|(\hat{\mu}+v)-(\mu+v)\|=\|\hat{\mu}-\mu\|\lesssim\sigma$, we shall output the ball $B'=B(\hat{\mu}+v,C\sigma+\sqrt{R^2-30\frac{R^2}{m}})$. This ball contains at least at least $3n/4$ points, and its volume is bounded by
$$\frac{\vol(B')}{\vol(B(\bar{\mu}+v,\sqrt{R^2-30\frac{R^2}{m}}))}\leq \left(1+\frac{C\sigma}{\sqrt{R^2-30\frac{R^2}{m}}}\right)^d=\exp\left(O\left(\frac{d}{m^{1/2}}\right)\right),$$
and therefore
$$\frac{\vol(B')}{\vol(B(\theta,R))}\leq \exp\left(O\left(\frac{d}{m^{1/2}}\right)-C'\frac{d}{m}\right)=\exp\left(O\left(\frac{d}{m^{1/2}}\right)\right).$$

We require $\epsilon$ to satisfy $\epsilon^2\leq \frac{R^2}{m}$ and $\epsilon\leq \frac{R}{m}$. We shall take $\epsilon= \frac{R}{m}$. This leads to the cardinality bound (of the cover) as $\left(\frac{R}{\epsilon}\right)^{O(m)}=m^{O(m)}$. In order that the bound is a polynomial in $d$, we should take $m\asymp\frac{\log d}{\log\log d}$.
\end{proof}


==> Paper/oldintro.tex <==
\section{Introduction}

\cnote{methods in the literature}




\subsection{Existing Methods}

\paragraph{Statistical methods.}
Given samples $Y_1,\cdots,Y_n$ independently drawn from an arbitrary distribution $P$ on $\mathbb{R}^d$, our goal is to learn a $(1-\alpha)$-level confidence set $\widehat{C}$ such that $P(\widehat{C})\geq 1-\alpha$ and $\vol(\widehat{C})$ is as small as possible. This classical problem, which goes under the name of learning minimum volume sets, learning density level sets or anomaly detection, has a long history in statistical learning and computer science. Learning algorithms that have been studied in the literature can roughly be categorized into the following three classes.
\begin{enumerate}
\item \textit{Excess mass functional.} A straightforward method of learning confidence set with small volume is
\begin{equation}
\min_{C\in\mathcal{C}}\vol(C)\quad\text{s.t. }\mathbb{P}_n(C)\geq 1-\alpha-\gamma, \label{eq:ERM}
\end{equation}
where $\mathcal{C}$ is a class of sets with some VC dimension bound and $\gamma$ is a slack parameter \citep{scott2005learning}. A more general objective function called excess mass functional proposed by \cite{hartigan1987estimation} is defined by
\begin{equation}
E_{\lambda}(C) = \mathbb{P}_n(C) - \lambda\vol(C), \label{eq:EMF}
\end{equation}
where the parameter $\lambda>0$ is determined by the confidence level. In fact, maximizing the excess mass functional over $C\in\mathcal{C}$ is equivalent to (\ref{eq:ERM}). This approach has been well studied in the literature. The original work \citep{hartigan1987estimation} considers $\mathcal{C}$ being the collection of convex sets. The collection of ellipsoids is considered by \cite{nolan1991excess}. Convergence rates of the maximizer of (\ref{eq:EMF}) are investigated by \cite{tsybakov1997nonparametric} in a nonparametric setting for star-shaped sets and convex sets.

\item \textit{One-class classification.} Another type of algorithms aim to learn a nonparametric function $f:\mathbb{R}^d\rightarrow\mathbb{R}$, and the the confidence set is taken as $\{y\in\mathbb{R}^d:f(y)\geq 0\}$. This approach was pioneered by \cite{scholkopf2001estimating} and they model the function $f$ in a feature space by
\begin{equation}
f(y)=\text{sign}\left(w^T\Phi(y)-\rho\right),
\end{equation}
where $\Phi:\mathbb{R}^d\rightarrow\mathbb{R}^k$ is some feature mapping. The parameters $w$ and $\rho$ are solutions to the following optimization problem,
\begin{equation}
\max_{w,\rho,\xi}\frac{1}{2}\|w\|^2+\frac{1}{\lambda n}\sum_{i=1}^n\xi_i-\rho\quad\text{s.t. }w^T\Phi(Y_i)-\rho+\xi_i\geq 0,\label{eq:OSVM}
\end{equation}
where $\xi\in\mathbb{R}^n$ is a margin vector and $\lambda$ is determined by the confidence level. The optimization (\ref{eq:OSVM}) is known as the one-class support vector machine (SVM) in the literature, which is equivalent to another optimization problem called support vector data description (SVDD) \citep{tax2004support} using some particular feature mapping. Recasting learning minimum volume sets as solving classification is natural. The excess mass functional (\ref{eq:EMF}) already suggests that the problem is equivalent to testing between two measures, empirical distribution against volume (uniform). Formally, this connection was established by \cite{steinwart2005classification}. Unlike traditional classification, here all the data points are generated from the same distribution, which leads to the name ``one-class classification" in the literature. Compared with directly learning confidence sets through (\ref{eq:ERM}) or (\ref{eq:EMF}), the one-class classification perspective is more flexible, and can be easily combined with deep learning models \citep{ruff2018deep}.

\item \textit{Density estimation plug-in.} The population version of the excess mass functional is $P(C)-\lambda\vol(C)$, which is maximized by the density level set
$$\{y\in\mathbb{R}^d: p(y)\geq t\},$$
by Neyman--Pearson lemma, since the density function $p$ can be regarded as the likelihood ratio between $P$ and volume \citep{garcia2003level}. Thus, it is natural to replace $p$ by some density estimator $\widehat{p}$. The plug-in strategy has been considered by \cite{hyndman1996computing,park2010computable,Lei2013DistributionFreePS} among others. Under certain nonparametric setting, the optimality of the plug-in strategy can be proved \citep{rigollet2009optimal}.
\end{enumerate}



\cnote{our main results}

Our goal of the paper is to construct a confidence set with volume guarantee when the dimension is high. For this purpose, the only type of methods that are applicable in high-dimensional settings is based on one-class classification \citep{scholkopf2001estimating,tax2004support,ruff2018deep}. However, we are not aware of any polynomial-time algorithm that has provable volume guarantee in the literature.

Given some collection of sets $\mathcal{C}$, we will consider the notion of \textit{restricted volume optimality}, defined by
\begin{equation} \label{eq:intro:optC}
% \opt_k(P,1-\alpha) = \inf\left\{\vol(C):P(C)\geq 1-\alpha, C \in \calC_k \right\}.\label{eq:res-opt}
\opt_{\mathcal{C}}(P, 1-\alpha) = \inf\left\{\vol(C) : P(C) \geq 1-\alpha, C \in \mathcal{C} \right\},
\end{equation}
which is also known as the generalized quantile function \citep{einmahl1992generalized,polonik1997minimum}. The empirical version of (\ref{eq:intro:optC}) is given by $\opt_{\mathcal{C}}(\mathbb{P}_n, 1-\alpha)$. When $\mathcal{C}$ is the collection of all balls in $\mathbb{R}^d$, our main result of the paper is a polynomial-time algorithm that computes a $\widehat{C}\in\mathcal{C}$ that satisfies $\mathbb{P}_n(\widehat{C})\geq 1-\alpha$, and
\begin{equation}
\vol(\widehat{C})^{1/d}\leq (1+o_{\gamma}(1))\opt_{\mathcal{C}}(\mathbb{P}_n, 1-\alpha+\gamma)^{1/d}, \label{eq:main-ball}
\end{equation}
for some slack parameter $\gamma\in(0,\alpha)$. The factor $o_{\gamma}(1)$ is of order $O\left(\sqrt{\frac{\log\log d}{\gamma\log d}}\right)$.
The result (\ref{eq:main-ball}) is actually deterministic and holds for arbitrary data points $X_1,\cdots,X_n$. An analogous bound to (\ref{eq:main-ball}) also holds when $\mathbb{P}_n$ is replaced by $P$, by using standard concentration tools \citep{devroye2001combinatorial}. We emphasize that the multiplicative factor $(1+o_{\gamma}(1))$ is nontrivial for a polynomial-time algorithm in high dimension. Without the consideration of computational cost, one can directly solve (\ref{eq:ERM}), and the multiplicative factor is not needed. On the other hand, if one relaxes $(1+o_{\gamma}(1))$ to $O(1)$, it can be achieved by simply searching over $B(X_i,\|X_i-X_j\|)$ for all $1\leq i<j\leq n$.

Our main idea to achieve (\ref{eq:main-ball}) is based on the fact that all data points will be close to the mean as long as the variance is bounded in all directions. Moreover, we show that for arbitrary data sets, the number of dimensions where the variance is much larger than a typical value must be small. This allows us to solve the problem separately in a low-dimensional subspace of large variance and a high-dimensional subspace of small variance. The center of the ball can then be found by a grid search in the low-dimensional subspace, and by a robust mean estimator in the high-dimensional subspace.

Extensions of (\ref{eq:main-ball}) to the setting where $\mathcal{C}$ is the collection of unions of balls are also considered. Similar bounds are achieved in polynomial time by $\widehat{C}$ being a union of balls and by $\widehat{C}$ being a union of ellipsoids with an additional outer loop of greedy search. In particular, a factor $o_{\gamma}(1)$ much faster than $O\left(\sqrt{\frac{\log\log d}{\gamma\log d}}\right)$ can be proved for $\widehat{C}$ being a union of ellipsoids. On the other hand, we also show that the problem with $\mathcal{C}$ being the collection of unions of ellipsoids is in general computationally hard, given the hardness of learning with errors by \cite{bruna2021continuous}.

\cnote{applications of the problem}

Successfully learning a small confidence set has implications in many statistical inference tasks, ranging from estimation to hypothesis testing. We will summarize a few important applications below.
\begin{enumerate}
\item \textit{Robust estimation.} Suppose $\widehat{C}$ is a $(1-\alpha)$-level confidence set with some $\alpha$ close to one. It was suggested by \cite{sager1978estimation,sager1979iterative} that one can use some point in $\widehat{C}$ as a mode estimator. More generally, robust location and scatter estimation through learning minimum volume sets is advocated by \cite{rousseeuw1984least,rousseeuw1985multivariate}. Specifically, Rousseeuw first computes $\widehat{C}$ as the minimum volume ellipsoid (MVE), and then the center and the shape of the $\widehat{C}$ are used as a robust location estimator and a robust scatter matrix estimator. Other applications of MVE are discussed in \cite{van2009minimum}.

\item \textit{Testing unimodality.} The original motivation of \cite{hartigan1987estimation} in learning a minimum volume convex set is to test whether a distribution is unimodal. The paper suggested testing statistic $\sup_{\lambda}\sup_{C\in\mathcal{C}}E_{\lambda}(C)$ that maximizes the excess mass functional (\ref{eq:EMF}). The idea was further developed and generalized by \cite{muller1991excess,polonik1995measuring,cheng1998calibrating}.

\item \textit{Anomaly detection.} The problem of anomaly detection, also known as outlier or novelty detection, aims to find a set that is not typical. Given a distribution $P$ with density $p$, its anomaly region is $\{y\in\mathbb{R}^d:p(y)<t\}$, the complement of a density level set. Thus, the problem is mathematically equivalent to learning a confidence set. We refer the readers to \cite{chandola2009anomaly,ruff2021unifying} for comprehensive review of this area.

\item \textit{Goodness-of-fit.} Consider a null hypothesis $H_0:P=P_0$. Whether data is generated from $P_0$ can be determined by the value of $|\mathbb{P}_n(C)-P_0(C)|$ for some set $C$ that is informative. The idea of using minimum volume sets in the goodness-of-fit test was considered by \cite{polonik1999concentration}. In particular, let $\widehat{C}_{\alpha}$ (resp. $C_{\alpha}$) be a $(1-\alpha)$-level confidence set computed from $\mathbb{P}_n$ (resp. $P_0$). The statistic
$$\sup_{\alpha}\left(|\mathbb{P}_n(\widehat{C}_{\alpha})-P_0(\widehat{C}_{\alpha})|+|\mathbb{P}_n(C_{\alpha})-P_0(C_{\alpha})|\right)$$
was proposed and its asymptotic property was analyzed by \cite{polonik1999concentration}.

\item \textit{Conformal prediction.} The goal of conformal prediction \citep{gammerman1998learning,Vovkbook,angelopoulos2023survey} is to find a set $\widehat{C}$ that is trained from $Y_1,\cdots,Y_n\sim P$ such that $\mathbb{P}(Y_{n+1}\in \widehat{C})\geq 1-\alpha$ for an independent future observation $Y_{n+1}\sim P$. Minimum volume sets are natural candidates for conformal prediction to achieve finite sample coverage and volume optimality simultaneously. For example, conformalized density level sets have already been considered by \cite{Lei2013DistributionFreePS}. More generally, any minimum volume set learning algorithm, including our proposals in the paper, can be conformalized through the construction of nested systems \citep{gupta2022nested,ourwork2024}.
\end{enumerate}



\iffalse
related papers:

Learning minimum volume sets \citep{scott2005learning}: ERM, penalty, VC dimension

convex sets with minimum volume \citep{hartigan1987estimation}, with applications in testing unimodality/bimodality \citep{muller1991excess}: search for a second convex set, exterior to the first one. The paper also proposed the excess mass objective function $$\max_{C\in\mathcal{C}}P_n(C)-\alpha\text{vol}(C)$$

\cite{nolan1991excess} considered exactly Hartigan's setting and motivation, but study ellipoid

\cite{tsybakov1997nonparametric} did nonparametric theory for empirical excess mass maximization of Hartigan with star-shaped sets or convex sets

minimum volume ellipsoids covering a constant fraction of samples is considered by \cite{rousseeuw1984least,rousseeuw1985multivariate} to obtain robust location and scale estimators (i.e. the center and psd shape of the MVE are used as robust estimators), a review of MVE in robust estimation is given by \cite{van2009minimum}. Even earlier, \cite{sager1978estimation,sager1979iterative} use a point in a minimum volume set as an estimator of the mode of the distribution.





minimum volume set (density level set) can be used to do goodness-of-fit test of a given null distribution \citep{polonik1999concentration}

estimating support of (high-dimensional) distributions \citep{scholkopf2001estimating,scholkopfu2000sv}: find $f$ and the set is characterized by $\{f\geq 0\}$ with $P(f<0)\leq\alpha$. $f$ is modeled by kernel expansion in some feature space. In particular, they write $$f(x)=\text{sign}(w^T\Phi(x)-\rho),$$
where $\Phi(\cdot)$ is some feature map. The parameter $w$ and $\rho$ are solution to
$$\max_{w,\rho,\xi}\frac{1}{2}\|w\|^2+\frac{1}{\rho n}\sum_{i=1}^n\xi_i-\rho\quad\text{s.t. }w^T\Phi(x_i)-\rho+\xi_i\geq 0,$$
which is called one-class SVM. An equivalent form called Support Vector Data
Description is given by \cite{tax2004support}, and its deep version is given by \cite{ruff2018deep}.
Since the set $\{f>0\}$ is also $\{\text{sign}(f)=1\}$, one can reformulate the set estimation problem as a binary classification problem between $P$ and uniform \citep{steinwart2005classification}. Sometimes this is also called one-class classification.

The above view covers density level sets with $f=p$. Mathematical characterization of density level sets by \cite{garcia2003level}. Plug-in strategy studied by \cite{rigollet2009optimal}.

There is a whole area called anomaly detection, also known as novelty detection or outlier detection. One finds a set (usually with minimum volume) such that $P(C)\geq 1-\alpha$ or equivalently $P(C)\leq \alpha$. Small probability set is called anomaly or outlier. Literature either find $\{f>0\}$ or $\{\hat{p}>t\}$ with a density estimator \citep{park2010computable}. All methods can be incorporated with deep learning. A classical review is \cite{chandola2009anomaly}. A recent review is \cite{ruff2021unifying}.



applications:
robust estimation, goodness of fit test, anomaly detection, testing modality, conformal prediction
\fi

==> unused/smoothdensities.tex <==
\anote{Work in progress}

A kernel density estimate of the given probability density function is a density function of the form
\begin{equation}\label{eq:kde}
f_m(x) = \frac{1}{m}\sum_{j=1}^m K(x,z_m), \text{ where } K(x,z) = \frac{1}{\sqrt{2\pi} \cdot \rho} \exp\Big(- \frac{|x-z|^2}{2 \rho^2} \Big)
\end{equation}
is the Gaussian kernel function with standard deviation (bandwidth?) $\rho$, and $z_1, \dots, z_m \in \R$ (they are typically samples drawn from the distribution). We show that whenever we have a good kernel density estimator $\widetilde{f}_m(x)$ for the density $f(x)$, then there is a union of intervals that is a near volume-optimal confidence set for $\widetilde{f}_m$, and hence $f$.

\begin{theorem}\label{thm:smoothdensity}
Let $f: \R \to \R$ be an arbitrary density function and let $\widetilde{f}_m: \R \to \R$ be a Gaussian Kernel density estimator of the form $\widetilde{f}_m(x) = \sum_{j=1}^m K(x,z_m)$ %for some set of points $z_1, \dots, z_m \in \R$ and $K(z,\cdot)$ is the Gaussian kernel function due to a Gaussian centered at $z$ with variance (bandwidth?) at least $\rho^2$. 
%Suppose $\widetilde{f}_m$ is a KDE for $f$ 
that is $\eta$ close in $L_1$ distance i.e., $\norm{f - \widetilde{f}_m}_{L_1} \le \eta$. Then for any given $\tau \in (0,1)$ and $\eta \in (0,1)$, there exists intervals $I_1, \dots, I_m \subset \R$ such that 
\begin{equation}\label{eq:smoothdensity}
\int_{\cup_{\ell=1}^m I_\ell} f(x) \dx \ge \tau - \eta,~~ \text{ and }\qquad \sum_{\ell=1}^m \vol(I_\ell) ~\le \min_{\substack{S \subset \R \text{ s.t }\\ \int_S f(x) \dx \ge \tau }} \vol(S).   
\end{equation}

\end{theorem}
The above theorem gives a guarantee for any PDF that is well approximated by a Gaussian kernel density estimator in $L_1$ distance. By standard bounds for kernel density estimation, we can derive bounds for any smooth density function that is approximated by a bounded support distribution\anote{Need to state a general sounding corollary and modify wording appropriately.}. 

\begin{corollary}
Smooth densities with bounded support?
\end{corollary}


The above theorem is implied by the following lemma which shows  that for a mixture of $k$ Gaussians in $1$-dimension there is always an optimal volume confidence set that corresponds to a union of $k$ intervals.   
\begin{lemma}[Union of intervals for mixtures of Gaussians in $1$-dimension]\label{lem:mixofGaussians}
%Let $h: \R \to \R$ be an arbitrary density function and let $\widetilde{h}_m: \R \to \R$ be a Gaussian Kernel density estimator of the form $\widetilde{h}_m(x) = \sum_{j=1}^m K(x,z_m)$ for some set of points $z_1, \dots, z_m \in \R$ and $K(z,\cdot)$ is the Gaussian kernel function due to a Gaussian centered at $z$ with variance (bandwidth?) at least $\rho^2$. 
%Suppose $\widetilde{f}_m$ is a KDE for $f$ that is $\eta$ close in $L_1$ distance i.e., $\norm{f - \widetilde{f}_m}_{L_1} \le \eta$. 
Suppose $f:\R \to \R_+$ is the density for a mixture of $k$ Gaussians in $1$-dimension given by $\sum_{i=1}^k w_i ~\calN(\mu_i, \sigma_i^2)$. 
For any given $\tau \in (0,1)$ there exists a collection of intervals $I_1, \dots, I_k \subset \R$ such that 
\begin{equation}\label{eq:mixofGaussians}
\int_{\cup_{\ell=1}^k I_\ell} f(x) \dx \ge \tau,~~ \text{ and }\qquad \sum_{\ell=1}^k \vol(I_\ell) ~\le \min_{\substack{S \subset \R \text{ s.t }\\ \int_S f(x) \dx \ge \tau }} \vol(S).   
\end{equation}
\end{lemma}
Note that in \eqref{eq:smoothdensity} and \eqref{eq:mixofGaussians}, the volume optimal set $S$ can be an arbitrary subset of $\R$.  

The above statement does not make any assumptions on the separation between the means, or the variances of the Gaussians. When $\tau \to 0$, the intervals $I_1, I_2, \dots$ converge to the modes of the distribution. The proof of the lemma uses the following technical theorem of \cite{modes1d} which establishes  that for any mixture of $k$ Gaussians in 1-dimension has at most $k$ modes (local maxima of the density function).  
\begin{theorem}[Modes of mixture of $k$ Gaussians~\citep{modes1d}]\label{thm:modes1d}
For any mixture of $k$ Gaussians over $\R$ ($1$-dimension), the number of modes i.e., local maxima of the PDF is at most $k$. 
\end{theorem}


\begin{proof}[Proof of Lemma~\ref{lem:mixofGaussians}]
Using Theorem~\ref{thm:modes1d}, there are $k' \le k$ local maxima for the density function $f$. We will use $k'$ intervals and define the rest of the intervals to be empty. Suppose $u_1 \le u_2 \le  \dots \le u_{k'} \in \R$ are the local maxima of $f$. The density $f(x)$ is differentiable, and its local minima and local maxima have to alternate. Hence there are exactly $k'-1$ local minima, denoted by $\ell_1, \ell_2, \dots, \ell_{k'-1}$ with $\ell_j \in [u_{j}, u_{j+1}]$ for all $ j \in \{1,2,\dots, k'-1\}$. (Note that there are no local minima less than $u_1$ or greater than $u_{k'}$ since $f(x) \to 0$ as $x \to \pm \infty$). For notational convenience let $\ell_0 = -\infty, \ell_{k'}=\infty$. Let $S^* \subset \R$ be an optimal solution to the problem on $\min_{S \subset \R} \vol(S) \text{ s.t. } \int_S f(x) \dx \ge \tau$.

%The lemma is established using the following claim. 
%\begin{claim}
%To establish the claim, 
We now show that there exists intervals $I_1, \dots, I_{k'}$ such that $\forall j \in [k'], I_{k'} \subseteq [\ell_{j-1}, \ell_{j}]$ and $u_j \in I_{j}$ that is optimal for \eqref{eq:mixofGaussians} i.e., \\
\begin{equation}(i) ~~\sum_{j=1}^{k'} \vol(I_j) \le \vol(S^*), \text{ and } (ii)~~ \int_{I_1 \cup \dots \cup I_{k'}} f(x) \dx \ge \tau. \label{eq:claim:smooth}
\end{equation}  

Consider $S_j = S^* \cap [\ell_{j-1}, \ell_j]$ for all $j \in [k']$. Next we observe for all $j \in \{1,\dots, k'-1\}$, $f$ is monotonically increasing in the interval $[\ell_{j-1}, u_{j}]$ and $f$ is monotonically decreasing in the intervals $[u_j, \ell_j]$, with a local maximum at $u_j$. Hence if $S_j$ comprises multiple disjoint intervals within $[\ell_{j-1}, \ell_{j}]$, we can pick one interval with the same volume within $[\ell_{j-1}, \ell_j]$ that also includes $u_j$ and covers at least as much probability mass. This establishes \eqref{eq:claim:smooth}, and hence the lemma.   

%\end{claim}
%Once we have the above claim, the lemma follows by observing that the 

\end{proof}

\paragraph{Approximate Optimality when the Kernel Density methods are efficient}

We now show that our method based on unions of intervals are competitive against any method that is outputs a level set of a (Gaussian) kernel density estimator (KDE) as in \eqref{eq:kde} with small $L_1$ error. 
\anote{What follows is based on what guarantee we get in 1-D in terms of sample complexity etc. for our method. I wasn't sure if there's a clean statement that can be used as such. This should use VC-dimension bounds for unions of $k$ intervals. }
In what follows, we will use $s(k, \alpha, \gamma)$ to denote the number of samples needed by the methods of the previous section (e.g., Section~\ref{sec:1d:dp}) so that on input $s(k,\alpha, \gamma)$ samples from $\mathcal{D}$ it outputs sets $S_1, \dots, S_k \subset \R$ such that with probability at least $0.99$,
\begin{equation}\label{eq:1d:statguarantee}
\Pr_{\mathcal{D}} \Big[S_1 \cup \dots \cup S_k \Big] \ge 1-\alpha - \gamma, \text{ and } \vol\big(\cup_{i =1}^k S_i\big) \le \min_{\substack{C_1, \dots, C_k \subset \R,\\ \Pr_{\mathcal{D}}[S_1 \cup \dots \cup S_k] \ge 1-\alpha}} \vol\big(C_1 \cup \dots \cup C_k \big).
\end{equation}
\anote{We need to write down this guarantee in an earlier section, but my guess is that $s(k,\alpha,\gamma) = O(k \log k/ \gamma^2)$ or even $O(k/\gamma^2)$ suffices (and shouldn't depend on $\alpha$). }

\begin{proposition}\label{prop:comparisontokde}
Consider a distribution $\mathcal{D}$ over $\R$ with density $f$ and suppose there is a level set $C^* \subset \R$ of a (Gaussian) kernel density estimator (KDE) $\widetilde{f}_m$ constructed from $m$ samples of $\mathcal{D}$ as in \eqref{eq:kde}
that is $\eta$ close in $L_1$ distance i.e., $\norm{f - \widetilde{f}_m}_{1} \le \eta$, and suppose $C^*$ has coverage $\Pr_{\mathcal{D}}[C^*] \ge 1-\alpha$. Then for any $\eta>0$, our method with $N=s(m,\alpha+2\eta,\eta)$ samples and $m$ intervals \anote{I guess this should be around $O(m/\eta^2)$ or $O(m\log m/\eta^2)$ should be easy?},  finds intervals $I_1, \dots, I_m \subset \R$ with probability at least $0.99$ such that 
\begin{equation}\label{eq:smoothdensity}
\Pr_{\mathcal{D}}[\cup_{\ell=1}^m I_\ell] \ge 1-\alpha - 4\eta,~~ \text{ and }\qquad \sum_{\ell=1}^m \vol(I_\ell) ~\le \vol(C^*).   
\end{equation}
\end{proposition}
Note that the work of \citet{Lei2013DistributionFreePS} assumes a KDE with a $L_\infty$ guarantee. For distributions whose effective support is bounded, this also implies the form of $L_1$ error assumption that we need. 
\anote{We can potentially replace Theorem~\ref{thm:smoothdensity} with the above proposition.}
\begin{proof}
The KDE $\widetilde{f}_m$ corresponds to the density of a mixture of (at most) $m$ Gaussians. Also $\Pr_{\mathcal{D}}(C^*) \ge 1-\alpha - \eta $. From Lemma~\ref{lem:mixofGaussians} applied with $\widetilde{f}_m$ and coverage $\tau = 1-\alpha - \eta$, we conclude that there exists intervals $I^*_1, I^*_2, \dots, I^*_m$ such that 
\begin{align*}\sum_{\ell=1}^k \vol(I^*_\ell) ~\le \vol(C^*), ~\text{ and } \int_{\cup_{\ell=1}^m I^*_\ell} \widetilde{f}_m(x)\dx \ge 1-\alpha-\eta, \\
 \implies ~~~\Pr_{\mathcal{D}}\Big[\cup_{\ell=1}^m I^*_\ell\Big] \ge \int_{\cup_{\ell=1}^m I^*_\ell} \widetilde{f}_m(x)\dx -\eta \ge 1-\alpha-2\eta, 
\end{align*}
since the $L_1$ error of $\widetilde{f}_m$ is at most $\eta$. By running our method with number of intervals $k=m$, $\gamma = 2\eta$ and $\epsilon=\eta$, and with $N=s(m,\alpha+2\eta, \eta)$ samples, we find intervals $I_1, \dots, I_m$ satisfying
$$\Pr_{\mathcal{D}}\Big[\cup_{\ell=1}^m I_\ell \Big] \ge 1-\alpha - 4\eta, ~~\text{ and } \sum_{\ell=1}^m \vol(I_\ell) \le \sum_{\ell=1}^m \vol(I^*_\ell) \le \vol(C^*). $$
This concludes the proof.
\end{proof}

==> unused/unused_1d.tex <==
\section{Basics}

Given a continuous distribution $P$ with density function $p$ on $\mathbb{R}^d$, conformal prediction outputs a set
$$\{q>t\}=\{x\in\mathbb{R}^d:q(x)>t\},$$
so that this set has probability at least $1-\alpha$. We will investigate conditions on $q$ and $t$ so that the volume of this set is as small as possible.

We define
$$\text{Opt}(p,1-\alpha)=\inf\{\vol(C):P(C)\geq 1-\alpha\}.$$
To achieve volume optimality, define
$$t(p,1-\alpha)=\inf\{t\geq 0:P(p>t)\leq 1-\alpha\}.$$
By definition, we must have
$$P(p>t(p,1-\alpha))\leq 1-\alpha,$$
and
$$P(p\geq t(p,1-\alpha))\geq 1-\alpha.$$
Therefore, any volume-optimal set must have the form
$$\{p>t(p,1-\alpha)\}\cup D,$$
where $D\subset\{p=t(p,1-\alpha)\}$, such that $P(D)=1-\alpha-P(p=t(p,1-\alpha))$.

The first question we will investigate is the condition on $q$ such that $\{q>t\}$ is volume optimal. The choice $q=p$ would not work, considering the example of uniform distribution.

\begin{theorem}
Consider the function
$$q(x)=\begin{cases}B
f(x) & x\in D_1=\{p>t(p,1-\alpha)\} \\
g(x) & x\in D_2=\{p=t(p,1-\alpha)\} \\
h(x) & x\in D_3=\{0<p<t(p,1-\alpha)\} \\
z(x) & x\in D_4=\{p=0\}
\end{cases}$$
that satisfies the following properties.
\begin{enumerate}
\item For any $x\in D_1$ and $x'\in D_2$, $f(x)>g(x')$.
\item For any $x\in D_2$ and $x'\in D_3$, $g(x)>h(x')$.
\item For any $x\in D_3$, $h(x)>\sup\{z(x):x\in D_4\}$.
\item For any $t\in \{g(x):x\in D_3\}$, $P(g=t)=0$.
\end{enumerate}
Then, for
$$t(q,1-\alpha)=\inf\{t\geq 0:P(q>t)\leq 1-\alpha\},$$
we must have both $P(q>t(q,1-\alpha))=1-\alpha$ and $\vol(q>t(q,1-\alpha))=\opt(p,1-\alpha)$.
\end{theorem}
\begin{proof}
For any $t>\sup\{g(x):x\in D_2\}$, since $\{q>t\}=\{f>t,p>t(p,1-\alpha)\}$, we must have $P(q>t)\leq P(p>t(p,1-\alpha))\leq 1-\alpha$. By the definition of $t(q,1-\alpha)$, we have $t(q,1-\alpha)\leq t$ for all $t>\sup\{g(x):x\in D_2\}$. This implies $t(q,1-\alpha)\leq \sup\{g(x):x\in D_2\}$. 
Moreover, we also have $t(q,1-\alpha)\geq \sup\{z(x):x\in D_4\}$, since otherwise $t(q,1-\alpha)<\sup\{z(x):x\in D_4\}$ implies $\{q>t(q,1-\alpha)\}\supset\{p>0\}$, but $P(q>t(q,1-\alpha))\geq P(p>0)=1$ contradicts the definition of $t(q,1-\alpha)$.
Therefore, we could write
$$\{q>t(q,1-\alpha)\}=\{p>t(p,1-\alpha)\}\cup \bar{D}_2\cup\bar{D}_3,$$
where $\bar{D}_2=\{g>t(q,1-\alpha),p=t(p,1-\alpha)\}\subset D_2$ and $\bar{D}_3=\{h>t(q,1-\alpha),p<t(p,1-\alpha)\}\subset D_3$.

\textit{Case 1.} Suppose $t(q,1-\alpha)<\sup\{h(x):x\in D_3\}$. Then,
$$\{q>t(q,1-\alpha)\}=\{p\geq t(p,1-\alpha)\}\cup \bar{D}_3.$$
By $P(q>t(q,1-\alpha))\leq 1-\alpha$ and $P(p\geq t(p,1-\alpha))\geq 1-\alpha$, we must have $P(\bar{D}_3)=0$. Since $\bar{D}_3\subset\{p>0\}$, we also have $\vol(\bar{D}_3)=0$.

\text{Case 2.} Suppose $t(q,1-\alpha)\geq \sup\{h(x):x\in D_3\}$. Then, $\bar{D}_3=\varnothing$, which also implies $P(\bar{D}_3)=0$ and $\vol(\bar{D}_3)=0$.

To summarize, in both cases, we get $P(\bar{D}_3)=0$ and $\vol(\bar{D}_3)=0$. We then have
$$P(q>t(q,1-\alpha))=P(p>t(p,1-\alpha))+P(\bar{D}_2),$$
and
$$\vol(q>t(q,1-\alpha))=\vol(p>t(p,1-\alpha))+\vol(\bar{D}_2).$$
By repeating the arguments above, we also have
$$P(q>t)=P(p>t(p,1-\alpha))+P(g>t,p=t(p,1-\alpha)),$$
and
$$\vol(q>t)=\vol(p>t(p,1-\alpha))+\vol(g>t,p=t(p,1-\alpha)),$$
for any $t$ such that $\sup\{z(x):x\in D_4\}\leq t\leq \sup\{g(x):x\in D_2\}$. Thus, we can write
$$t(q,1-\alpha)=\inf\{t:\sup\{z(x):x\in D_4\}\leq t\leq \sup\{g(x):x\in D_2\},P(p>t(p,1-\alpha))+P(g>t,p=t(p,1-\alpha)\leq 1-\alpha)\}.$$
The condition $P(g=t)=0$ implies $P(q>t(q,1-\alpha))=P(p>t(p,1-\alpha))+P(g>t(q,1-\alpha),p=t(p,1-\alpha))=1-\alpha$. The volume optimality is a consequence of the fact that $\bar{D}_2$ has constant density.
\end{proof}

The next result characterizes approximate optimality.

\begin{theorem}\label{thm:approx-opt}
Consider $\epsilon<\alpha$ and the function
$$q(x)=\begin{cases}
f(x) & x\in D_1=\{p>t(p,1-\alpha+\epsilon)\} \\
g(x) & x\in D_2=\{p=t(p,1-\alpha+\epsilon)\} \\
h(x) & x\in D_3=\{0<p<t(p,1-\alpha+\epsilon)\} \\
z(x) & x\in D_4=\{p=0\}
\end{cases}$$
that satisfies the following properties.
\begin{enumerate}
\item For any $x\in D_1$ and $x'\in D_2$, $f(x)\geq g(x')$.
\item For any $x\in D_2$ and $x'\in D_3$, $g(x)\geq h(x')$.
\item For any $x\in D_3$, $h(x)\geq \sup\{z(x):x\in D_4\}$.
\item For any $t\in [\inf\{g(x):x\in D_2\},\sup\{g(x):x\in D_2\}]$, $P(q=t)\leq \epsilon$.
\end{enumerate}
Then, for $t(q,1-\alpha+\epsilon)=\inf\{t\geq 0: P(q>t)\leq 1-\alpha+\epsilon\}$, we must have both $P(q>t(q,1-\alpha+\epsilon))\geq 1-\alpha$ and $\vol(q>t(q,1-\alpha+\epsilon))\leq \text{Opt}(p,1-\alpha+\epsilon)$.
\end{theorem}
\begin{proof}
For any $t>\sup\{g(x):x\in D_2\}$, since $\{q>t\}=\{f>t,p>t(p,1-\alpha+\epsilon)\}$, we must have $P(q>t)\leq P(p>t(p,1-\alpha+\epsilon))\leq 1-\alpha+\epsilon$. By the definition of $t(q,1-\alpha)$, we have $t(q,1-\alpha+\epsilon)\leq t$ for all $t>\sup\{g(x):x\in D_2\}$. This implies $t(q,1-\alpha+\epsilon)\leq \sup\{g(x):x\in D_2\}$. 
Moreover, we also have $t(q,1-\alpha+\epsilon)\geq \sup\{z(x):x\in D_4\}$, since otherwise $t(q,1-\alpha+\epsilon)<\sup\{z(x):x\in D_4\}$ implies $\{q>t(q,1-\alpha+\epsilon)\}\supset\{p>0\}$, but $P(q>t(q,1-\alpha+\epsilon))\geq P(p>0)=1$ contradicts the definition of $t(q,1-\alpha+\epsilon)$. To summarize, we have shown that
$$\sup\{z(x):x\in D_4\}\leq t(q,1-\alpha+\epsilon)\leq \sup\{g(x):x\in D_2\}.$$

Let us write $\mathcal{T}=[\sup\{z(x):x\in D_4\},\sup\{g(x):x\in D_2\}]$ For any $t\in\mathcal{T}$ such that $P(q>t)\leq 1-\alpha+\epsilon$, we can write
$$\{q>t\}=D_1(t)\cup D_2(t)\cup D_3(t),$$
where $D_1(t)=\{f>t,p>t(p,1-\alpha+\epsilon)\}\subset D_1$, $D_2(t)=\{g>t, p=t(p,1-\alpha+\epsilon)\}\subset D_2$ and $D_3(t)=\{h>t, 0<p<t(p,1-\alpha+\epsilon)\}\subset D_3$. Suppose $t<\sup\{h(x):x\in D_3\}$. Then $D_1(t)=\{p<t(p,1-\alpha+\epsilon)\}$ and  $D_2(t)=\{p=t(p,1-\alpha+\epsilon)\}$, and thus $\{q>t\}=\{p\geq t(p,1-\alpha+\epsilon)\}\cup D_3(t)$. Since $P(q>t)\leq 1-\alpha+\epsilon$ and $P(p\geq t(p,1-\alpha+\epsilon))\geq 1-\alpha+\epsilon$, we must have $P(D_3(t))=0$. The fact that $D_3(t)\subset\{p>0\}$ also implies $\vol(D_3(t))=0$. Suppose $t\geq \sup\{h(x):x\in D_3\}$. Then, $D_3(t)=\varnothing$, which still implies $P(D_3(t))=0$ and $\vol(D_3(t))=0$.

Hence, for any $t\in\mathcal{T}$ such that $P(q>t)\leq 1-\alpha+\epsilon$, we must have
$$P(q>t)=P(D_1(t))+P(D_2(t)),$$
and
$$\vol(q>t)=\vol(D_1(t))+\vol(D_2(t)).$$
We have already shown that $t(q,1-\alpha+\epsilon)\in\mathcal{T}$. This implies the above two identities also hold for $t=t(q,1-\alpha+\epsilon)$.

\textit{Volume of $\{q>t(q,1-\alpha+\epsilon)\}$.} Suppose $D_2(t(q,1-\alpha+\epsilon))=\varnothing$. Then,
$$\vol(q>t(q,1-\alpha+\epsilon))\leq \vol(p>t(p,1-\alpha+\epsilon))\leq \text{Opt}(t,1-\alpha+\epsilon).$$
Suppose $D_2(t(q,1-\alpha+\epsilon))\neq\varnothing$. Then, $\{q>t(q,1-\alpha+\epsilon)\}=\{p>t(p,1-\alpha+\epsilon)\}\cup D_2(t(q,1-\alpha+\epsilon))$, which is in the form of volume optimal set, and therefore $\vol(q>t(q,1-\alpha+\epsilon))\leq\text{Opt}(p,1-\alpha+\epsilon)$.

\textit{Coverage of $\{q>t(q,1-\alpha+\epsilon)\}$.} Suppose $t(q,1-\alpha+\epsilon)<\inf\{g(x):x\in D_2\}$. We have $P(q>t(q,1-\alpha+\epsilon))\geq P(p\geq t(p,1-\alpha+\epsilon))\geq 1-\alpha+\epsilon\geq 1-\alpha$. Otherwise, we must have $t(q,1-\alpha+\epsilon)\in[\inf\{g(x):x\in D_2\},\sup\{g(x):x\in D_2\}]$, so that
$$t(q,1-\alpha+\epsilon)=\inf\{t\in[\inf\{g(x):x\in D_2\},\sup\{g(x):x\in D_2\}]:P(q>t)\leq 1-\alpha+\epsilon\}.$$
We know that $P(q=t)\leq\epsilon$ in this range, and therefore $P(q>t(q,1-\alpha+\epsilon))\geq 1-\alpha$.
\end{proof}

Below, we give an explicit construction of $q$ that satisfies the conditions in the above theorem. Define
$$S_1\in\argmin\{\vol(S):P(S)=\epsilon\}.$$
For $t=2,\cdots,T=1/\epsilon$, define
$$S_t\in\argmin\{\vol(S):P(S)=\epsilon, S\cap (S_1\cup\cdots S_{t-1})=\varnothing\}.$$
Then, the function
$$q(x)=\sum_{t=1}^T\mathbb{I}\{x\in S_1\cup\cdots\cup S_t\}$$
satisfies approximate the conditions of volume optimality.

Let us state the following result, which is more convenient (and more restrictive) than the theorem above.

\begin{corollary}\label{cor:q-population}
Suppose $q$ satisfies the following properties.
\begin{enumerate}
\item If $p(x)>p(x')$, then $q(x)\geq q(x')$.
\item For any $t\in\mathbb{R}$, $P(q=t)\leq\epsilon$.
\end{enumerate}
Then, we have both $P(q>t(q,1-\alpha+\epsilon))\geq 1-\alpha$ and $\vol(q>t(q,1-\alpha+\epsilon))\leq \text{Opt}(p,1-\alpha+\epsilon)$.
\end{corollary}

\subsection{Error of Estimating $t(q,\cdot)$}

Suppose $q$ is a function that satisfies
\begin{enumerate}
\item For any $x,x'\in\mathbb{R}^d$ such that $p(x)> p(x')$, we have $q(x)\geq q(x')$.
\item For any $t$, $P(q=t)\leq \epsilon$.
\end{enumerate}
In other words, the conditions of Theorem \ref{thm:approx-opt} are satisfied for all $\alpha>\epsilon$. An immediate consequence is that for any $t$,
$$\text{vol}(q>t)\leq \text{Opt}(p,P(q>t)+\epsilon).$$
Define $\delta_n$ so that
$$\sup_t\left|\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(X_i)>t\}-P(q>t)\right|\leq\delta_n,$$
with high probability. For example, one could take $\delta_n\asymp n^{-1/2}$ according to DKW inequality. With this quantity, we immediately have
$$\sup_t\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(X_i)=t\}\leq \epsilon+2\delta_n.$$

Define
$$\hat{t}(q,1-\alpha)=\inf\left\{t:\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(X_i)>t\}\leq 1-\alpha\right\}.$$
It is not hard to see $\hat{t}(q,1-\alpha)=q_{(n\alpha)}$, where $q_{(1)}\leq\cdots\leq q_{(n)}$ are order statistics of $q(X_1),\cdots,q(X_n)$. We will consider the property of the set
$$\{q>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)\}.$$
By the definition of $\hat{t}(q,1-\alpha+\epsilon+2\delta_n)$ and the property of $q$, we have
$$1-\alpha\leq \frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(X_i)>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)\}\leq 1-\alpha+\epsilon+2\delta_n.$$
By exchangeability of $q(X_1),\cdots,q(X_n),q(X_{n+1})$, we have
$$\mathbb{E}\int_{q>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)}p(x)dx=P\left(q(X_{n+1})>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)\right)\geq 1-\alpha.$$
We can bound its volume by
\begin{eqnarray*}
\vol(q>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)) &\leq& \text{Opt}\left(p,\int_{q>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)}p +\epsilon\right) \\
&\leq& \text{Opt}\left(p,\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(X_i)>\hat{t}(q,1-\alpha+\epsilon+2\delta_n)\}+\epsilon+\delta_n\right) \\
&\leq& \text{Opt}(p,1-\alpha + 2\epsilon +3\delta_n).
\end{eqnarray*}
In summary, the error is given by $O(\epsilon+n^{-1/2})$ for estimating the threshold via quantile.

\subsection{Error of Estimating $q$}

Could we relax Condition 1 in Corollary \ref{cor:q-population}? Below is one version that may work.

\begin{theorem}
Suppose $q$ satisfies the following properties.
\begin{enumerate}
\item $\sup_xP(q(X)<q(x),p(X)\geq p(x))\leq \epsilon_1$.
\item $\sup_tP(q=t)\leq \epsilon_2$.
Then, for $C=\{q>t(q,1-\alpha+\epsilon_2)\}$, we have both $P(C)\geq 1-\alpha$ and $\vol(C)\leq\text{Opt}(p,1-\alpha+\epsilon_1+\epsilon_2)$.
\end{enumerate}
\end{theorem}
\begin{proof}[Proof Sketch]
The coverage property $P(C)\geq 1-\alpha$ is guaranteed by the construction and Condition 2. To bound the volume, we observe that
$$C=\{x:P(q(X)<q(x))\geq\alpha-\epsilon_2\}.$$
Since
\begin{eqnarray*}
C &=& \{x:P(q(X)<q(x),p(X)<p(x))+P(q(X)<q(x),p(X)\geq p(x))\geq\alpha-\epsilon_2\} \\
&\subset& \{x:P(q(X)<q(x),p(X)<p(x))\geq \alpha-\epsilon_1-\epsilon_2\} \\
&\subset& \{x:P(p(X)<p(x))\geq \alpha-\epsilon_1-\epsilon_2\}.
\end{eqnarray*}
Therefore, $\vol(C)\leq \text{Opt}(p,1-\alpha+\epsilon_1+\epsilon_2)$.
\end{proof}

Could we relax $\sup_xP(q(X)<q(x),p(X)\geq p(x))\leq \epsilon_1$ to $P(q(X)<q(X'),p(X)\geq p(X'))\leq \epsilon_1$? Here, $X$ and $X'$ are independent copies from $P$.

Let us consider the following construction of $q$ that satisfies the conditions of the theorem. 
\begin{lemma}
Consider $q(x)=\sum_{t=1}^T\mathbb{I}\{x\in C_t\}$ with nested sets $C_1\subset C_2\subset\cdots \subset C_T$ satisfying the following properties.
\begin{enumerate}
\item $P(C_t)=\frac{t}{T}$ for each $t\in[T]$.
\item For each $t\in[T]$, there exists some
$$S\in\argmin\left\{\vol(S):P(S)=\frac{t}{T}+\epsilon\right\},$$
such that $C_t\subset S$.
\end{enumerate}
Then, we must have $\sup_xP(q(X)<q(x),p(X)> p(x))\leq \epsilon$ and $\sup_tP(q=t)\leq \frac{1}{T}$.
\end{lemma}
\begin{proof}
We only need to prove the first conclusion. Observe that $\{C_1,C_2\backslash C_1,\cdots,C_T\backslash C_{T-1}\}$ forms a partition. There must exists some $t\in[T]$, such that $x\in C_t\backslash C_{t-1}$. By the definition of $q$, the event $q(X)<q(x)$ is equivalent to $X\in C_t^c$. Moreover, we know that $x\in C_t\backslash C_{t-1}\subset C_t\subset S$ for some $S\in\argmin\left\{\vol(S):P(S)=\frac{t}{T}+\epsilon\right\}$. Then, we know that $p(X)>p(x)$ implies $X\in S$. Finally, $P(q(X)<q(x),p(X)> p(x))\leq P(X\in C_t^c,X\in S)=P(S)-P(C^t)=\epsilon$.
\end{proof}

Notice the gap between $\sup_xP(q(X)<q(x),p(X)> p(x))\leq \epsilon$ and $\sup_xP(q(X)<q(x),p(X)\geq p(x))\leq \epsilon$, which we shall try to fix later.

\begin{theorem}
Suppose $q$ satisfies the following properties.
\begin{enumerate}
\item $\sup_xP(q(X)<q(x),p(X) > p(x))\leq \epsilon_1$.
\item $\sup_tP(q=t)\leq \epsilon_2$.
\end{enumerate}
Then, for $C=\{q>t(q,1-\alpha+\epsilon_2)\}$, we have both $P(C)\geq 1-\alpha$ and $\vol(C)\leq\text{Opt}(p,1-\alpha+\epsilon_1+2\epsilon_2)$.
\end{theorem}

\begin{proof}
    We have
    $$
    C \subset C'= \{x:P(q(X)<q(x),p(X)\leq p(x))\geq \alpha-\epsilon_1-\epsilon_2\}.
    $$
    Let $t_1 = t(p,1-\alpha+\varepsilon_1 + \varepsilon_2)$. Note that 
    $$
    C' \subset \{x: p(x) > t_1\} + \{x: P(q(X)<q(x),p(X)\leq p(x))\geq \alpha-\epsilon_1-\epsilon_2 , p(x) = t_1\}.
    $$
    Suppose $S$ is an optimal solution that covers $1-\alpha + \varepsilon_1 + 2\varepsilon_2$ probability mass of $p$. Let $D = S \setminus \{x: p(x) > t_1\}$. If $\vol(\{x: p(x) = t_1\}) \leq \vol(D)$, then we have $\vol(C') \leq \opt(p,1-\alpha+\varepsilon_1 + 2\varepsilon_2)$. 
    Suppose $\vol(\{x: p(x) = t_1\}) > \vol(D)$.
    Since $\sup_t P(q = t) \leq \varepsilon_2$, we have
    $$
    \vol(\{x: P(q(X)<q(x),p(X)\leq t_1)\geq \alpha-\epsilon_1-\epsilon_2 , p(x) = t_1\})\leq \vol(D).
    $$
\end{proof}

{\color{red}After a second thought, I feel that the condition on $P(q(X)<q(X'),p(X)\geq p(X'))$ is not the right way to characterize the closeness between $p$ and $q$. Consider the example with $p(x)\propto (1-\delta x)\mathbb{I}\{x\in[0,1]\}$ and $q(x)=x$. It is clear that $P(q(X)<q(X'),p(X)\geq p(X'))=1$ for arbitrarily small $\delta$. However, it is not hard to check that
$$\vol(q>t(q,1-\alpha))\leq \text{Opt}(p,1-\alpha+O(\delta)).$$}

\subsection{Conformal Prediction with Volume Optimality}

Consider independent observations $X_1,\cdots,X_n,X_{n+1}\sim P$, where $P$ is assumed to be some probability distribution on $\mathbb{R}$. The joint distribution of $X_1,\cdots,X_n,X_{n+1}$ is denoted as the product measure $P^{n+1}$. Conformal prediction outputs a data-dependent set $\widehat{C}(X_1,\cdots,X_n)$ such that
$$P^{n+1}(X_{n+1}\in \widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha.$$
Let $\lambda$ denote the Lebesgue measure on $\mathbb{R}$. The length/volume of $\widehat{C}(X_1,\cdots,X_n)$ is measured by $\lambda(\widehat{C}(X_1,\cdots,X_n))$, which is a random variable depending on $X_1,\cdots,X_n$. In this section, we discuss how to control the expected volume $P^n\lambda(\widehat{C}(X_1,\cdots,X_n))$,
where we use $P^n$ to stand for the expectation operator under the distribution $P^n$. We say $\widehat{C}(X_1,\cdots,X_n)$ is $\epsilon$-optimal if
$$P^n\lambda(\widehat{C}(X_1,\cdots,X_n))\leq \text{Opt}(p,1-\alpha+\epsilon),$$
where $p=\frac{dP}{d\lambda}$. The following result shows that distribution-free $\epsilon$-optimality is impossible.

\begin{theorem}\label{thm:impossibility}
Suppose $P^{n+1}(X_{n+1}\in \widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha$ for all $P$. Then, for any $\epsilon<\alpha$, there exists some $P$, such that
$P^n\lambda(\widehat{C}(X_1,\cdots,X_n))\geq \text{Opt}(p,1-\alpha+\epsilon)$.
\end{theorem}

The result shows that there is no $\epsilon$ such that a non-trivial volume bound can hold uniformly over all distributions. The proof of the theorem relies on the following lemma.

\begin{lemma}\label{lem:tv}
For any $\delta,\epsilon>0$ and any integer $n>0$, there exists some distribution $\Pi$ supported on
$$\mathcal{P}_{\epsilon}=\left\{P:\text{supp}(P)\subset[0,1],\TV(P,\lambda)\geq 1-\epsilon\right\},$$
such that $\TV\left(\lambda^n,\int P^n d\Pi\right)\leq \delta$. Here, we use $\lambda=\text{Uniform}([0,1])$ with a slight abuse of notation.
\end{lemma}
\begin{proof}
For $j\in[m]$, define $A_j=\left[\frac{j-1}{m},\frac{j}{m}\right)$. For any $Z\in\{0,1\}^m$, define the density function
$$p_Z(x)=\frac{\sum_{j=1}^mZ_j\mathbb{I}\{x\in A_j\}}{\frac{1}{m}\sum_{j=1}^mZ_j},$$
and the corresponding distribution is denoted by $P_Z$. Define
$$\mathcal{Z}=\left\{Z\in\{0,1\}^m:\left|\frac{1}{m}\sum_{j=1}^mZ_j-\beta\right|\leq\left(\frac{\beta}{m}\right)^{1/3}\right\}.$$
Define $\Pi$ to be the distribution $\tilde{\Pi}=\otimes_{j=1}^m\text{Bernoulli}(\beta)$ conditioning on $\mathcal{Z}$. That is, $\Pi(B)=\frac{\tilde{\Pi}(B\cap\mathcal{Z})}{\tilde{\Pi}(\mathcal{Z})}$. The last notation we need is $A_Z=\cup_{j:Z_j=1}A_j$, so that $p_Z(x)=\frac{1}{\frac{1}{m}\sum_{j=1}^mZ_j}\mathbb{I}\{x\in A_Z\}$.

For any $Z\in\mathcal{Z}$, $\TV(P_Z,\lambda)\geq \lambda(A_Z^c)=1-\frac{1}{m}\sum_{j=1}^mZ_j\geq 1-\beta-\left(\frac{\beta}{m}\right)^{1/3}$. Therefore, as long as $\beta+\left(\frac{\beta}{m}\right)^{1/3}\leq\epsilon$, we have $P_Z\in\mathcal{P}_{\epsilon}$ for all $Z\in\mathcal{Z}$.

We bound $\TV(\lambda^n,\int P_Z^n d\Pi(Z))$ by chi-squared divergence,
\begin{eqnarray*}
\frac{1}{2}\TV\left(\lambda^n,\int P_Z^n d\Pi(Z)\right)^2 &\leq& \int \frac{\left(\int P_Z^n d\Pi(Z)\right)^2}{\lambda^n}-1 \\
&=& \mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \Pi}\left(\int p_Z(x)p_{Z'}(x)dx\right)^n-1 \\
&=& \mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \Pi}\left(\frac{1}{\frac{1}{m}\sum_{j=1}^mZ_j}\frac{1}{\frac{1}{m}\sum_{j=1}^mZ'_j}\frac{1}{m}\sum_{j=1}^mZ_jZ_j'\right)^n-1 \\
&\leq& \left(\beta-\left(\frac{\beta}{m}\right)^{1/3}\right)^{-2n}\mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \Pi}\left(\frac{1}{m}\sum_{j=1}^mZ_jZ_j'\right)^n-1 \\
&=& \left(\beta-\left(\frac{\beta}{m}\right)^{1/3}\right)^{-2n}\frac{\mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \tilde{\Pi}}\left(\frac{1}{m}\sum_{j=1}^mZ_jZ_j'\right)^n\mathbb{I}\{Z\in\mathcal{Z}\}\mathbb{I}\{Z'\in\mathcal{Z}\}}{\tilde{\Pi}(Z\in \mathcal{Z})^2}-1 \\
&\leq& \left(\beta-\left(\frac{\beta}{m}\right)^{1/3}\right)^{-2n}\left(1-\left(\frac{\beta}{m}\right)^{1/3}\right)^{-2}\mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \tilde{\Pi}}\left(\frac{1}{m}\sum_{j=1}^mZ_jZ_j'\right)^n-1.
\end{eqnarray*}
Since
\begin{eqnarray*}
&& \mathbb{E}_{Z,Z'\stackrel{iid}{\sim} \tilde{\Pi}}\left(\frac{1}{m}\sum_{j=1}^mZ_jZ_j'\right)^n \\
&\leq& \left(\beta^2 + \left(\frac{\beta^2}{m}\right)^{1/3}\right)^n + \tilde{\Pi}\left(\frac{1}{m}\sum_{j=1}^mZ_jZ_j'>\beta^2 + \left(\frac{\beta^2}{m}\right)^{1/3}\right) \\
&\leq& \left(\beta^2 + \left(\frac{\beta^2}{m}\right)^{1/3}\right)^n + \left(\frac{\beta^2}{m}\right)^{1/3},
\end{eqnarray*}
we have
$$\frac{1}{2}\TV\left(\lambda^n,\int P_Z^n d\Pi(Z)\right)^2\leq \frac{\left(\beta^2 + \left(\frac{\beta^2}{m}\right)^{1/3}\right)^n + \left(\frac{\beta^2}{m}\right)^{1/3}}{\left(\beta-\left(\frac{\beta}{m}\right)^{1/3}\right)^{2n}\left(1-\left(\frac{\beta}{m}\right)^{1/3}\right)^{2}}-1.$$
It is clear that the above bound tends to zero when $m\rightarrow\infty$. Therefore, $\TV\left(\lambda^n,\int P_Z^n d\Pi(Z)\right)\leq\delta$ for a sufficiently large $m$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:impossibility}]
By Lemma \ref{lem:tv}, there exist $\Pi_{n,\delta}$ and $\Pi_{n+1,\delta}$ supported on $\mathcal{P}_{\delta}$, such that $\TV\left(\lambda^n, \int P^n d\Pi_{n,\delta}\right)\leq\delta$ and $\TV\left(\lambda^{n+1}, \int P^{n+1} d\Pi_{n+1,\delta}\right)\leq\delta$. Since $P^{n+1}(X_{n+1}\in \widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha$ for all $P$, we have
$$\int P^{n+1}(X_{n+1}\in \widehat{C}(X_1,\cdots,X_n))d\Pi_{n+1,\delta}\geq 1-\alpha.$$
By $\TV\left(\lambda^{n+1}, \int P^{n+1} d\Pi_{n+1,\delta}\right)\leq\delta$, we have
$$\lambda^n\lambda(\widehat{C}(X_1,\cdots,X_n))=\lambda^{n+1}(X_{n+1}\in \widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha-\delta.$$
By $\TV\left(\lambda^n, \int P^n d\Pi_{n,\delta}\right)\leq\delta$, we have
$$\int P^n\lambda(\widehat{C}(X_1,\cdots,X_n))d\Pi_{n,\delta}\geq 1-\alpha-2\delta.$$
Then, there must exists some $P\in\text{supp}(\Pi_{n,\delta})\subset\mathcal{P}_{\delta}$, such that
$$P^n\lambda(\widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha-2\delta.$$
The fact that $P\in \mathcal{P}_{\delta}$ implies $\TV(P,\lambda)\geq 1-\delta$. There exists some $B$ such that $P(B)-\lambda(B)\geq 1-\delta$, which implies $P(B)\geq 1-\delta$ and $\lambda(B)\leq\delta$, and therefore $\text{Opt}(p,1-\delta)\leq \delta$. We finally have
\begin{eqnarray*}
P^n\lambda(\widehat{C}(X_1,\cdots,X_n)) &\geq& 1-\alpha-2\delta \\
&\geq& \delta \\
&\geq& \text{Opt}(p,1-\delta) \\
&\geq& \text{Opt}(p,1-\alpha+\epsilon),
\end{eqnarray*}
as long as $\delta$ is sufficiently small so that $\delta<\min(\alpha/3, \alpha-\epsilon)$.
\end{proof}



According to the impossibility result, it is necessary to define some notion of restricted optimality. Let us define
$$\text{Opt}_k(p,1-\alpha)=\inf\left\{\vol(C_1\cup\cdots\cup C_k):P(C_1\cup\cdots\cup C_k)\geq 1-\alpha, C_j\text{ are intervals}\right\}.$$
Define $\mathcal{C}_k$ to be the collection of all union of $k$ intervals. Then, we have
$$\sup_{C\in\mathcal{C}_k}|P_n(C)-P(C)|\leq \delta_{n,k},$$
with high probability, where $P_n$ is the empirical distribution. For example, one could take $\delta_{n,k}\asymp \frac{k}{\sqrt{n}}$, or perhaps it can be improved to $\sqrt{\frac{k}{n}}$. Theorem \ref{thm:DP} shows that there is a polynomial-time algorithm that computes $\widehat{C}(X_1,\cdots,X_n)$ satisfying
$$P_n(\widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha-\gamma,$$
and
$$\lambda(\widehat{C}(X_1,\cdots,X_n))\leq \text{Opt}_k(P_n,1-\alpha).$$
Therefore, we have
$$P(\widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha-\gamma-\delta_{n,k},$$
and
\begin{eqnarray*}
\lambda(\widehat{C}(X_1,\cdots,X_n)) &\leq& \text{Opt}_k(P_n,1-\alpha) \\
&=& \inf\{\vol(C):P_n(C)\geq 1-\alpha, C\in\mathcal{C}_k\} \\
&\leq& \inf\{\vol(C):P(C)\geq 1-\alpha+\delta_{n,k}, C\in\mathcal{C}_k\} \\
&=& \text{Opt}_k(p,1-\alpha+\delta_{n,k}).
\end{eqnarray*}
In fact, one could adjust the parameter of the dynamic programming, so that with high probability, we have
$$P(\widehat{C}(X_1,\cdots,X_n))\geq 1-\alpha,$$
and
$$\lambda(\widehat{C}(X_1,\cdots,X_n))\leq \text{Opt}_k(p,1-\alpha+\gamma+2\delta_{n,k}),$$
with high probability. One could integrate out the probability tail to get in-expectation bounds (this requires additional details to be checked).

\subsection{Conformalizing DP or Greedy Algorithm}

According to the above result, one does not need to use conformal prediction to achieve coverage and restricted volume optimality. However, a conformalizing step is necessary in a supervised setting to guarantee marginal coverage even under model misspecification. Below, we first describe the conformal procedure of Chernozhukov et al., and then extend it to serve our purpose.

Let $F(y|x)=P(Y\leq y|X=x)$ be the conditional CDF. The prediction interval proposed by Chernozhukov et al. is
$$\left\{y\in\mathbb{R}:\left|\hat{F}(y|X_{n+1})-\frac{1}{2}\right|\leq t\right\},$$
where $\hat{F}(y|x)$ is assumed to be close to $F(y|x)$, and $t$ is estimated by some quantile of $$\left\{\left|\hat{F}(Y_1|X_1)-\frac{1}{2}\right|,\cdots,\left|\hat{F}(Y_n|X_n)-\frac{1}{2}\right|\right\}.$$
An asymmetric version is also discussed in their paper.

We are going to improve this idea by considering a conformalized dynamic programming procedure. Suppose $(X_1,Y_1),\cdots, (X_n,Y_n),(X_{n+1},Y_{n+1})$ are i.i.d. generated by $P$. Assume that we have access to $\hat{F}(y|x)$. We will treat $\hat{F}(y|x)$ as a fixed function, or independent from everything else. In practice, this can be guaranteed by constructing $\hat{F}(y|x)$ from an independent data set after data splitting. To measure the error of CDF, define
$$\|\hat{F}-F\|_{k,\infty}=\sup_{C\in\mathcal{C}_k}\left|\int_Cd\hat{F}-\int_CdF\right|.$$

\begin{assumption}\label{ass:F}
The conditional CDF $\hat{F}(\cdot|\cdot)$ satisfies $\mathbb{P}\left(\|\hat{F}(\cdot|X_{n+1})-F(\cdot|X_{n+1})\|_{k,\infty}\leq\delta\right)\geq 1-\delta$.
\end{assumption}
It is easy to check that the high-probability bound implies
$$\mathbb{E}\|\hat{F}(\cdot|X_{n+1})-F(\cdot|X_{n+1})\|_{k,\infty}\leq 2\delta.$$

For each $x$, suppose we construct a nested system $S_1(x)\subset\cdots\subset S_m(x)$ from $\hat{F}(y|x)$. We require that the nested system satisfies
\begin{equation}
\int_{S_j(x)}d\hat{F}(\cdot|x) = \frac{j}{m},\quad\text{for all }j\in[m]. \label{eq:eq-mass}
\end{equation}
Then, define
$$q(y,x)=\sum_{j=1}^m\mathbb{I}\{y\in S_j(x)\}.$$
The following result is a direct consequence of the nested structure.
\begin{lemma}\label{lem:nest}
For any $j\in[m+1]$, $y\in S_j(x)$ if and only if $q(y,x)\geq m-j+1$, where the set $S_{m+1}(x)$ is defined as $\mathbb{R}$.
\end{lemma}

Define $q_{(1)}\leq\cdots\leq q_{(n)}$ to be the order statistics from $q(Y_1,X_1),\cdots, q(Y_n,X_n)$. Then, the prediction interval for $Y_{n+1}$ is constructed as
$$\left\{y\in\mathbb{R}: q(y,X_{n+1})\geq q_{((n+1)\alpha)}\right\}.$$

\begin{theorem}
We have
$$\mathbb{P}\left(q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}\right)\geq 1-\alpha.$$
Suppose Assumption \ref{ass:F} holds and the nested system satisfies (\ref{eq:eq-mass}). We also have
$$\mathbb{P}\left(q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}|X_{n+1}\right)\geq 1-\alpha-3\delta,$$
with probability at least $1-\delta$.
\end{theorem}
\begin{proof}
The marginal coverage is from exchangeability. Write the $\sigma$-field generated by $(X_1,Y_1),\cdots, (X_n,Y_n)$ as $\mathcal{F}_n$. The operators $\mathbb{E}_{X_{n+1}}$ and $\mathbb{E}_{\mathcal{F}_n}$ are expectations under the marginal distributions of $X_{n+1}$ and of $(X_1,Y_1),\cdots, (X_n,Y_n)$. By Lemma \ref{lem:nest}, $q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}$ is equivalent to $Y_{n+1}\in S_{\hat{j}}(X_{n+1})$ for some $\hat{j}$ measurable with respect to $\mathcal{F}_n$. Then,
\begin{eqnarray}
\nonumber \mathbb{P}\left(q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}\right) &=& \mathbb{E}_{\mathcal{F}_n}\mathbb{E}_{X_{n+1}}\mathbb{P}\left(q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}|X_{n+1},\mathcal{F}_n\right) \\
\nonumber &=& \mathbb{E}_{\mathcal{F}_n}\mathbb{E}_{X_{n+1}}\mathbb{P}\left(Y_{n+1}\in S_{\hat{j}}(X_{n+1})|X_{n+1},\mathcal{F}_n\right) \\
\nonumber &=& \mathbb{E}_{\mathcal{F}_n}\mathbb{E}_{X_{n+1}}\int_{S_{\hat{j}}(X_{n+1})}dF(\cdot|X_{n+1}) \\
\nonumber &\leq& \mathbb{E}_{\mathcal{F}_n}\mathbb{E}_{X_{n+1}}\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1}) + \mathbb{E}\|\hat{F}(\cdot|X_{n+1})-F(\cdot|X_{n+1})\|_{k,\infty} \\
\nonumber &\leq& \mathbb{E}_{\mathcal{F}_n}\mathbb{E}_{X_{n+1}}\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1}) + 2\delta \\
\label{eq:cond-ind} &=& \mathbb{E}_{\mathcal{F}_n}\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1}) + 2\delta \\
\nonumber &\leq& \mathbb{E}_{\mathcal{F}_n}\int_{S_{\hat{j}}(X_{n+1})}dF(\cdot|X_{n+1}) + 3\delta \\
\nonumber &=& \mathbb{P}\left(q(Y_{n+1},X_{n+1})\geq q_{((n+1)\alpha)}|X_{n+1}\right) + 3\delta.
\end{eqnarray}
The equality (\ref{eq:cond-ind}) uses the fact that
$$\mathbb{E}_{X_{n+1}}\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1})=\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1}).$$
This is due to the condition (\ref{eq:eq-mass}) so that $\int_{S_{\hat{j}}(X_{n+1})}d\hat{F}(\cdot|X_{n+1})=\frac{\hat{j}}{m}$, which is independent of $X_{n+1}$, since $\hat{j}$ measurable with respect to $\mathcal{F}_n$.
\end{proof}

The above results on marginal and conditional coverage hold for arbitrary nested systems satsifying (\ref{eq:eq-mass}). To achieve volume optimality, let us assume that there exists $S_{j^*}(x)$ for some $j^*\in[m]$, such that
\begin{equation}
\int_{S_{j^*}(x)}d\hat{F}(\cdot|x)\geq 1-\alpha+\frac{1}{n}+3\delta, \label{eq:dp-c}
\end{equation}
and
\begin{equation}
\Vol(S_{j^*}(x))\leq \text{Opt}_k\left(\hat{F}(\cdot|x),1-\alpha+\frac{1}{n}+3\delta+\gamma\right), \label{eq:dp-v}
\end{equation}
for all $x$. This can be achieved by making sure $S_{j^*}(x)$ is computed by the dynamic programming.

\begin{theorem}
Suppose Assumption \ref{ass:F} holds with some $\delta^2\geq \frac{\log(2\sqrt{n})}{2n}$, and the nested system satsifying (\ref{eq:eq-mass}) contains $S_{j^*}(x)$ that satisfies (\ref{eq:dp-c}) and (\ref{eq:dp-v}). We have
$$\Vol\left(\left\{y\in\mathbb{R}: q(y,X_{n+1})\geq q_{((n+1)\alpha)}\right\}\right)\leq \text{Opt}_k\left(F(\cdot|X_{n+1}),1-\alpha+\frac{1}{n}+4\delta+\gamma\right),$$
with probability at least $1-\delta$.
\end{theorem}
\begin{proof}
Since (\ref{eq:dp-c}) holds for all $x$, we have
$$\mathbb{E}\int_{S_{j^*}(X_{n+1})}d\hat{F}(\cdot|X_{n+1})\geq 1-\alpha+\frac{1}{n}+3\delta.$$
Assumption \ref{ass:F} implies that 
\begin{eqnarray*}
\mathbb{P}\left(Y_{n+1}\in S_{j^*}(X_{n+1})\right) &=& \mathbb{E}\int_{S_{j^*}(X_{n+1})}dF(\cdot|X_{n+1}) \\
&\geq& \mathbb{E}\int_{S_{j^*}(X_{n+1})}d\hat{F}(\cdot|X_{n+1})- \mathbb{E}\|\hat{F}(\cdot|X_{n+1})-F(\cdot|X_{n+1})\|_{k,\infty}\\
&\geq& 1-\alpha+\frac{1}{n}+\delta.
\end{eqnarray*}
By Hoeffding inequality and the condition on $\delta$, we know that
$$\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{Y_i\in S_{j^*}(X_i)\}\geq \mathbb{P}\left(Y_{n+1}\in S_{j^*}(X_{n+1})\right)-\delta,$$
with probability at least $1-\delta$. Combining the two inequalities above and Lemma \ref{lem:nest}, we know that
$$\frac{1}{n}\sum_{i=1}^n\mathbb{I}\{q(Y_i,X_i)\geq m-j^*+1\}\geq 1-\alpha+\frac{1}{n}.$$
This immediately implies $q_{(n\alpha)}=q_{(n(\alpha-n^{-1})+1)}\geq m-j^*+1$ by the definition of order statistics. Therefore,
\begin{eqnarray}
\nonumber && \Vol\left(\left\{y\in\mathbb{R}: q(y,X_{n+1})\geq q_{((n+1)\alpha)}\right\}\right) \\
\nonumber &\leq& \Vol\left(\left\{y\in\mathbb{R}: q(y,X_{n+1})\geq q_{(n\alpha)}\right\}\right) \\
\nonumber &\leq& \Vol\left(\left\{y\in\mathbb{R}: q(y,X_{n+1})\geq m-j^*+1\right\}\right) \\
\nonumber &=& \Vol(S_{j^*}(X_{n+1})) \\
\label{eq:use-dp-v} &\leq& \text{Opt}_k\left(\hat{F}(\cdot|X_{n+1}),1-\alpha+\frac{1}{n}+3\delta+\gamma\right) \\
\nonumber &\leq& \text{Opt}_k\left(F(\cdot|X_{n+1}),1-\alpha+\frac{1}{n}+4\delta+\gamma\right),
\end{eqnarray}
where we have used (\ref{eq:dp-v}) in (\ref{eq:use-dp-v}).
\end{proof}

In practice, the dynamic programming works with a finite set of data points instead of a general CDF. This issue can be resolved by a discrete approximation of the conditional CDF. Given $\hat{F}(y|x)$, we independently sample $Y_1(x),\cdots,Y_L(x)$ from this distribution. Then, we can approximate $\hat{F}(y|x)$ by
$$\tilde{F}(y|x)=\frac{1}{L}\sum_{l=1}^L\mathbb{I}\{Y_l(x)\leq y\}.$$
\begin{lemma}
Suppose $\hat{F}(\cdot|\cdot)$ satisfies Assumption \ref{ass:F} with some $\delta$. Then, $\hat{F}(\cdot|\cdot)$ also satisfies the same assumption with $\delta$ replaced by $\delta + 100\sqrt{\frac{k+\log L}{L}}$.
\end{lemma}
We omit the proof of this lemma, since it is a direct consequence of the VC dimension bound of $\mathcal{C}_k$. The constant $100$ is conservative, and can be checked in the literature. If computational budget allows, we can set $L=n$ by default.

To close this section, we discuss the role of $m$. It seems that the theoretical results do not depend on $m$. This is actually not true. From (\ref{eq:eq-mass}) and (\ref{eq:dp-c}), we know that the set $S_{j^*}$ computed by dynamic programming is indexed by $j^*$ satisfying
$$\frac{j^*}{m}\geq 1-\alpha+\frac{1}{n}+3\delta.$$
Moreover, in order that the volume guarantee (\ref{eq:dp-v}) holds, the dynamic programming also requires the above inequality becomes an approximate identity, which leads to the condition $m\gg \delta^{-1}$. Therefore, we could set the default choice as $m=\sqrt{n}$.

Our theory suggests that only $S_{j^*}$ needs to be computed by the dynamic programming. The rest of the nested system does not matter. This is true if the knowledge of $\delta$ is available. Then, with $m$ sufficiently large, we can set $j^*\approx m\left(1-\alpha+\frac{1}{n}+3\delta\right)$. In practice, however, one needs to guess $\delta$ according to some conservative estimate of the error of $\hat{F}(\cdot|\cdot)$. On the other hand, suppose we know that $\delta\in [\delta_{\min},\delta_{\max}]$. As long as we have volume guarantee for all $S_j$ with $j\in\left[m\left(1-\alpha+\frac{1}{n}+3\delta_{\min}\right),m\left(1-\alpha+\frac{1}{n}+3\delta_{\max}\right)\right]$, the algorithm would automatically adapt to the correct $\delta$ in the range. In other words, volume guarantees for more than one set in the system would alleviate the need of knowing $\delta$.

\section{Volume Optimality in Supervised Settings}

In the unsupervised setting, the volume-optimal set with $1-\alpha$ coverage is given by $\{p>t\}$ for some $t$, at least when $P(p=t)=0$. This fact is analogous to Neyman-Pearson lemma, which will be the key to our understanding of the supervised setting. Recall that according to Neyman-Pearson, the solution to
$$\min Q(C)\quad\text{s.t. } P(C)\geq 1-\alpha,$$
is given b y $C=\left\{\frac{dP}{dQ}> t\right\}$ for some $t$. The original Neyman-Pearson lemma requires both $P$ and $Q$ to be probability distributions. This result is also true if $Q$ is just a sigma-finite measure (needs a reference or a proof). For example, when $Q$ is the Lebesgue measure, this leads to the solution for the volume-optimal set with $1-\alpha$ coverage.

Now let us consider a supervised setting with $(X,Y)\sim P$ with $p(x,y)$ being the joint density function. For simplicity, we assume $X\in \mathbb{R}^d$ and $Y\in\mathbb{R}$. The goal is to find a prediction set $C(x)\subset \mathbb{R}$ for each $x$ or some $R\subset\mathbb{R}^{d+1}$. The relation between $C(x)$ and $R$ is given by
$$C(x)=\{y\in\mathbb{R}:(x,y)\in R\},$$
and
$$R=\{(x,y)\in\mathbb{R}^d\times\mathbb{R}:y\in C(x)\}.$$
Generally, we have the equivalence between $y\in C(x)$ and $(x,y)\in R$.



\paragraph{Notions of Coverage.}

\begin{enumerate}
\item \textit{Marginal Coverage.} It is required that $P(Y\in C(X))\geq 1-\alpha$.
\item \textit{Conditional Coverage.} It is required that $P(Y\in C(X)|X=x)\geq 1-\alpha$ for each $x$. Without any assumption on $P$, the only valid set is $C(x)=\mathbb{R}$. Intuitively, we may never observe $X=x$.
\item \textit{Local Coverage.} It is required that $P(Y\in C(X)|X\in A)$ for all $A\in\mathcal{A}$. This notion is between marginal and conditional, and is also called group coverage in some papers. It can be easily achieved by only considering data points in $A$.
\item \textit{Coverage under Covariate-Shift.} It is required that $\int P(Y\in C(X)|X=x)q(x)dx\geq 1-\alpha$. When the distribution $q$ is the same as $p$, this is marginal coverage. When $q$ becomes a delta-measure, it is conditional coverage. Suppose conditional coverage holds, then we will have coverage under arbitrary covariate-shift.
\item \textit{Uniform Coverage under Covariate-Shift.} It is required that $\inf_{q\in\mathcal{Q}}\int P(Y\in C(X)|X=x)q(x)dx\geq 1-\alpha$, which can be achieved when the class $\mathcal{Q}$ has low complexity. I believe this one is the right notion (or the most flexible one) to work with.
\end{enumerate}

\paragraph{Notions of Volume Optimality.}

I am surprised that this part has almost never been discussed in the literature.
\begin{enumerate}
\item \textit{Naive Volume.} One hopes to optimize $\Vol(R)$, and the optimal solution under marginal coverage is given by $\{(x,y): p(x,y)> t\}$ for some $t$. This is not different from the unsupervised setting, and is not very interesting.
\item \textit{Average (Marginal) Volume.} The goal is to optimize $\int \Vol(C(x))p(x)dx$.
\item \textit{Conditional Volume.} The goal is to optimize $\Vol(C(x))$ for all/some $x$.
\item \textit{Average Volume with Covariate-Shift.} The goal is to optimize $\int\Vol(C(x))q(x)dx$.
\item \textit{Uniform Volume Control with Covariate-Shift.} The goal is to optimize $\sup_{q\in\mathcal{Q}}\int\Vol(C(x))q(x)dx$.
\end{enumerate}

\paragraph{Coverage-Volume Tradeoff.}

One can take an arbitrary notion of coverage from the list and an arbitrary notion of volume optimality from the list and solve that problem. For example, let us consider covariate shift with distribution $q$. The solution to
$$\min \int\Vol(C(x))q(x)dx\quad \text{s.t. }\int P(Y\in C(X)|X=x)q(x)dx\geq 1-\alpha$$
is given by $\{p(y|x)>t\}$ for some $t$, assuming that the density has no tie. This is by applying the Neyman-Pearson lemma and the fact that
$$p(y|x)=\frac{d(P(\cdot|\cdot)Q(\cdot))}{d(\lambda \times Q)},$$
where $\lambda$ is Lebesgue measure on $\mathbb{R}^d$ and $Q$ is a distribution on $\mathbb{R}$ with density $q$.

Interestingly, the above optimal solution does not require the knowledge of $q$. It is therefore natural to conjecture that the solution to
$$\min \sup_{q\in\mathcal{Q}}\int\Vol(C(x))q(x)dx\quad \text{s.t. }\inf_{q\in\mathcal{Q}}\int P(Y\in C(X)|X=x)q(x)dx\geq 1-\alpha$$
is still given by $\{p(y|x)>t\}$ for some $t$. Can we prove that?

\section{Notes}

General Depth-based Algorithm:
\begin{itemize}
    \item We use data points $X_1,\dots, X_n$ to construct a depth function $f : X \to \bbR$. 
    \item Compute $f(X_{n+1}),\dots,f(X_{2n})$ for data points $X_{n+1},\dots, X_{2n}$.
    \item For an error level $\alpha \in (0,1)$, we set the prediction region $\hat{C}_{\alpha} = \{x \in X : f(x) \geq f_{(\alpha n)}\}$, where $f_{(\alpha n)}$ is the $\alpha n$-th smallest value among $f(X_{n+1}),\dots,f(X_{2n})$.
\end{itemize}
We first show that this general framework satisfies the coverage condition.
\begin{theorem}
    Suppose data points $X_{n+1},\dots, X_{2n+1}$ are $i.i.d.$ For any error level $\alpha \in (0,1)$, the prediction set $\hat{C}_{\alpha}$ satisfies 
    $$
    \Pr\{X_{2n+1} \in \hat{C}_{\alpha}\} \geq 1-\alpha.
    $$
\end{theorem}

\begin{proof}
    By the construction of the prediction set, $X_{2n+1} \in \hat{C}_{\alpha}$ if and only if $f(X_{2n+1}) \geq f_{(\alpha n)}$, where $f_{\alpha n}$ is the $\alpha n$-th smallest value among $f(X_{n+1}),\dots,f(X_{2n})$. 
    Since $X_{n+1},\dots, X_{2n+1}$ are $i.i.d.$, $f(X_{2n+1})$ is uniformly distributed over values $f(X_{n+1}),\dots,f(X_{2n})$. Thus, we have
    $$
    \Pr\{X_{2n+1} \in \hat{C}_{\alpha}\}  = \Pr\{f(X_{2n+1} \geq f_{(\alpha n)})\} \geq 1-\alpha.
    $$
\end{proof}

\textbf{Observation:} Suppose pick the depth function $f$ as the pdf function $p$ of $X$.
Let $t_{\alpha}$ be the threshold such that  $\int_{p(x) \geq t_\alpha} p(x) \,\mathrm{d} x  = 1-\alpha$. Then, the minimum volume prediction set is $C^* = \{x\in X : p(x) \geq t_\alpha\}$.
Let $p_{(\alpha n)}$ be the $\alpha n$-th smallest value among $p(X_{n+1}), \dots, p(X_{2n})$. Then, the prediction set $\hat{C} = \{x\in X: p(x) \geq p_{(\alpha n)}\}$ has volume close to $\mathrm{Vol}(C^*)$,
$$
\mathrm{Vol}(\hat{C}) = (1+o(1))\mathrm{Vol}(C^*).
$$

Algorithm 2:
\begin{itemize}
    \item For each point $x_i$ ($i$ from $1$ to $n$), let $E_i$ be the smallest volume Ellipsoid containing $x_i$ and $0.02n$ other points.
    \item Let the depth function $f(x) = 1/\mathrm{Vol}(E_x)$, where the set $E_x$ is the smallest ellipsoid among the $n$ ellipsoids $E_1, \dots, E_n$ containing $x$.
    \item Run the depth-based conformal prediction with the depth function $f$.
\end{itemize}

\textbf{Hardness:} \cite*{bruna2021continuous} showed the hardness of the Continuous Learning with errors (CLWE) and its decision variant. 
The decision variant of the continuous LWE is to distinguish the CLWE samples $(y_i,z_i)$ from the samples where $z_i$ is uniformly sampled from $[0,1)$. It is also hard to distinguish the standard Gaussian distribution from the mixture of "Gaussian pancakes", which is the mixture of equally spaced Gaussian components with separation $1/\sqrt{d}$.

\section{One Dimensional Robust Conformal Prediction}

\subsection{Conformal Prediction without Features}

Let $Y_i$, $i=1,\dots, 2n$ be i.i.d. data points sampled from the distribution $(1-\varepsilon)P+\varepsilon \cdot Q$ on $\bbR$. Consider a new data point $Y_{2n+1}$ sampled from $P$, which is independent of $Y_i$, $i=1,\dots, 2n$. Given an error level $\alpha \in (0,1)$, we want to find a prediction region $\hat{C} \subset \bbR$ such that
\begin{enumerate}
    \item It holds that
    $$
    \Pr\{Y_{2n+1} \in \hat{C}\} \geq 1-\alpha.
    $$
    \item 
    If the distribution $P = \calN(0,\sigma^2)$, then the volume of the prediction region $\hat{C}$ is comparable to $\sigma^2$ with high probability.
\end{enumerate}

% Algorithm:
% \begin{enumerate}
%     \item Split the data points $Y_i$, $i=1,\dots,2n$ into two sets 
%     \begin{align*}
%     D_1 &= \{Y_i: i=1,2,\dots, n\}; \\
%     D_2 &= \{Y_i: i=n+1,n+2,\dots, 2n\}.
%     \end{align*}
%     \item Set $\hat{\mu} = \mathrm{Med}(D_1)$ be the median of points in $D_1$. 
%     \item Set $R_i = |Y_i - \hat{\mu}|$ for $i = n+1,\dots, 2n$ be the residual for points in $D_2$. 
%     \item Output $\hat{C} = [\hat{\mu}- q, \hat{\mu}+q]$, where $q = \lceil(1-\alpha)(n+1) + 2\varepsilon \cdot n \rceil$-th smallest of $R_i$, $i = n+1,\dots, 2n$. 
% \end{enumerate}

% \begin{theorem}
%     For any error level $\alpha > 2\varepsilon$, the prediction region $\hat{C}$ satisfies that 
%     $$
%     \Pr\{Y_{2n+1} \in \hat{C}\} \geq 1-\alpha - e^{-2\varepsilon n}.
%     $$
% \end{theorem}

% \begin{proof}
%     Let $R_{2n+1} = Y_{2n+1} - \hat{\mu}$ be the residual for the new data point $Y_{2n+1}$. 
%     For points in $D_2$, we consider the following generating process, which is equivalent to the original sampling process. 
%     For each $Y_i \in D_2$, we first sample a random variable $Z_i$ from the Bernoulli distribution with probability $\varepsilon$. 
%     If $Z_i = 1$, then $Y_i$ is sampled from $Q$; otherwise, it is sampled from $P$. We first sample all $Z_i$ for $Y_i$ in $D_2$. Then, let $G_2 = \{Y_i: Z_i = 0, i=n+1,n+2,\dots,2n \}$ be the random variables $Y_i$ corresponding to $Z_i = 0$ in $D_2$. Note that random variables $Y_i$ in $G_2$  are i.i.d. sampled from distribution $P$. 
%     Let $B_2= D_2 \setminus G_2$ be random variables sampled from $Q$ in $D_2$. Then, we have $|B_2| = \sum_{i=n+1}^{2n} Z_i$. Since $Z_i$ are i.i.d. Bernoulli random variables, by Chernoff bound, we have 
%     $$
%     \Pr\{|B_2| \geq 2\varepsilon n \}\leq (e^{-1}/4)^{\varepsilon n} \leq e^{-2\varepsilon n}.
%     $$
%     With probability at least $1-e^{-2\varepsilon n}$, we have at most $2\varepsilon n$ points in $B_2$.
    
%     Note that $Y_{2n+1} \in \hat{C}$ if and only if $R_{2n+1}$ is among the $q = \lceil(1-\alpha)(n+1) + 2\varepsilon \cdot n \rceil$-th smallest of $R_i$, $i = n+1,\dots, 2n, 2n+1$.  Suppose $|B_2| \leq 2\varepsilon n$. If $R_{2n+1}$ is among the $\lceil(1-\alpha)(n+1) \rceil$ smallest of $R_i$ corresponding to $Y_i \in G_2$ and $Y_{2n+1}$, then $R_{2n+1}$ is among the $q = \lceil(1-\alpha)(n+1) + 2\varepsilon \cdot n \rceil$ smallest of $R_i$, $i = n+1,\dots, 2n, 2n+1$, which implies $Y_{2n+1} \in \hat{C}$. Since $Y_i \in G_2$ and $Y_{2n+1}$ are i.i.d. sampled from $P$ and $\hat{\mu}$ is computed from the points in $D_1$, the residual $R_{i}$ for $Y_i \in G_2$ and $Y_{2n+1}$ are independent i.i.d. random variables. Thus, we have
%     $$
%     \Pr\{Y_{2n+1} \,\text{is among the $\lceil(1-\alpha)(n+1) \rceil$ smallest of $R_i$ for $Y_i \in G_2$ and $Y_{2n+1}$}\} \geq 1-\alpha.
%     $$
%     This holds when $|B_2| \leq 2\varepsilon n$. By the union bound, we have 
%     $$
%     \Pr\{Y_{2n+1} \in \hat{C}\} \geq 1-\alpha - e^{-2\varepsilon n}.
%     $$
% \end{proof}

% \begin{theorem}
%     For the number of points $2n \geq C/\varepsilon^2$ for some constant $C$, the volume of the prediction region given by our algorithm is at most $2(\mathrm{Quantile}_P(1-(\alpha - 6\varepsilon)/2) + \varepsilon)$, where $\mathrm{Quantile}_P$ is the quantile function for $P$. The smallest region when the density function of $P$ is known has the volume $2\mathrm{Quantile}_P(1-(1-\alpha)/2)$. 
% \end{theorem}

% \begin{proof}
%     We first bound the volume of the smallest region when the density function of $P$ is known. Let $F$ be the cumulative distribution function for $P = \calN(\mu,\sigma^2)$. Then, for $\alpha \in (0,1)$, the smallest region is $C^* = [\mu - q^*, \mu+q^*]$ where $q^*$ satisfies $F(\mu+q^*) - F(\mu-q^*) = 1-\alpha$. We have for any $t > 0$
%     $$
%     \frac{\sigma t}{(t^2+1)\sqrt{2\pi}}e^{-t^2/2\sigma^2} \leq  1-(F(\mu+t) - F(\mu-t)) \leq \frac{\sigma}{t\sqrt{2\pi}}e^{-t^2/2\sigma^2}.
%     $$

%     We now bound the volume of our prediction set $\hat{C}$. Suppose $D_2$ contains at most $2\varepsilon n$ points sampled from $Q$. This condition holds with probability at least $1-e^{-2\varepsilon n}$.
%     Let $q' = q - |\mu- \hat{\mu}|$. We have that interval $[\mu-q', \mu+q']$ is a subset of $[\hat{\mu}-q, \hat{\mu}+q]$. Let $p = F(\mu+q') - F(\mu-q')$ be the probability that a point sampled from $P$ is in $[\mu-q', \mu+q']$.

%     Then, we show that $p \leq 1-\alpha + 6\varepsilon$ with probability at least $1-e^{-\varepsilon^2 n}$. We use $G_2$ to denote the random points sampled from $P$. Since there are at least $1-2\varepsilon n$ points in $G_2$, we pick a subset $G_2'$ of $G_2$ with $n-2\varepsilon n$ points. 
%     Let $q''$ be the threshold such that $F(\mu+q'') - F(\mu-q'') = 1-\alpha + 6
%     \varepsilon$. If there are more than $(1-\alpha)(n+1) + 2\varepsilon n$ points in $G_2'$ satisfies $Y_i \in [\mu-q'',\mu+q'']$, then we have $q,q'$ given by our algorithm satisfies $q' \leq q''$ and $p \leq 1-\alpha + 6\varepsilon$. Let $Z$ be the number of points in $G_2'$ contained in $[\mu-q'',\mu+q'']$. By Hoeffding's inequality, we have for $\alpha > 6\varepsilon$
%     $$
%     \Pr\{Z \leq (1-\alpha)(n+1)+2\varepsilon n\} = \Pr\{Z \leq (1-\alpha+6\varepsilon)(n-2\varepsilon n+1) -\varepsilon n\} \leq e^{-\varepsilon^2 n}.
%     $$
%     Thus, we have $p \leq 1-\alpha + 6\varepsilon$ with probability at least $1-e^{-\varepsilon^2 n}$. 

%     If $p \leq 1-\alpha + 6\varepsilon$, we have $q' \leq \sqrt{2\sigma} \cdot \mathrm{erf}^{-1}(1-(\alpha-6\varepsilon)/2)$. When the number of points $n$ is greater than $C/\varepsilon^2$, we have $|\hat{\mu} -\mu| \leq \varepsilon$. In this case, we have $q = q'+|\hat{\mu} -\mu| \leq q' + \varepsilon$.
% \end{proof}

% \subsection{Conformal Prediction with Features}

% Let $(X_i,Y_i)$, $i =1,2,\dots,2n$ be the set of i.i.d. data sampled from the distribution $(1-\varepsilon)P+\varepsilon \cdot Q$ on $\calX \times \calY$. We first consider the feature space $\calX = \bbR^d$ and the label space $\calY = \bbR$.
% Consider a new data point $(X_{2n+1},Y_{2n+1})$ sampled from $P$, which is independent of $(X_i,Y_i)$, $i =1,2,\dots,2n$. 

% Given the feature $X_{2n+1}$ and $\alpha \in (0,1)$, we want to find a prediction region $\hat{C}(X_{2n+1})$ such that 
% \begin{enumerate}
%     \item It holds that
%     $$
%     \Pr\{Y_{2n+1} \in \hat{C}(X_{2n+1})\} \geq 1-\alpha.
%     $$
%     \item 
%     If the distribution $P|_X = f(X) + \calN(0,\sigma^2)$, then the volume of the prediction region $\hat{C}(X_{2n+1})$ is comparable to $\sigma^2$ with high probability.
% \end{enumerate}

% Algorithm:

% \begin{enumerate}
%     \item Split the data $(X_i,Y_i)$, $i=1,\dots,2n$ into two sets 
%     \begin{align*}
%     D_1 &= \{(X_i,Y_i), i=1,2,\dots, n\}; \\
%     D_2 &= \{(X_i,Y_i), i=n+1,n+2,\dots, 2n\}.
%     \end{align*}
%     \item 
% \end{enumerate}

\subsection{One Dimensional Setting}

We consider a one-dimensional distribution $\calD$ on $\bbR$. Suppose $C^*_1,C^*_2,\dots, C^*_k$ is one of the optimal solution that covers $1-\alpha$ fraction of probability mass in $\calD$. Let $\calF$ be the family of all intervals. 

\begin{theorem}
    Given a one-dimensional distribution $\calD$ on $\bbR$ and confidence level $\alpha$, let $C^*_1,C^*_2,\dots, C^*_k$ is one of the optimal solution (minimum volume) that covers $1-\alpha$ fraction of probability mass in $\calD$.
    For any $\gamma \geq \epsilon > 0$, Algorithm Greedy Marginal Density outputs $t = O(k/\gamma)$ sets $S_1, S_2, \dots, S_t \in \calF$ such that $\Pr_\calD[S_1 \cup \dots \cup S_t] \ge 1-\alpha -\gamma$ such that 
    
    \begin{equation}\label{eq:unions_1d}
        \vol(S_1 \cup \dots \cup S_t) \le 6 \cdot (\vol(C^*_1)+\dots+\vol(C^*_k)).
    \end{equation}

\end{theorem}

Intuition: At each iteration $t$, we divide the optimal sets $C^*_i$ into two types: (1) heavy set; and (2) light set. A set $C^*_i$ is called a heavy set in iteration $t$ if 
$\Pr_{\calD}[C^*_i \setminus (S_1\cup \dots \cup S_{t-1})] \geq \gamma /k$. The rest optimal sets are called light sets. Then, we consider different cases according to whether $S_t$ partially covers some heavy sets. For each set $S_t$, we bound the part of $S_t$ that is in the heavy sets and the part that is not in the heavy sets separately. For the part of $S_t$ not in the heavy sets, we find an equivalent set in the heavy set that is uncovered yet such that this set covers the same amount of probability mass and the volume of this set can upper bound the volume of the part of $S_t$ outside the heavy sets.

\begin{proof}
    We consider the set $S_t$ chosen in each iteration of the algorithm. We consider the following cases: (1) $S_t$ is contained in some $C^*_i$, $S_t \subseteq C^*_i$; (2) $S_t$ only fully covers some $C^*_i$, $C^*_i \subseteq S_t$; (3) $S_t$ partially covers one set $C^*_i$, which means $C^*_i\cap S_t\neq \varnothing$ and $C^*_i \setminus S_t \neq \varnothing$; (4) $S_t$ partially covers two sets $C^*_i, C^*_j$; (5) $S_t$ is disjoint with any $C^*_i$. (In these cases, we only consider those sets  $C^*_i$ with $\Pr_{\calD} [C^*_i \setminus (S_1\cup \dots \cup S_{t-1})] \geq \gamma/k$.)

    First, the case (5) can not happen. Since the algorithm stops only when $\Pr(S_1\cup \dots \cup S_t) \geq 1-\alpha - \gamma$. Thus, in each iteration, there exists a set $C^*_i$ such that $\Pr_{\calD}[C^*_i\setminus (S_1\cup \dots \cup S_{t-1})] \geq \gamma/k$. If $S_t$ is disjoint with any $C^*_i$, then since the density of $S_t \setminus (S_1\cup \dots \cup S_{t-1})$ is larger than the density of $C^*_i\setminus (S_1\cup \dots \cup S_{t-1})$, by moving the low-density region in $C^*_i$ to $S_t$ will provide a solution with smaller volume. Then, we will focus on cases that can happen. 

    The first case that $S_t$ is contained in some optimal set $C^*_i$ is easy for us. 
    
    Now, we consider the second case. In this case, the set $S_t$ fully covers some optimal sets $C^*_i$ (it may fully cover multiple optimal sets). Let $I_t$ be the indices of optimal sets that are covered by $S_t$ and $\vol(C^*_i \setminus (S_1\cup \dots \cup S_{t-1})) \geq \gamma/k$. Then, we only need to bound the volume of set $S'_t = S_t \setminus (S_1\cup \dots \cup S_t)$ excluding $C^*_i$ for $i \in I_t$. Hence, we consider the part $S'_t \setminus \bigcup_{i \in I_t} C^*_i$ and bound its volume by some uncovered portion of the optimal solution. We sort the sets $C^*_i \setminus (S_1 \cup \dots \cup S_t)$ that has the probability mass $\Pr_{\calD} [C^*_i \setminus (S_1 \cup \dots \cup S_t)] \geq \gamma/k$ by their density in a decreasing order. We use $C^t_1,C^t_2,\dots, C^t_{k_t}$ to denote the sorted sequence of these sets. If the probability mass of $S'_t\setminus \bigcup_{i \in I_t} C^*_i$ is greater than the total probability mass that covered by $C^t_1,C^t_2, \dots, C^t_{k_t}$. Then, we know that the algorithm will stop after this iteration and $\Pr_{\calD}(S_t) \leq 1-\alpha$. If the probability mass of $S'_t\setminus \bigcup_{i \in I_t} C^*_i$ is at most the total probability mass that covered by $C^t_1,C^t_2, \dots, C^t_{k_t}$, then we use $S''_t$ be the densest set in $C^t_1,C^t_2, \dots, C^t_{k_t}$ that covers $\Pr_{\calD} [S'_t\setminus \bigcup_{i \in I_t} C^*_i]$ probability mass. ($S''_t$ is not required to be an interval. ) Then, since the density of $S'_t$ is larger than any set $C^*_i \setminus (S_1\cup\dots\cup S_{t-1})$, we have the density of $S'_t\setminus \bigcup_{i \in I_t} C^*_i$ is larger than the density of any set $C^t_1,C^t_2, \dots, C^t_{k_t}$. Thus, we have $\vol(S'_t\setminus \bigcup_{i \in I_t} C^*_i) \leq \vol(S''_t)$. In the analysis of the later iteration, we add the set $S''_t$ into the covered set $S_1,\dots, S_{t}$. 

    Then, we analyze the third and fourth cases. We first show that these two cases are essentially similar and provide an analysis for both cases. In the third case, we know that one endpoint of $S_t$ is contained in a set $C^*_i$ that is partially covered by $S_t$. We show that the other endpoint of set $S_t$ is exactly at the endpoint of some set $C^*_j$, which means it exactly covers a set $C^*_j$ on the other side. If this is not the case, then we know there is an interval on the other end of set $S_t$ which is not contained in any $C^*_i$. Since the density of this interval is no larger than the density of sets $C^*_i$, we can shift the endpoints of $S_t$ such that it fully covers $C^*_i$ and get a set with a higher marginal density. 

    Thus, we consider the third and fourth cases in the following approach. Let $C^*_i$ and $C^*_j$ be two sets that contain the endpoints of $S_t$. Let $S'_t = S_t \setminus (S_1\cup \dots \cup S_{t-1})$. Let $A_1 = S'_t \cap C^*_i$ and $A_2 = S'_t \cap C^*_j$ and $B_1 = S'_t \setminus C^*_i$ and $B_2 = S'_t \setminus C^*_j$. (For the third case, $B_1$ or $B_2$ is empty.)  
    Let $I_t$ be the indices of optimal sets that are fully covered $S_t$ and $\vol(C^*_i \setminus (S_1\cup \dots \cup S_{t-1})) \geq \gamma/k$. Let $A = S'_t \setminus \bigcup_{i \in I_t} C^*_i $ and $A_3 = A \setminus (A_1 \cup A_2)$. 
    Let $C^t_i = C^*_i \setminus (S_1\cup \dots \cup S_{t-1})$ and $C^t_j = C^*_j \setminus (S_1\cup \dots \cup S_{t-1})$.

    
    \begin{lemma}
        Suppose the density of $A_3$ is at most $\rho(A_3) \leq 1/2 
        \cdot \max\{\rho(B_1), \rho(B_2)\}$, where $\rho(S) = \Pr_{\calD}[S]/\vol(S)$ is the density of set $S$. Then, we have $\vol(A_3) \leq 4[\vol(C^t_i) + \vol(C^t_j)]$.
    \end{lemma}

    \begin{proof}
        We prove this by contradiction. Suppose $\vol(A_3) \geq 4[\vol(C^t_i) + \vol(C^t_j)]$. Without loss of generality, we assume that $\Pr_{\calD}[A_1] \leq \Pr_{\calD}[A_2]$. Note that $A = A_1 \cup A_2 \cup A_3$. Then, we have 
        $$
        \rho(A) = \frac{\Pr_{\calD}[A]}{\vol(A)} \leq \frac{\Pr_{\calD}[A_3]}{\vol(A)} + \frac{2\Pr_{\calD}[A_2]}{\vol(A)} \leq \rho(A_3) + \frac{2 \Pr_{\calD}[A_2]}{4\vol(C^t_j)} \leq  \frac{1}{2} \max\{\rho(B_1),\rho(B_2)\} + \frac{1}{2}\rho(C^t_j).
        $$
        Since the density of $S'_t$ is at least the density of any set $C^*_i\setminus (S_1\cup \dots \cup S_{t-1})$ for $i \in I_t$, we have the density of $A$ is at least the density of $S'_t$, $\rho(A) \geq \rho(S'_t)$.
        Note that $\rho(S'_t) \geq \rho(B_1)$, $\rho(S'_t) \geq \rho(B_2)$ since otherwise we can include $B_1$ and $B_2$ and construct a denser interval. Since the algorithm picks the densest interval, we have $\rho(S'_t) \geq \rho(C^t_j)$.
        
        However, we have $\rho(S'_t) \geq \rho(B_1)$, $\rho(S'_t) \geq \rho(B_2)$ and $\rho(S'_t) \geq \rho(C^t_j)$, which provides a contradiction.
    \end{proof}


    Thus, if $\rho(A_3) \leq 1/2 \cdot \max\{\rho(B_1), \rho(B_2)\}$, then we can bound the volume of $A_3$ by the above lemma. Now, suppose $\rho(A_3) > 1/2 \cdot \max\{\rho(B_1), \rho(B_2)\}$. Then, we will find an uncovered set in the optimal solution that covers the same probability mass. If $\Pr_{\calD}[A_3] \leq \Pr_{\calD} [B_1 \cup B_2]$. Let $S''_t \subseteq B_1 \cup B_2$ be the lowest density set in $B_1\cup B_2$ that covers $\Pr_{\calD} [A_3]$ probability mass. Thus, we have $\rho(S''_t) \leq 2 \rho(A_3)$. Then, we have $\vol(A_3) \leq 2\vol(S''_t)$. If $\Pr_{\calD}[A_3] > \Pr_{\calD} [B_1 \cup B_2]$, then we consider $A_3$ with the uniform mass (only for analysis) and first move $\Pr_{\calD}[B_1\cup B_2]$ mass in $A_3$ to $B_1\cup B_2$. Let $A_3'$ be a subset of $A_3$ that covers $\Pr_{\calD}[B_1\cup B_2]$ probability mass. Then, we have $\vol(A_3') \leq 2\vol(B_1 \cup B_2)$. Since $S'_t$ has the maximum marginal density, we have $\rho(S'_t) \geq \rho(C^t_i)$ for any heavy set $C^t_i$. Since $\rho(A_3) \leq \rho(B_1 \cup B_2)$, we have $\rho(A_3) \geq \rho(C^t_j)$ for any uncovered heavy set $C^t_j$. Thus, we can find a set $S''_t$ in the uncovered heavy sets to cover the rest amount of mass in $A_3$. Let $A_3'' = A_3 \setminus A_3'$. Then, we have $\vol(A_3'') \leq \vol(S''_t)$.

    Therefore, by combining all the above cases, we have that the part of $S_t$ which is not contained in some heavy sets $C^*_i$ can be bounded by the four times the volume of heavy sets that cover the same amount of probability mass. By adding the part of $S_t$ contained in heavy sets and the set in the last iteration, we have the conclusion.
\end{proof}


\subsection{One Dimensional Setting New}

We consider a one-dimensional distribution $\calD$ on $\bbR$. 
Let $\calF$ be the family of all intervals. 
We modify the Algorithm Greedy Marginal Density as follows. At each iteration, we find the interval $S_t \in \calF$ that it covers exactly $\gamma/2k$ probability mass, $\Pr_D\{S_t \setminus (S_1\cup S_2\cup \dots\cup S_{t-1})\} = \gamma/2k$. The algorithm stops if $\Pr_D\{S_1\cup S_2\cup \dots\cup S_{t}\} \geq 1-\alpha - 2\gamma$. 


\begin{theorem}\label{thm:greedy-1d}
    Given a one-dimensional distribution $\calD$ on $\bbR$ and confidence level $\alpha$, let $C^*_1,C^*_2,\dots, C^*_k$ be the unique optimal solution that cover $1-\alpha-\gamma$ fraction of probability mass in $\calD$.
    For any $\gamma > 0$, Algorithm Greedy Marginal Density outputs $t = O(k/\gamma)$ sets $S_1, S_2, \dots, S_t \in \calF$ such that $\Pr_\calD[S_1 \cup \dots \cup S_t] \ge 1-\alpha - 2\gamma$ such that 
    
    \begin{equation}\label{eq:unions_1d}
        \vol(S_1 \cup \dots \cup S_t) \leq  \opt(p,1-\alpha).
    \end{equation}

\end{theorem}


\begin{proof}
    If the interval $S_t$ is fully contained in some interval $C^*_i$, then it is easy for us since it is fully contained in an optimal solution. 

    Now, suppose $S_t \setminus (C^*_1\cup \dots \cup C^*_k) \neq \varnothing$. Then, we consider the following two cases: (1) $S_t$ intersects with only one $C^*_i$; (2) $S_t$ intersects with multiple $C^*_i$. 

    Consider the first case that $S_t \cap C^*_i \neq \varnothing$ and $S_t \cap C^*_j =\varnothing$ for all $j\neq i$. Then, we have $C^*_i \subset S_1\cup \dots \cup S_t$. Suppose $C^*_i$ is not fully covered by $S_1 \cup \dots \cup S_t$. Since $C^*_1,\dots, C^*_k$ is the unique optimal solution that covers $1-\alpha-\gamma$ fraction of probability mass, we have the density of $C^*_i \setminus (S_1\cup\dots\cup S_t)$ is larger than the density of $S_t \setminus C^*_i$. Then, we can find an interval which has a larger marginal density than $S_t$. Thus, there are at most $k$ such intervals $S_t$ that fully cover the remaining part of some $C^*_i$. For an interval $S_t$ in this case, let $A_t = S_t \setminus C^*_i$. Since the marginal density of $S_t$ is at least $t(p,1-\alpha-\gamma)$ and the marginal probability mass coverage of $S_t$ is $\gamma/2k$, we have 
    $$
    \vol(A_t) \leq \frac{\gamma}{2k \cdot t(p,1-\alpha-\gamma)}.
    $$

    Now we consider the second case that $S_t$ intersects more than one $C^*_i$. 
    Consider two intervals $C^*_i$ and $C^*_j$ that intersect with $S_t$. If there are some parts between two intervals $C^*_i$ and $C^*_j$ are not covered by $S_1\cup\dots \cup S_{t-1}$. Then, $S_t$ will fully cover all parts between two intervals. Since there are at most $k$ intervals $C^*_i$, there are at most $k-1$ such $S_t$. Let $A_t = S_t \setminus (C*_1\cup\dots\cup C^*_k)$. Then, we have
    $$
    \vol(A_t) \leq \frac{\gamma}{2k \cdot t(p,1-\alpha-\gamma)}.
    $$
    If there is no uncovered part between optimal intervals that are first covered by $S_t$, then we must have $S_t$ fully cover some $C^*_i$ which is not fully covered by $S_1,\cdots, S_{t-1}$. This is equivalent to a first case set. 

    Let $A = (S_1 \cup\dots\cup S_t)\setminus (C^*_1 \cup\dots\cup C^*_k)$ be the set covered by the algorithm solution $S_1, \dots,S_t$ but not by the optimal solution $C^*_1,\dots, C^*_k$. By combining two cases above, we have 
    $$
    \vol(A) \leq \frac{\gamma}{t(p,1-\alpha-\gamma)} \leq \opt(p,1-\alpha) - \vol (C^*_1 \cup \dots \cup C^*_k).
    $$
\end{proof}

Without the uniqueness of the optimal solution for $1-\alpha-\gamma$, we can get a $2$ approximation in volume with the analysis in section 6.2.

I think the modified greedy algorithm works without the uniqueness assumption.

\begin{proof}
    We use the uniqueness assumption only for the first case that $S_t$ intersects with exactly one $C^*_i$ and $S_t \setminus (C^*_1\cup \dots\cup C^*_k) \neq \varnothing$. 
    We now show that for each $C^*_i$, the total volume that is covered by such $S_t$ and is not inside $C^*_i$ is at most $\gamma/(k\cdot t(p,1-\alpha-\gamma))$. (Actually, we can do a better analysis by combining the first and second cases.)

    If $S_1\cup\dots\cup S_t$ fully covers $C^*_i$, then we are good. Now suppose $C^*_i \setminus (S_1\cup \dots \cup S_t) \neq \varnothing$. Let $A_t = S_t \setminus (C^*_i \cup S_1\cup\dots \cup S_{t-1})$. Since this set $S_t$ has the maximum marginal density among sets that cover $\gamma/2k$ marginal probability mass, we have the density of $A_t$ is $t(p,1-\alpha-\gamma)$. Also, we have the uncovered portion of $C^*_i$ with probability mass $\Pr_D\{A_t\}$ closest to $S_t$ has density $t(p,1-\alpha-\gamma)$. In this case, the density remains the same by shifting $S_t$ to cover more portion of $C^*_i$. Since the marginal probability coverage of $S_t$ is $\gamma/2k$, we have $\Pr_D\{A_t\} \leq \gamma / 2k$. 
    If there is a set $S_{t'}$ for $t' > t$ that covers the part $A_{t'}$ that are further away than $A_t$, then we show that $\Pr_D\{A_{t'} \cup A_t\}\leq \gamma/2k$. 
    We know that $S_{t'}$ covers a part $B_{t'} \subset C^*_i$ with probability mass $\Pr_D\{B_{t'}\} = \Pr_D\{A_t\}$ and density $t(p,1-\alpha-\gamma)$. Thus, we have $\Pr_D\{A_{t'} \cup A_t\} = \Pr_D\{B_{t'} \cup A_{t'}\} \leq \Pr_D\{S_{t'}\} \leq \gamma/2k$. Since this set $S_{t'}$ has the maximum marginal density, there is an uncovered portion of $C^*_i$ with probability mass $\Pr_D\{A_t \cup A_{t'}\}$ closest to $S_{t'}$ has density $t(p,1-\alpha-\gamma)$. Therefore, a similar analysis holds for more such sets $S_t$. 
\end{proof}
